A Swift Look at SN 2011fe: The Earliest Ultraviolet Observations of a Type Ia Supernova

We present the earliest ultraviolet (UV) observations of the bright Type Ia supernova SN 2011fe/PTF11kly in the nearby galaxy M101 at a distance of only 6.4 Mpc. It was discovered shortly after explosion by the Palomar Transient Factory and first observed by Swift/UVOT about a day after explosion. The early UV light is well-defined, with ~20 data points per filter in the five days after explosion. These early and well-sampled UV observations form new template light curves for comparison with observations of other SNe Ia at low and high redshift. We report fits from semi-empirical models of the explosion and find the time evolution of the early UV flux to be well fit by the superposition of two parabolic curves. Finally, we use the early UV flux measurements to examine a possible shock interaction with a non-degenerate companion. From models predicting the measurable shock emission, we find that even a solar mass companion at a distance of a few solar radii is unlikely at more than 95% confidence.

==> tab1.tex <==
uvw2 & 55797.9285 & \nodata  & 18.80 &   0.10 $ \pm $  0.06 &    6.03e-13 $ \pm $    3.59e-13 \\ 
uvw2 & 55797.9954 & \nodata  & 18.80 &   0.14 $ \pm $  0.07 &    7.92e-13 $ \pm $    3.65e-13 \\ 
uvw2 & 55799.0045 & 17.53 $ \pm $ 0.16 & 18.42 &   0.87 $ \pm $  0.13 &    5.15e-12 $ \pm $    7.58e-13 \\ 
uvw2 & 55799.1339 & 17.59 $ \pm $ 0.15 & 18.56 &   0.82 $ \pm $  0.11 &    4.90e-12 $ \pm $    6.67e-13 \\ 
uvw2 & 55799.2115 & 17.46 $ \pm $ 0.14 & 18.50 &   0.93 $ \pm $  0.12 &    5.43e-12 $ \pm $    6.97e-13 \\ 
uvw2 & 55799.4016 & 17.42 $ \pm $ 0.14 & 18.48 &   0.96 $ \pm $  0.12 &    5.83e-12 $ \pm $    7.34e-13 \\ 
uvw2 & 55799.5407 & 17.29 $ \pm $ 0.12 & 18.51 &   1.09 $ \pm $  0.12 &    6.42e-12 $ \pm $    6.94e-13 \\ 
uvw2 & 55800.0696 & 16.84 $ \pm $ 0.09 & 18.33 &   1.64 $ \pm $  0.14 &    9.67e-12 $ \pm $    8.24e-13 \\ 
uvw2 & 55800.2071 & 16.67 $ \pm $ 0.10 & 18.08 &   1.93 $ \pm $  0.18 &    1.14e-11 $ \pm $    1.04e-12 \\ 
uvw2 & 55800.3419 & 16.67 $ \pm $ 0.09 & 18.18 &   1.92 $ \pm $  0.16 &    1.13e-11 $ \pm $    9.31e-13 \\ 
uvw2 & 55800.6152 & 16.45 $ \pm $ 0.07 & 18.24 &   2.35 $ \pm $  0.15 &    1.37e-11 $ \pm $    8.79e-13 \\ 
uvw2 & 55800.7380 & 16.34 $ \pm $ 0.07 & 18.07 &   2.61 $ \pm $  0.18 &    1.53e-11 $ \pm $    1.03e-12 \\ 
uvw2 & 55800.8097 & 16.21 $ \pm $ 0.08 & 17.81 &   2.94 $ \pm $  0.22 &    1.72e-11 $ \pm $    1.31e-12 \\ 
uvw2 & 55800.9362 & 16.16 $ \pm $ 0.09 & 17.74 &   3.07 $ \pm $  0.24 &    1.79e-11 $ \pm $    1.39e-12 \\ 
uvw2 & 55801.0265 & 16.22 $ \pm $ 0.10 & 17.68 &   2.90 $ \pm $  0.25 &    1.70e-11 $ \pm $    1.48e-12 \\ 
uvw2 & 55801.1410 & 16.06 $ \pm $ 0.07 & 17.84 &   3.38 $ \pm $  0.22 &    1.96e-11 $ \pm $    1.27e-12 \\ 
uvw2 & 55801.2218 & 16.08 $ \pm $ 0.07 & 17.91 &   3.31 $ \pm $  0.20 &    1.94e-11 $ \pm $    1.19e-12 \\ 
uvw2 & 55801.2868 & 16.05 $ \pm $ 0.08 & 17.68 &   3.40 $ \pm $  0.25 &    1.97e-11 $ \pm $    1.46e-12 \\ 
uvw2 & 55801.4155 & 16.01 $ \pm $ 0.09 & 17.53 &   3.52 $ \pm $  0.29 &    2.06e-11 $ \pm $    1.70e-12 \\ 
uvw2 & 55801.4891 & 15.84 $ \pm $ 0.06 & 17.77 &   4.14 $ \pm $  0.23 &    2.40e-11 $ \pm $    1.35e-12 \\ 
uvw2 & 55801.5599 & 15.85 $ \pm $ 0.08 & 17.48 &   4.08 $ \pm $  0.30 &    2.38e-11 $ \pm $    1.77e-12 \\ 
uvw2 & 55801.6875 & 15.84 $ \pm $ 0.07 & 17.57 &   4.12 $ \pm $  0.28 &    2.42e-11 $ \pm $    1.64e-12 \\ 
uvw2 & 55801.8229 & 15.68 $ \pm $ 0.07 & 17.52 &   4.78 $ \pm $  0.29 &    2.82e-11 $ \pm $    1.73e-12 \\ 
uvw2 & 55801.9535 & 15.59 $ \pm $ 0.07 & 17.41 &   5.19 $ \pm $  0.32 &    3.09e-11 $ \pm $    1.93e-12 \\ 
uvw2 & 55802.0284 & 15.53 $ \pm $ 0.06 & 17.43 &   5.47 $ \pm $  0.32 &    3.23e-11 $ \pm $    1.87e-12 \\ 
uvw2 & 55802.1573 & 15.38 $ \pm $ 0.05 & 17.46 &   6.32 $ \pm $  0.31 &    3.79e-11 $ \pm $    1.86e-12 \\ 
uvw2 & 55802.2175 & 15.42 $ \pm $ 0.05 & 17.61 &   6.06 $ \pm $  0.27 &    3.58e-11 $ \pm $    1.59e-12 \\ 
uvw2 & 55803.0186 & 14.91 $ \pm $ 0.08 & 16.61 &   9.75 $ \pm $  0.68 &    6.14e-11 $ \pm $    4.28e-12 \\ 
uvw2 & 55804.2967 & 14.15 $ \pm $ 0.04 & 16.50 &  19.52 $ \pm $  0.75 &    1.31e-10 $ \pm $    5.06e-12 \\ 
uvw2 & 55805.3656 & 13.66 $ \pm $ 0.04 & 16.11 &  30.71 $ \pm $  1.08 &    2.18e-10 $ \pm $    7.65e-12 \\ 
uvw2 & 55805.4179 & 13.63 $ \pm $ 0.04 & 16.09 &  31.66 $ \pm $  1.10 &    2.25e-10 $ \pm $    7.80e-12 \\ 
uvw2 & 55806.3603 & 13.32 $ \pm $ 0.04 & 15.80 &  42.00 $ \pm $  1.43 &    3.09e-10 $ \pm $    1.05e-11 \\ 
uvw2 & 55806.7572 & 13.21 $ \pm $ 0.04 & 15.66 &  46.52 $ \pm $  1.62 &    3.43e-10 $ \pm $    1.19e-11 \\ 
uvw2 & 55807.0345 & 13.16 $ \pm $ 0.04 & 15.45 &  48.70 $ \pm $  1.97 &    3.57e-10 $ \pm $    1.44e-11 \\ 
uvw2 & 55807.1008 & 13.11 $ \pm $ 0.04 & 15.54 &  50.85 $ \pm $  1.81 &    3.73e-10 $ \pm $    1.33e-11 \\ 
uvw2 & 55807.1708 & 13.10 $ \pm $ 0.04 & 15.54 &  51.57 $ \pm $  1.81 &    3.81e-10 $ \pm $    1.34e-11 \\ 
uvw2 & 55807.3048 & 13.06 $ \pm $ 0.04 & 15.51 &  53.65 $ \pm $  1.88 &    3.96e-10 $ \pm $    1.38e-11 \\ 
uvw2 & 55807.4355 & 13.03 $ \pm $ 0.04 & 15.47 &  54.94 $ \pm $  1.94 &    4.06e-10 $ \pm $    1.44e-11 \\ 
uvw2 & 55807.6930 & 13.03 $ \pm $ 0.06 & 15.05 &  54.83 $ \pm $  2.85 &    4.07e-10 $ \pm $    2.12e-11 \\ 
uvw2 & 55807.6938 & 13.09 $ \pm $ 0.04 & 15.51 &  52.24 $ \pm $  1.87 &    3.88e-10 $ \pm $    1.39e-11 \\ 
uvw2 & 55807.7012 & 13.01 $ \pm $ 0.04 & 15.51 &  55.84 $ \pm $  1.87 &    4.13e-10 $ \pm $    1.38e-11 \\ 
uvw2 & 55807.8228 & 12.97 $ \pm $ 0.04 & 15.46 &  58.09 $ \pm $  1.95 &    4.33e-10 $ \pm $    1.45e-11 \\ 
uvw2 & 55808.0416 & 12.93 $ \pm $ 0.04 & 15.39 &  60.40 $ \pm $  2.09 &    4.52e-10 $ \pm $    1.56e-11 \\ 
uvw2 & 55808.1023 & 12.91 $ \pm $ 0.04 & 15.35 &  61.42 $ \pm $  2.17 &    4.59e-10 $ \pm $    1.62e-11 \\ 
uvw2 & 55808.2336 & 12.91 $ \pm $ 0.04 & 15.33 &  61.26 $ \pm $  2.19 &    4.57e-10 $ \pm $    1.64e-11 \\ 
uvw2 & 55808.7598 & 12.88 $ \pm $ 0.04 & 15.33 &  62.87 $ \pm $  2.21 &    4.73e-10 $ \pm $    1.66e-11 \\ 
uvw2 & 55808.7678 & 12.85 $ \pm $ 0.04 & 15.36 &  64.92 $ \pm $  2.15 &    4.84e-10 $ \pm $    1.60e-11 \\ 
uvw2 & 55808.9014 & 12.82 $ \pm $ 0.04 & 15.28 &  66.62 $ \pm $  2.30 &    4.98e-10 $ \pm $    1.72e-11 \\ 
uvw2 & 55809.3615 & 12.86 $ \pm $ 0.04 & 15.36 &  64.55 $ \pm $  2.14 &    4.80e-10 $ \pm $    1.59e-11 \\ 
uvw2 & 55809.6401 & 12.77 $ \pm $ 0.04 & 15.26 &  70.07 $ \pm $  2.35 &    5.25e-10 $ \pm $    1.77e-11 \\ 
uvw2 & 55809.7605 & 12.66 $ \pm $ 0.05 & 14.81 &  77.41 $ \pm $  3.55 &    5.83e-10 $ \pm $    2.67e-11 \\ 
uvw2 & 55809.7613 & 12.73 $ \pm $ 0.04 & 15.18 &  72.08 $ \pm $  2.52 &    5.43e-10 $ \pm $    1.90e-11 \\ 
uvw2 & 55810.1104 & 12.72 $ \pm $ 0.04 & 15.23 &  72.77 $ \pm $  2.41 &    5.45e-10 $ \pm $    1.81e-11 \\ 
uvw2 & 55810.2983 & 12.69 $ \pm $ 0.04 & 15.20 &  75.06 $ \pm $  2.48 &    5.66e-10 $ \pm $    1.87e-11 \\ 
uvw2 & 55811.0317 & 12.69 $ \pm $ 0.05 & 14.93 &  74.99 $ \pm $  3.20 &    5.71e-10 $ \pm $    2.43e-11 \\ 
uvw2 & 55811.0327 & 12.65 $ \pm $ 0.04 & 15.12 &  78.24 $ \pm $  2.67 &    5.96e-10 $ \pm $    2.03e-11 \\ 
uvw2 & 55811.1840 & 12.60 $ \pm $ 0.04 & 15.08 &  81.35 $ \pm $  2.77 &    6.13e-10 $ \pm $    2.09e-11 \\ 
uvw2 & 55811.2510 & 12.60 $ \pm $ 0.04 & 15.05 &  81.53 $ \pm $  2.84 &    6.17e-10 $ \pm $    2.15e-11 \\ 
uvw2 & 55811.3174 & 12.61 $ \pm $ 0.04 & 15.08 &  81.22 $ \pm $  2.78 &    6.14e-10 $ \pm $    2.10e-11 \\ 
uvw2 & 55811.4514 & 12.62 $ \pm $ 0.04 & 15.09 &  80.11 $ \pm $  2.74 &    6.06e-10 $ \pm $    2.07e-11 \\ 
uvw2 & 55811.6342 & 12.59 $ \pm $ 0.05 & 14.83 &  82.30 $ \pm $  3.48 &    6.22e-10 $ \pm $    2.63e-11 \\ 
uvw2 & 55811.6352 & 12.64 $ \pm $ 0.04 & 15.11 &  78.32 $ \pm $  2.69 &    5.92e-10 $ \pm $    2.03e-11 \\ 
uvw2 & 55812.3723 & 12.59 $ \pm $ 0.04 & 15.07 &  82.45 $ \pm $  2.79 &    6.30e-10 $ \pm $    2.13e-11 \\ 
uvw2 & 55812.5726 & 12.65 $ \pm $ 0.04 & 15.11 &  78.29 $ \pm $  2.70 &    5.92e-10 $ \pm $    2.04e-11 \\ 
uvw2 & 55813.1161 & 12.59 $ \pm $ 0.04 & 15.06 &  82.33 $ \pm $  2.82 &    6.25e-10 $ \pm $    2.14e-11 \\ 
uvw2 & 55814.2524 & 12.62 $ \pm $ 0.04 & 14.89 &  80.22 $ \pm $  3.29 &    6.17e-10 $ \pm $    2.53e-11 \\ 
uvw2 & 55814.2536 & 12.61 $ \pm $ 0.04 & 15.09 &  80.97 $ \pm $  2.75 &    6.23e-10 $ \pm $    2.12e-11 \\ 
uvw2 & 55814.3277 & 12.60 $ \pm $ 0.04 & 15.08 &  81.49 $ \pm $  2.77 &    6.28e-10 $ \pm $    2.13e-11 \\ 
uvw2 & 55814.3938 & 12.61 $ \pm $ 0.04 & 15.09 &  80.89 $ \pm $  2.76 &    6.23e-10 $ \pm $    2.12e-11 \\ 
uvw2 & 55814.4618 & 12.62 $ \pm $ 0.04 & 15.10 &  79.99 $ \pm $  2.72 &    6.16e-10 $ \pm $    2.09e-11 \\ 
uvw2 & 55814.7905 & 12.62 $ \pm $ 0.04 & 15.08 &  80.02 $ \pm $  2.77 &    6.15e-10 $ \pm $    2.13e-11 \\ 
uvw2 & 55814.8605 & 12.63 $ \pm $ 0.04 & 15.10 &  79.43 $ \pm $  2.72 &    6.13e-10 $ \pm $    2.10e-11 \\ 
uvw2 & 55814.9134 & 12.66 $ \pm $ 0.04 & 15.00 &  77.09 $ \pm $  2.97 &    5.93e-10 $ \pm $    2.29e-11 \\ 
uvw2 & 55814.9151 & 12.63 $ \pm $ 0.04 & 15.12 &  79.44 $ \pm $  2.67 &    6.11e-10 $ \pm $    2.06e-11 \\ 
uvw2 & 55814.9994 & 12.63 $ \pm $ 0.04 & 15.10 &  79.27 $ \pm $  2.72 &    6.09e-10 $ \pm $    2.09e-11 \\ 
uvw2 & 55815.2528 & 12.65 $ \pm $ 0.04 & 15.15 &  77.85 $ \pm $  2.60 &    5.95e-10 $ \pm $    1.99e-11 \\ 
uvw2 & 55815.3919 & 12.69 $ \pm $ 0.04 & 15.16 &  75.14 $ \pm $  2.57 &    5.81e-10 $ \pm $    1.99e-11 \\ 
uvw2 & 55816.3175 & 12.71 $ \pm $ 0.04 & 15.02 &  74.10 $ \pm $  2.92 &    5.70e-10 $ \pm $    2.25e-11 \\ 
uvw2 & 55816.3184 & 12.73 $ \pm $ 0.04 & 15.17 &  72.18 $ \pm $  2.55 &    5.55e-10 $ \pm $    1.96e-11 \\ 
uvw2 & 55816.3250 & 12.72 $ \pm $ 0.04 & 15.21 &  72.76 $ \pm $  2.47 &    5.60e-10 $ \pm $    1.90e-11 \\ 
uvw2 & 55816.3885 & 12.75 $ \pm $ 0.04 & 15.23 &  70.94 $ \pm $  2.42 &    5.48e-10 $ \pm $    1.87e-11 \\ 
uvw2 & 55817.1879 & 12.81 $ \pm $ 0.04 & 15.22 &  67.39 $ \pm $  2.43 &    5.18e-10 $ \pm $    1.87e-11 \\ 
uvw2 & 55817.2042 & 12.79 $ \pm $ 0.04 & 15.25 &  68.32 $ \pm $  2.36 &    5.25e-10 $ \pm $    1.82e-11 \\ 
uvw2 & 55817.2552 & 12.78 $ \pm $ 0.04 & 15.20 &  69.29 $ \pm $  2.49 &    5.32e-10 $ \pm $    1.91e-11 \\ 
uvw2 & 55817.2703 & 12.78 $ \pm $ 0.04 & 15.23 &  69.33 $ \pm $  2.41 &    5.32e-10 $ \pm $    1.85e-11 \\ 
uvw2 & 55817.3219 & 12.75 $ \pm $ 0.04 & 15.17 &  71.29 $ \pm $  2.56 &    5.47e-10 $ \pm $    1.96e-11 \\ 
uvw2 & 55817.3349 & 12.80 $ \pm $ 0.04 & 15.25 &  67.58 $ \pm $  2.38 &    5.19e-10 $ \pm $    1.83e-11 \\ 
uvw2 & 55817.3886 & 12.76 $ \pm $ 0.04 & 15.18 &  70.37 $ \pm $  2.54 &    5.40e-10 $ \pm $    1.95e-11 \\ 
uvw2 & 55817.3970 & 12.80 $ \pm $ 0.04 & 15.20 &  67.78 $ \pm $  2.48 &    5.20e-10 $ \pm $    1.91e-11 \\ 
uvw2 & 55817.4685 & 12.86 $ \pm $ 0.04 & 15.23 &  64.44 $ \pm $  2.42 &    4.94e-10 $ \pm $    1.86e-11 \\ 
uvw2 & 55817.4748 & 12.80 $ \pm $ 0.04 & 15.14 &  68.14 $ \pm $  2.63 &    5.23e-10 $ \pm $    2.02e-11 \\ 
uvw2 & 55817.8633 & 12.86 $ \pm $ 0.04 & 15.36 &  64.52 $ \pm $  2.15 &    4.94e-10 $ \pm $    1.65e-11 \\ 
uvw2 & 55817.9397 & 12.85 $ \pm $ 0.04 & 15.29 &  65.16 $ \pm $  2.27 &    4.99e-10 $ \pm $    1.74e-11 \\ 
uvw2 & 55817.9998 & 12.85 $ \pm $ 0.04 & 15.23 &  64.89 $ \pm $  2.41 &    4.96e-10 $ \pm $    1.84e-11 \\ 
uvw2 & 55818.4028 & 12.92 $ \pm $ 0.04 & 15.42 &  60.75 $ \pm $  2.02 &    4.61e-10 $ \pm $    1.53e-11 \\ 
uvw2 & 55819.0638 & 13.03 $ \pm $ 0.04 & 15.49 &  55.04 $ \pm $  1.89 &    4.20e-10 $ \pm $    1.44e-11 \\ 
uvw2 & 55820.0830 & 13.11 $ \pm $ 0.04 & 15.50 &  50.86 $ \pm $  1.89 &    3.77e-10 $ \pm $    1.40e-11 \\ 
uvw2 & 55820.1497 & 13.15 $ \pm $ 0.04 & 15.51 &  49.34 $ \pm $  1.86 &    3.65e-10 $ \pm $    1.38e-11 \\ 
uvw2 & 55820.2170 & 13.10 $ \pm $ 0.04 & 15.48 &  51.61 $ \pm $  1.91 &    3.80e-10 $ \pm $    1.41e-11 \\ 
uvw2 & 55820.2837 & 13.10 $ \pm $ 0.04 & 15.47 &  51.56 $ \pm $  1.93 &    3.79e-10 $ \pm $    1.42e-11 \\ 
uvw2 & 55820.3510 & 13.08 $ \pm $ 0.04 & 15.46 &  52.45 $ \pm $  1.95 &    3.85e-10 $ \pm $    1.43e-11 \\ 
uvw2 & 55820.8724 & 13.23 $ \pm $ 0.06 & 15.27 &  45.52 $ \pm $  2.33 &    3.31e-10 $ \pm $    1.70e-11 \\ 
uvw2 & 55820.8735 & 13.20 $ \pm $ 0.04 & 15.62 &  47.18 $ \pm $  1.69 &    3.43e-10 $ \pm $    1.23e-11 \\ 
uvw2 & 55820.9377 & 13.26 $ \pm $ 0.05 & 15.41 &  44.61 $ \pm $  2.05 &    3.27e-10 $ \pm $    1.50e-11 \\ 
uvw2 & 55820.9393 & 13.22 $ \pm $ 0.04 & 15.66 &  46.25 $ \pm $  1.62 &    3.39e-10 $ \pm $    1.19e-11 \\ 
uvw2 & 55822.2116 & 13.31 $ \pm $ 0.06 & 15.26 &  42.33 $ \pm $  2.35 &    3.04e-10 $ \pm $    1.69e-11 \\ 
uvw2 & 55822.2125 & 13.40 $ \pm $ 0.04 & 15.79 &  39.13 $ \pm $  1.45 &    2.81e-10 $ \pm $    1.04e-11 \\ 
uvw2 & 55822.8811 & 13.54 $ \pm $ 0.07 & 15.35 &  34.48 $ \pm $  2.16 &    2.45e-10 $ \pm $    1.54e-11 \\ 
uvw2 & 55822.8820 & 13.47 $ \pm $ 0.04 & 15.83 &  36.78 $ \pm $  1.39 &    2.62e-10 $ \pm $    9.86e-12 \\ 
uvw2 & 55823.0150 & 13.42 $ \pm $ 0.06 & 15.36 &  38.32 $ \pm $  2.15 &    2.72e-10 $ \pm $    1.53e-11 \\ 
uvw2 & 55823.0160 & 13.50 $ \pm $ 0.04 & 15.89 &  35.55 $ \pm $  1.32 &    2.53e-10 $ \pm $    9.37e-12 \\ 
uvw2 & 55823.0825 & 13.50 $ \pm $ 0.07 & 15.32 &  35.64 $ \pm $  2.21 &    2.48e-10 $ \pm $    1.54e-11 \\ 
uvw2 & 55823.0834 & 13.45 $ \pm $ 0.04 & 15.81 &  37.48 $ \pm $  1.42 &    2.60e-10 $ \pm $    9.85e-12 \\ 
uvw2 & 55824.4213 & 13.67 $ \pm $ 0.07 & 15.39 &  30.43 $ \pm $  2.08 &    2.10e-10 $ \pm $    1.43e-11 \\ 
uvw2 & 55824.4222 & 13.68 $ \pm $ 0.04 & 16.01 &  30.16 $ \pm $  1.18 &    2.08e-10 $ \pm $    8.12e-12 \\ 
uvw2 & 55825.2920 & 13.77 $ \pm $ 0.06 & 15.77 &  27.90 $ \pm $  1.46 &    1.93e-10 $ \pm $    1.01e-11 \\ 
uvw2 & 55825.2937 & 13.78 $ \pm $ 0.04 & 16.19 &  27.46 $ \pm $  1.00 &    1.90e-10 $ \pm $    6.90e-12 \\ 
uvw2 & 55826.9044 & 14.06 $ \pm $ 0.08 & 15.75 &  21.30 $ \pm $  1.50 &    1.45e-10 $ \pm $    1.02e-11 \\ 
uvw2 & 55826.9054 & 14.02 $ \pm $ 0.04 & 16.33 &  22.17 $ \pm $  0.88 &    1.51e-10 $ \pm $    5.96e-12 \\ 
uvw2 & 55826.9686 & 13.95 $ \pm $ 0.08 & 15.58 &  23.61 $ \pm $  1.74 &    1.59e-10 $ \pm $    1.17e-11 \\ 
uvw2 & 55826.9695 & 14.00 $ \pm $ 0.04 & 16.29 &  22.44 $ \pm $  0.91 &    1.51e-10 $ \pm $    6.13e-12 \\ 
uvw2 & 55827.0382 & 14.06 $ \pm $ 0.09 & 15.61 &  21.23 $ \pm $  1.71 &    1.50e-10 $ \pm $    1.20e-11 \\ 
uvw2 & 55827.0390 & 14.00 $ \pm $ 0.04 & 16.27 &  22.48 $ \pm $  0.92 &    1.58e-10 $ \pm $    6.51e-12 \\ 
uvw2 & 55827.0519 & 13.98 $ \pm $ 0.06 & 15.99 &  22.86 $ \pm $  1.20 &    1.56e-10 $ \pm $    8.17e-12 \\ 
uvw2 & 55827.1127 & 14.00 $ \pm $ 0.04 & 16.25 &  22.57 $ \pm $  0.94 &    1.53e-10 $ \pm $    6.37e-12 \\ 
uvw2 & 55827.2475 & 14.02 $ \pm $ 0.05 & 16.24 &  22.01 $ \pm $  0.95 &    1.49e-10 $ \pm $    6.47e-12 \\ 
uvw2 & 55827.3107 & 14.03 $ \pm $ 0.05 & 16.27 &  21.95 $ \pm $  0.93 &    1.49e-10 $ \pm $    6.29e-12 \\ 
uvw2 & 55827.4447 & 13.99 $ \pm $ 0.05 & 16.23 &  22.67 $ \pm $  0.96 &    1.54e-10 $ \pm $    6.55e-12 \\ 
uvw2 & 55827.5189 & 14.04 $ \pm $ 0.04 & 16.32 &  21.73 $ \pm $  0.89 &    1.48e-10 $ \pm $    6.03e-12 \\ 
uvw2 & 55827.6545 & 14.11 $ \pm $ 0.05 & 16.30 &  20.27 $ \pm $  0.90 &    1.38e-10 $ \pm $    6.13e-12 \\ 
uvw2 & 55829.4403 & 14.16 $ \pm $ 0.07 & 15.87 &  19.33 $ \pm $  1.34 &    1.30e-10 $ \pm $    9.01e-12 \\ 
uvw2 & 55829.4415 & 14.32 $ \pm $ 0.04 & 16.60 &  16.73 $ \pm $  0.68 &    1.12e-10 $ \pm $    4.57e-12 \\ 
uvw2 & 55829.5104 & 14.41 $ \pm $ 0.10 & 15.82 &  15.41 $ \pm $  1.40 &    1.04e-10 $ \pm $    9.44e-12 \\ 
uvw2 & 55829.5113 & 14.32 $ \pm $ 0.05 & 16.53 &  16.76 $ \pm $  0.73 &    1.13e-10 $ \pm $    4.90e-12 \\ 
uvw2 & 55829.8412 & 14.28 $ \pm $ 0.10 & 15.71 &  17.46 $ \pm $  1.54 &    1.15e-10 $ \pm $    1.02e-11 \\ 
uvw2 & 55829.8420 & 14.36 $ \pm $ 0.05 & 16.55 &  16.20 $ \pm $  0.72 &    1.07e-10 $ \pm $    4.74e-12 \\ 
uvw2 & 55829.8594 & 14.29 $ \pm $ 0.05 & 16.36 &  17.27 $ \pm $  0.85 &    1.16e-10 $ \pm $    5.72e-12 \\ 
uvw2 & 55829.9751 & 14.35 $ \pm $ 0.05 & 16.57 &  16.26 $ \pm $  0.70 &    1.09e-10 $ \pm $    4.71e-12 \\ 
uvw2 & 55829.9924 & 14.34 $ \pm $ 0.05 & 16.58 &  16.45 $ \pm $  0.70 &    1.10e-10 $ \pm $    4.69e-12 \\ 
uvw2 & 55830.0557 & 14.35 $ \pm $ 0.05 & 16.53 &  16.28 $ \pm $  0.73 &    1.09e-10 $ \pm $    4.89e-12 \\ 
uvw2 & 55830.3899 & 14.49 $ \pm $ 0.05 & 16.58 &  14.36 $ \pm $  0.69 &    9.72e-11 $ \pm $    4.70e-12 \\ 
uvw2 & 55830.5280 & 14.39 $ \pm $ 0.05 & 16.54 &  15.70 $ \pm $  0.72 &    1.05e-10 $ \pm $    4.80e-12 \\ 
uvw2 & 55831.7902 & 14.67 $ \pm $ 0.10 & 16.10 &  12.10 $ \pm $  1.08 &    8.25e-11 $ \pm $    7.37e-12 \\ 
uvw2 & 55831.7913 & 14.59 $ \pm $ 0.05 & 16.81 &  13.11 $ \pm $  0.56 &    8.94e-11 $ \pm $    3.85e-12 \\ 
uvw2 & 55831.9131 & 14.50 $ \pm $ 0.10 & 15.96 &  14.17 $ \pm $  1.24 &    9.06e-11 $ \pm $    7.92e-12 \\ 
uvw2 & 55831.9141 & 14.56 $ \pm $ 0.05 & 16.76 &  13.47 $ \pm $  0.59 &    8.61e-11 $ \pm $    3.78e-12 \\ 
uvw2 & 55832.9829 & 14.73 $ \pm $ 0.11 & 16.03 &  11.44 $ \pm $  1.16 &    7.70e-11 $ \pm $    7.79e-12 \\ 
uvw2 & 55832.9838 & 14.76 $ \pm $ 0.05 & 16.89 &  11.16 $ \pm $  0.52 &    7.51e-11 $ \pm $    3.52e-12 \\ 
uvw2 & 55833.1173 & 14.88 $ \pm $ 0.10 & 16.28 &  10.00 $ \pm $  0.92 &    6.68e-11 $ \pm $    6.13e-12 \\ 
uvw2 & 55833.1347 & 14.75 $ \pm $ 0.05 & 16.89 &  11.24 $ \pm $  0.52 &    7.52e-11 $ \pm $    3.48e-12 \\ 
uvw2 & 55833.1839 & 14.70 $ \pm $ 0.09 & 16.20 &  11.86 $ \pm $  0.99 &    7.94e-11 $ \pm $    6.64e-12 \\ 
uvw2 & 55833.2014 & 14.72 $ \pm $ 0.05 & 16.87 &  11.59 $ \pm $  0.53 &    7.78e-11 $ \pm $    3.59e-12 \\ 
uvw2 & 55833.2505 & 14.81 $ \pm $ 0.07 & 16.54 &  10.64 $ \pm $  0.72 &    7.15e-11 $ \pm $    4.87e-12 \\ 
uvw2 & 55833.2634 & 14.82 $ \pm $ 0.06 & 16.85 &  10.53 $ \pm $  0.54 &    7.08e-11 $ \pm $    3.65e-12 \\ 
uvw2 & 55833.3212 & 14.75 $ \pm $ 0.06 & 16.69 &  11.26 $ \pm $  0.63 &    7.59e-11 $ \pm $    4.23e-12 \\ 
uvw2 & 55833.3356 & 14.74 $ \pm $ 0.05 & 16.82 &  11.38 $ \pm $  0.56 &    7.67e-11 $ \pm $    3.76e-12 \\ 
uvw2 & 55833.3842 & 14.73 $ \pm $ 0.06 & 16.79 &  11.43 $ \pm $  0.57 &    7.72e-11 $ \pm $    3.88e-12 \\ 
uvw2 & 55833.4021 & 14.78 $ \pm $ 0.05 & 16.91 &  10.97 $ \pm $  0.52 &    7.42e-11 $ \pm $    3.49e-12 \\ 
uvw2 & 55833.4526 & 14.86 $ \pm $ 0.09 & 16.41 &  10.21 $ \pm $  0.81 &    6.92e-11 $ \pm $    5.52e-12 \\ 
uvw2 & 55833.4544 & 14.76 $ \pm $ 0.05 & 17.01 &  11.14 $ \pm $  0.47 &    7.55e-11 $ \pm $    3.17e-12 \\ 
uvw2 & 55833.5230 & 14.67 $ \pm $ 0.11 & 15.98 &  12.15 $ \pm $  1.21 &    8.24e-11 $ \pm $    8.21e-12 \\ 
uvw2 & 55833.5240 & 14.79 $ \pm $ 0.05 & 16.90 &  10.89 $ \pm $  0.52 &    7.39e-11 $ \pm $    3.53e-12 \\ 
uvw2 & 55835.3895 & 15.00 $ \pm $ 0.10 & 16.44 &   8.94 $ \pm $  0.79 &    5.87e-11 $ \pm $    5.20e-12 \\ 
uvw2 & 55835.3911 & 14.91 $ \pm $ 0.05 & 17.10 &   9.77 $ \pm $  0.43 &    6.42e-11 $ \pm $    2.83e-12 \\ 
uvw2 & 55835.4591 & 14.97 $ \pm $ 0.11 & 16.24 &   9.23 $ \pm $  0.95 &    5.95e-11 $ \pm $    6.13e-12 \\ 
uvw2 & 55835.4602 & 15.00 $ \pm $ 0.05 & 17.10 &   8.95 $ \pm $  0.43 &    5.76e-11 $ \pm $    2.78e-12 \\ 
uvw2 & 55836.4638 & 15.07 $ \pm $ 0.05 & 17.18 &   8.40 $ \pm $  0.40 &    5.81e-11 $ \pm $    2.77e-12 \\ 
uvw2 & 55836.5320 & 15.15 $ \pm $ 0.12 & 16.33 &   7.79 $ \pm $  0.88 &    5.09e-11 $ \pm $    5.72e-12 \\ 
uvw2 & 55836.5331 & 15.05 $ \pm $ 0.05 & 17.13 &   8.57 $ \pm $  0.42 &    5.60e-11 $ \pm $    2.73e-12 \\ 
uvw2 & 55836.6802 & 15.10 $ \pm $ 0.07 & 16.96 &   8.14 $ \pm $  0.49 &    5.25e-11 $ \pm $    3.16e-12 \\ 
uvw2 & 55836.7385 & 15.14 $ \pm $ 0.07 & 16.98 &   7.86 $ \pm $  0.48 &    5.07e-11 $ \pm $    3.12e-12 \\ 
uvw2 & 55836.8052 & 15.08 $ \pm $ 0.07 & 16.94 &   8.35 $ \pm $  0.50 &    5.38e-11 $ \pm $    3.21e-12 \\ 
uvw2 & 55836.8718 & 15.05 $ \pm $ 0.06 & 16.92 &   8.58 $ \pm $  0.51 &    5.53e-11 $ \pm $    3.28e-12 \\ 
uvw2 & 55836.9392 & 15.12 $ \pm $ 0.07 & 16.96 &   8.00 $ \pm $  0.49 &    5.14e-11 $ \pm $    3.15e-12 \\ 
uvw2 & 55837.0112 & 15.09 $ \pm $ 0.06 & 17.10 &   8.25 $ \pm $  0.43 &    5.29e-11 $ \pm $    2.77e-12 \\ 
uvw2 & 55837.0612 & 15.16 $ \pm $ 0.06 & 17.11 &   7.69 $ \pm $  0.43 &    4.93e-11 $ \pm $    2.74e-12 \\ 
uvw2 & 55837.0725 & 15.06 $ \pm $ 0.06 & 16.93 &   8.46 $ \pm $  0.50 &    5.42e-11 $ \pm $    3.22e-12 \\ 
uvw2 & 55837.1283 & 15.19 $ \pm $ 0.08 & 16.82 &   7.50 $ \pm $  0.56 &    4.80e-11 $ \pm $    3.58e-12 \\ 
uvw2 & 55837.1392 & 15.09 $ \pm $ 0.07 & 16.95 &   8.26 $ \pm $  0.50 &    5.28e-11 $ \pm $    3.18e-12 \\ 
uvw2 & 55837.2054 & 15.19 $ \pm $ 0.10 & 16.53 &   7.51 $ \pm $  0.73 &    4.79e-11 $ \pm $    4.64e-12 \\ 
uvw2 & 55837.2143 & 15.07 $ \pm $ 0.07 & 16.84 &   8.37 $ \pm $  0.55 &    5.33e-11 $ \pm $    3.48e-12 \\ 
uvw2 & 55837.3958 & 15.27 $ \pm $ 0.12 & 16.45 &   6.96 $ \pm $  0.79 &    4.42e-11 $ \pm $    5.00e-12 \\ 
uvw2 & 55837.3970 & 15.21 $ \pm $ 0.06 & 17.27 &   7.35 $ \pm $  0.37 &    4.67e-11 $ \pm $    2.35e-12 \\ 
uvw2 & 55838.3336 & 15.17 $ \pm $ 0.10 & 16.55 &   7.66 $ \pm $  0.72 &    5.12e-11 $ \pm $    4.79e-12 \\ 
uvw2 & 55838.3352 & 15.24 $ \pm $ 0.05 & 17.36 &   7.16 $ \pm $  0.34 &    4.79e-11 $ \pm $    2.27e-12 \\ 
uvw2 & 55838.9378 & 15.21 $ \pm $ 0.12 & 16.37 &   7.37 $ \pm $  0.84 &    4.66e-11 $ \pm $    5.33e-12 \\ 
uvw2 & 55838.9389 & 15.27 $ \pm $ 0.06 & 17.29 &   6.99 $ \pm $  0.36 &    4.42e-11 $ \pm $    2.30e-12 \\ 
uvw2 & 55839.6081 & 15.17 $ \pm $ 0.12 & 16.37 &   7.68 $ \pm $  0.84 &    4.88e-11 $ \pm $    5.36e-12 \\ 
uvw2 & 55839.6093 & 15.38 $ \pm $ 0.06 & 17.36 &   6.32 $ \pm $  0.34 &    4.02e-11 $ \pm $    2.15e-12 \\ 
uvw2 & 55840.2080 & 15.30 $ \pm $ 0.12 & 16.54 &   6.79 $ \pm $  0.72 &    4.44e-11 $ \pm $    4.72e-12 \\ 
uvw2 & 55840.2095 & 15.41 $ \pm $ 0.06 & 17.44 &   6.13 $ \pm $  0.31 &    4.00e-11 $ \pm $    2.05e-12 \\ 
uvw2 & 55840.3482 & 15.29 $ \pm $ 0.16 & 16.19 &   6.87 $ \pm $  1.00 &    4.50e-11 $ \pm $    6.52e-12 \\ 
uvw2 & 55840.3490 & 15.44 $ \pm $ 0.07 & 17.28 &   6.00 $ \pm $  0.37 &    3.93e-11 $ \pm $    2.40e-12 \\ 
uvw2 & 55841.3412 & 15.31 $ \pm $ 0.12 & 16.47 &   6.72 $ \pm $  0.77 &    4.46e-11 $ \pm $    5.12e-12 \\ 
uvw2 & 55841.3425 & 15.40 $ \pm $ 0.06 & 17.39 &   6.19 $ \pm $  0.33 &    4.11e-11 $ \pm $    2.18e-12 \\ 
uvw2 & 55841.8837 & 15.56 $ \pm $ 0.15 & 16.52 &   5.36 $ \pm $  0.73 &    3.35e-11 $ \pm $    4.58e-12 \\ 
uvw2 & 55841.8848 & 15.46 $ \pm $ 0.06 & 17.40 &   5.83 $ \pm $  0.33 &    3.64e-11 $ \pm $    2.05e-12 \\ 
uvw2 & 55842.0079 & 15.52 $ \pm $ 0.18 & 16.28 &   5.54 $ \pm $  0.92 &    3.97e-11 $ \pm $    6.56e-12 \\ 
uvw2 & 55842.0087 & 15.47 $ \pm $ 0.07 & 17.27 &   5.82 $ \pm $  0.37 &    4.17e-11 $ \pm $    2.64e-12 \\ 
uvw2 & 55842.0268 & 15.47 $ \pm $ 0.08 & 17.07 &   5.79 $ \pm $  0.44 &    3.88e-11 $ \pm $    2.97e-12 \\ 
uvw2 & 55842.0932 & 15.48 $ \pm $ 0.07 & 17.31 &   5.75 $ \pm $  0.35 &    3.84e-11 $ \pm $    2.37e-12 \\ 
uvw2 & 55842.1604 & 15.48 $ \pm $ 0.07 & 17.35 &   5.76 $ \pm $  0.34 &    3.85e-11 $ \pm $    2.29e-12 \\ 
uvw2 & 55842.3489 & 15.57 $ \pm $ 0.15 & 16.53 &   5.28 $ \pm $  0.73 &    3.77e-11 $ \pm $    5.23e-12 \\ 
uvw2 & 55842.3500 & 15.42 $ \pm $ 0.06 & 17.37 &   6.08 $ \pm $  0.34 &    4.35e-11 $ \pm $    2.41e-12 \\ 
uvw2 & 55842.5653 & 15.49 $ \pm $ 0.07 & 17.36 &   5.72 $ \pm $  0.34 &    3.78e-11 $ \pm $    2.25e-12 \\ 
uvw2 & 55842.8878 & 15.64 $ \pm $ 0.15 & 16.56 &   4.97 $ \pm $  0.71 &    3.33e-11 $ \pm $    4.75e-12 \\ 
uvw2 & 55842.8889 & 15.53 $ \pm $ 0.06 & 17.44 &   5.49 $ \pm $  0.32 &    3.68e-11 $ \pm $    2.12e-12 \\ 
uvw2 & 55842.9612 & 15.55 $ \pm $ 0.07 & 17.36 &   5.40 $ \pm $  0.34 &    3.61e-11 $ \pm $    2.28e-12 \\ 
uvw2 & 55843.4823 & 15.55 $ \pm $ 0.15 & 16.52 &   5.38 $ \pm $  0.74 &    3.63e-11 $ \pm $    4.96e-12 \\ 
uvw2 & 55843.4834 & 15.54 $ \pm $ 0.06 & 17.45 &   5.42 $ \pm $  0.31 &    3.65e-11 $ \pm $    2.10e-12 \\ 
uvw2 & 55843.7468 & 15.59 $ \pm $ 0.16 & 16.46 &   5.22 $ \pm $  0.78 &    3.35e-11 $ \pm $    4.99e-12 \\ 
uvw2 & 55843.7478 & 15.60 $ \pm $ 0.07 & 17.44 &   5.14 $ \pm $  0.32 &    3.30e-11 $ \pm $    2.02e-12 \\ 
uvw2 & 55844.0152 & 15.66 $ \pm $ 0.16 & 16.58 &   4.85 $ \pm $  0.70 &    3.18e-11 $ \pm $    4.56e-12 \\ 
uvw2 & 55844.0164 & 15.56 $ \pm $ 0.06 & 17.47 &   5.35 $ \pm $  0.31 &    3.50e-11 $ \pm $    2.01e-12 \\ 
uvw2 & 55844.0819 & 15.78 $ \pm $ 0.17 & 16.59 &   4.36 $ \pm $  0.69 &    2.99e-11 $ \pm $    4.76e-12 \\ 
uvw2 & 55844.0830 & 15.61 $ \pm $ 0.07 & 17.48 &   5.08 $ \pm $  0.30 &    3.49e-11 $ \pm $    2.09e-12 \\ 
uvw2 & 55845.4193 & 15.93 $ \pm $ 0.19 & 16.64 &   3.79 $ \pm $  0.66 &    2.76e-11 $ \pm $    4.79e-12 \\ 
uvw2 & 55845.4204 & 15.66 $ \pm $ 0.07 & 17.51 &   4.85 $ \pm $  0.29 &    3.54e-11 $ \pm $    2.15e-12 \\ 
uvw2 & 55845.4858 & 16.64 $ \pm $ 0.30 & 16.84 &   1.97 $ \pm $  0.55 &    1.39e-11 $ \pm $    3.85e-12 \\ 
uvw2 & 55845.4867 & 15.72 $ \pm $ 0.07 & 17.48 &   4.59 $ \pm $  0.30 &    3.23e-11 $ \pm $    2.13e-12 \\ 
uvw2 & 55845.5527 & 15.74 $ \pm $ 0.20 & 16.41 &   4.53 $ \pm $  0.82 &    3.24e-11 $ \pm $    5.82e-12 \\ 
uvw2 & 55845.5535 & 15.74 $ \pm $ 0.08 & 17.43 &   4.51 $ \pm $  0.32 &    3.22e-11 $ \pm $    2.28e-12 \\ 
uvw2 & 55845.5705 & 15.54 $ \pm $ 0.09 & 17.11 &   5.46 $ \pm $  0.43 &    3.73e-11 $ \pm $    2.91e-12 \\ 
uvw2 & 55845.6198 & 15.74 $ \pm $ 0.09 & 17.29 &   4.53 $ \pm $  0.36 &    3.08e-11 $ \pm $    2.46e-12 \\ 
uvw2 & 55845.6369 & 15.64 $ \pm $ 0.07 & 17.44 &   4.94 $ \pm $  0.32 &    3.37e-11 $ \pm $    2.15e-12 \\ 
uvw2 & 55845.6871 & 15.64 $ \pm $ 0.08 & 17.30 &   4.96 $ \pm $  0.36 &    3.38e-11 $ \pm $    2.45e-12 \\ 
uvw2 & 55845.7042 & 15.61 $ \pm $ 0.07 & 17.43 &   5.10 $ \pm $  0.32 &    3.47e-11 $ \pm $    2.17e-12 \\ 
uvw2 & 55845.7537 & 15.73 $ \pm $ 0.08 & 17.34 &   4.55 $ \pm $  0.35 &    3.09e-11 $ \pm $    2.35e-12 \\ 
uvw2 & 55845.7709 & 15.70 $ \pm $ 0.07 & 17.47 &   4.72 $ \pm $  0.31 &    3.21e-11 $ \pm $    2.09e-12 \\ 
uvw2 & 55845.8878 & 15.84 $ \pm $ 0.09 & 17.40 &   4.11 $ \pm $  0.33 &    2.79e-11 $ \pm $    2.22e-12 \\ 
uvw2 & 55845.9042 & 15.68 $ \pm $ 0.07 & 17.45 &   4.78 $ \pm $  0.31 &    3.24e-11 $ \pm $    2.13e-12 \\ 
uvw2 & 55846.6974 & 15.68 $ \pm $ 0.15 & 16.62 &   4.77 $ \pm $  0.67 &    3.13e-11 $ \pm $    4.42e-12 \\ 
uvw2 & 55846.6986 & 15.69 $ \pm $ 0.07 & 17.56 &   4.76 $ \pm $  0.28 &    3.12e-11 $ \pm $    1.86e-12 \\ 
uvw2 & 55847.4335 & 15.98 $ \pm $ 0.19 & 16.70 &   3.64 $ \pm $  0.62 &    2.64e-11 $ \pm $    4.53e-12 \\ 
uvw2 & 55847.4348 & 15.86 $ \pm $ 0.07 & 17.67 &   4.05 $ \pm $  0.25 &    2.95e-11 $ \pm $    1.85e-12 \\ 
uvw2 & 55848.0413 & 16.00 $ \pm $ 0.06 & 18.00 &   3.56 $ \pm $  0.19 &    2.52e-11 $ \pm $    1.34e-12 \\ 
uvw2 & 55849.5087 & 15.83 $ \pm $ 0.05 & 17.89 &   4.16 $ \pm $  0.21 &    2.94e-11 $ \pm $    1.47e-12 \\ 
uvw2 & 55850.7165 & 15.86 $ \pm $ 0.06 & 17.88 &   4.05 $ \pm $  0.21 &    2.89e-11 $ \pm $    1.50e-12 \\ 
uvw2 & 55851.7289 & 15.98 $ \pm $ 0.07 & 17.74 &   3.63 $ \pm $  0.24 &    2.59e-11 $ \pm $    1.71e-12 \\ 
uvw2 & 55852.3205 & 15.98 $ \pm $ 0.06 & 17.97 &   3.62 $ \pm $  0.19 &    2.60e-11 $ \pm $    1.39e-12 \\ 
uvw2 & 55853.7159 & 16.02 $ \pm $ 0.06 & 17.99 &   3.50 $ \pm $  0.19 &    2.50e-11 $ \pm $    1.36e-12 \\ 
uvw2 & 55854.7929 & 16.08 $ \pm $ 0.09 & 17.59 &   3.31 $ \pm $  0.28 &    2.44e-11 $ \pm $    2.04e-12 \\ 
uvw2 & 55855.5853 & 16.10 $ \pm $ 0.07 & 17.95 &   3.26 $ \pm $  0.20 &    2.32e-11 $ \pm $    1.41e-12 \\ 
uvw2 & 55855.6554 & 16.14 $ \pm $ 0.07 & 17.97 &   3.14 $ \pm $  0.19 &    2.24e-11 $ \pm $    1.38e-12 \\ 
uvw2 & 55856.3880 & 16.14 $ \pm $ 0.07 & 17.96 &   3.12 $ \pm $  0.20 &    2.22e-11 $ \pm $    1.39e-12 \\ 
uvw2 & 55856.4548 & 16.12 $ \pm $ 0.07 & 17.93 &   3.18 $ \pm $  0.20 &    2.27e-11 $ \pm $    1.42e-12 \\ 
uvw2 & 55857.4583 & 16.12 $ \pm $ 0.06 & 17.99 &   3.20 $ \pm $  0.19 &    2.30e-11 $ \pm $    1.36e-12 \\ 
uvw2 & 55857.5214 & 16.07 $ \pm $ 0.08 & 17.67 &   3.33 $ \pm $  0.26 &    2.35e-11 $ \pm $    1.80e-12 \\ 
uvw2 & 55858.5243 & 16.16 $ \pm $ 0.09 & 17.72 &   3.07 $ \pm $  0.24 &    2.19e-11 $ \pm $    1.75e-12 \\ 
uvw2 & 55859.5326 & 16.20 $ \pm $ 0.07 & 17.97 &   2.95 $ \pm $  0.19 &    2.08e-11 $ \pm $    1.37e-12 \\ 
uvw2 & 55860.0053 & 16.24 $ \pm $ 0.07 & 17.97 &   2.87 $ \pm $  0.19 &    2.02e-11 $ \pm $    1.36e-12 \\ 
uvw2 & 55860.0631 & 16.27 $ \pm $ 0.09 & 17.84 &   2.77 $ \pm $  0.22 &    1.93e-11 $ \pm $    1.52e-12 \\ 
uvw2 & 55861.1362 & 16.53 $ \pm $ 0.07 & 18.25 &   2.19 $ \pm $  0.15 &    1.53e-11 $ \pm $    1.04e-12 \\ 
uvw2 & 55862.2726 & 16.25 $ \pm $ 0.07 & 18.11 &   2.84 $ \pm $  0.17 &    1.99e-11 $ \pm $    1.20e-12 \\ 
uvw2 & 55863.0083 & 16.28 $ \pm $ 0.07 & 18.12 &   2.75 $ \pm $  0.17 &    1.96e-11 $ \pm $    1.20e-12 \\ 
uvw2 & 55864.8822 & 16.29 $ \pm $ 0.07 & 18.13 &   2.74 $ \pm $  0.17 &    1.94e-11 $ \pm $    1.18e-12 \\ 
uvw2 & 55865.2155 & 16.41 $ \pm $ 0.07 & 18.19 &   2.44 $ \pm $  0.16 &    1.70e-11 $ \pm $    1.09e-12 \\ 
uvw2 & 55866.8880 & 16.42 $ \pm $ 0.07 & 18.18 &   2.41 $ \pm $  0.16 &    1.71e-11 $ \pm $    1.13e-12 \\ 
uvw2 & 55867.3576 & 16.47 $ \pm $ 0.09 & 17.98 &   2.31 $ \pm $  0.19 &    1.58e-11 $ \pm $    1.31e-12 \\ 
uvw2 & 55867.9593 & 16.45 $ \pm $ 0.08 & 18.13 &   2.36 $ \pm $  0.17 &    1.64e-11 $ \pm $    1.16e-12 \\ 
uvw2 & 55868.0924 & 16.52 $ \pm $ 0.07 & 18.26 &   2.22 $ \pm $  0.15 &    1.53e-11 $ \pm $    1.02e-12 \\ 
uvw2 & 55868.4893 & 16.50 $ \pm $ 0.10 & 17.94 &   2.25 $ \pm $  0.20 &    1.56e-11 $ \pm $    1.38e-12 \\ 
uvw2 & 55869.1622 & 16.55 $ \pm $ 0.08 & 18.25 &   2.15 $ \pm $  0.15 &    1.49e-11 $ \pm $    1.04e-12 \\ 
uvw2 & 55873.1143 & 16.66 $ \pm $ 0.08 & 18.28 &   1.94 $ \pm $  0.14 &    1.32e-11 $ \pm $    9.92e-13 \\ 
uvw2 & 55875.7226 & 16.52 $ \pm $ 0.10 & 17.97 &   2.21 $ \pm $  0.19 &    1.43e-11 $ \pm $    1.25e-12 \\ 
uvw2 & 55877.9381 & 16.69 $ \pm $ 0.08 & 18.30 &   1.89 $ \pm $  0.14 &    1.30e-11 $ \pm $    9.87e-13 \\ 
uvw2 & 55879.2057 & 16.90 $ \pm $ 0.09 & 18.38 &   1.56 $ \pm $  0.13 &    1.04e-11 $ \pm $    8.77e-13 \\ 
uvw2 & 55881.9527 & 16.99 $ \pm $ 0.10 & 18.42 &   1.43 $ \pm $  0.13 &    9.53e-12 $ \pm $    8.54e-13 \\ 
uvw2 & 55885.8991 & 16.96 $ \pm $ 0.10 & 18.42 &   1.47 $ \pm $  0.13 &    9.85e-12 $ \pm $    8.59e-13 \\ 
uvw2 & 55887.3067 & 17.03 $ \pm $ 0.10 & 18.42 &   1.38 $ \pm $  0.13 &    9.19e-12 $ \pm $    8.50e-13 \\ 
uvw2 & 55889.7816 & 17.19 $ \pm $ 0.11 & 18.49 &   1.19 $ \pm $  0.12 &    8.07e-12 $ \pm $    8.13e-13 \\ 
uvw2 & 55891.8400 & 17.14 $ \pm $ 0.10 & 18.49 &   1.24 $ \pm $  0.12 &    8.29e-12 $ \pm $    8.01e-13 \\ 
uvw2 & 55893.9122 & 17.18 $ \pm $ 0.11 & 18.50 &   1.20 $ \pm $  0.12 &    7.61e-12 $ \pm $    7.53e-13 \\ 
uvw2 & 55895.9169 & 17.22 $ \pm $ 0.11 & 18.50 &   1.16 $ \pm $  0.12 &    7.33e-12 $ \pm $    7.52e-13 \\ 
uvw2 & 55897.4626 & 17.29 $ \pm $ 0.14 & 18.34 &   1.09 $ \pm $  0.14 &    7.38e-12 $ \pm $    9.32e-13 \\ 
uvw2 & 55899.6630 & 17.51 $ \pm $ 0.14 & 18.58 &   0.89 $ \pm $  0.11 &    5.64e-12 $ \pm $    7.07e-13 \\ 
uvw2 & 55901.5371 & 17.56 $ \pm $ 0.14 & 18.61 &   0.85 $ \pm $  0.11 &    5.02e-12 $ \pm $    6.41e-13 \\ 
uvw2 & 55903.7360 & 17.50 $ \pm $ 0.13 & 18.59 &   0.90 $ \pm $  0.11 &    5.04e-12 $ \pm $    6.13e-13 \\ 
uvw2 & 55905.0725 & 17.73 $ \pm $ 0.15 & 18.66 &   0.73 $ \pm $  0.10 &    4.55e-12 $ \pm $    6.46e-13 \\ 
uvw2 & 55909.9525 & 17.67 $ \pm $ 0.15 & 18.64 &   0.77 $ \pm $  0.10 &    4.84e-12 $ \pm $    6.62e-13 \\ 
uvw2 & 55913.8960 & 17.89 $ \pm $ 0.18 & 18.67 &   0.62 $ \pm $  0.10 &    3.97e-12 $ \pm $    6.49e-13 \\ 
uvm2 & 55797.9407 &  \nodata & 18.70 &   0.03 $ \pm $  0.05 &    2.07e-13 $ \pm $    3.91e-13 \\ 
uvm2 & 55798.0082 &  \nodata  & 18.72 &   0.01 $ \pm $  0.05 &    5.90e-14 $ \pm $    3.69e-13 \\ 
uvm2 & 55799.0079 &  \nodata  & 18.42 &   0.17 $ \pm $  0.06 &    1.34e-12 $ \pm $    4.92e-13 \\ 
uvm2 & 55799.1391 & 18.69 $ \pm $ 0.36 & 18.70 &   0.18 $ \pm $  0.06 &    1.44e-12 $ \pm $    4.78e-13 \\ 
uvm2 & 55799.2167 &  \nodata  & 18.73 &   0.16 $ \pm $  0.06 &    1.28e-12 $ \pm $    4.60e-13 \\ 
uvm2 & 55799.4050 & 18.21 $ \pm $ 0.31 & 18.38 &   0.29 $ \pm $  0.08 &    2.27e-12 $ \pm $    6.52e-13 \\ 
uvm2 & 55799.5472 & 18.60 $ \pm $ 0.33 & 18.71 &   0.20 $ \pm $  0.06 &    1.55e-12 $ \pm $    4.68e-13 \\ 
uvm2 & 55800.0754 & 18.02 $ \pm $ 0.21 & 18.58 &   0.34 $ \pm $  0.07 &    2.67e-12 $ \pm $    5.31e-13 \\ 
uvm2 & 55800.2102 & 17.98 $ \pm $ 0.23 & 18.46 &   0.35 $ \pm $  0.07 &    2.76e-12 $ \pm $    5.87e-13 \\ 
uvm2 & 55800.3460 & 17.98 $ \pm $ 0.22 & 18.51 &   0.35 $ \pm $  0.07 &    2.75e-12 $ \pm $    5.59e-13 \\ 
uvm2 & 55800.6230 & 17.79 $ \pm $ 0.18 & 18.52 &   0.42 $ \pm $  0.07 &    3.23e-12 $ \pm $    5.47e-13 \\ 
uvm2 & 55800.7431 & 17.61 $ \pm $ 0.17 & 18.44 &   0.50 $ \pm $  0.08 &    3.84e-12 $ \pm $    5.95e-13 \\ 
uvm2 & 55800.8124 & 17.59 $ \pm $ 0.18 & 18.33 &   0.50 $ \pm $  0.09 &    3.89e-12 $ \pm $    6.65e-13 \\ 
uvm2 & 55800.9385 & 17.57 $ \pm $ 0.19 & 18.24 &   0.52 $ \pm $  0.09 &    3.95e-12 $ \pm $    7.03e-13 \\ 
uvm2 & 55801.0114 & 17.43 $ \pm $ 0.20 & 18.09 &   0.59 $ \pm $  0.11 &    4.53e-12 $ \pm $    8.16e-13 \\ 
uvm2 & 55801.1446 & 17.47 $ \pm $ 0.16 & 18.34 &   0.56 $ \pm $  0.09 &    4.32e-12 $ \pm $    6.50e-13 \\ 
uvm2 & 55801.2261 & 17.25 $ \pm $ 0.14 & 18.28 &   0.69 $ \pm $  0.09 &    5.36e-12 $ \pm $    6.97e-13 \\ 
uvm2 & 55801.2687 & 17.54 $ \pm $ 0.23 & 18.05 &   0.53 $ \pm $  0.11 &    4.05e-12 $ \pm $    8.39e-13 \\ 
uvm2 & 55801.4020 & 17.17 $ \pm $ 0.18 & 17.92 &   0.74 $ \pm $  0.12 &    5.72e-12 $ \pm $    9.57e-13 \\ 
uvm2 & 55801.4935 & 17.34 $ \pm $ 0.15 & 18.32 &   0.64 $ \pm $  0.09 &    4.86e-12 $ \pm $    6.57e-13 \\ 
uvm2 & 55801.5455 & 17.31 $ \pm $ 0.17 & 18.11 &   0.66 $ \pm $  0.10 &    5.02e-12 $ \pm $    7.96e-13 \\ 
uvm2 & 55801.6694 & 17.07 $ \pm $ 0.17 & 17.88 &   0.82 $ \pm $  0.13 &    6.29e-12 $ \pm $    1.00e-12 \\ 
uvm2 & 55801.8036 & 16.94 $ \pm $ 0.17 & 17.75 &   0.92 $ \pm $  0.15 &    7.09e-12 $ \pm $    1.13e-12 \\ 
uvm2 & 55801.9369 & 16.72 $ \pm $ 0.15 & 17.68 &   1.12 $ \pm $  0.15 &    8.74e-12 $ \pm $    1.21e-12 \\ 
uvm2 & 55802.0091 & 17.04 $ \pm $ 0.17 & 17.83 &   0.84 $ \pm $  0.14 &    6.45e-12 $ \pm $    1.03e-12 \\ 
uvm2 & 55802.1611 & 16.63 $ \pm $ 0.10 & 18.05 &   1.23 $ \pm $  0.11 &    9.57e-12 $ \pm $    8.56e-13 \\ 
uvm2 & 55802.2251 & 16.77 $ \pm $ 0.09 & 18.25 &   1.08 $ \pm $  0.09 &    8.33e-12 $ \pm $    7.12e-13 \\ 
uvm2 & 55804.2998 & 15.17 $ \pm $ 0.05 & 17.25 &   4.70 $ \pm $  0.23 &    3.84e-11 $ \pm $    1.88e-12 \\ 
uvm2 & 55805.3697 & 14.59 $ \pm $ 0.04 & 16.91 &   8.05 $ \pm $  0.32 &    6.67e-11 $ \pm $    2.62e-12 \\ 
uvm2 & 55805.4235 & 14.53 $ \pm $ 0.04 & 16.89 &   8.46 $ \pm $  0.32 &    7.02e-11 $ \pm $    2.67e-12 \\ 
uvm2 & 55806.3656 & 14.09 $ \pm $ 0.04 & 16.51 &  12.71 $ \pm $  0.46 &    1.06e-10 $ \pm $    3.82e-12 \\ 
uvm2 & 55806.7601 & 13.96 $ \pm $ 0.04 & 16.34 &  14.28 $ \pm $  0.53 &    1.19e-10 $ \pm $    4.44e-12 \\ 
uvm2 & 55807.0864 & 13.93 $ \pm $ 0.05 & 16.10 &  14.67 $ \pm $  0.67 &    1.22e-10 $ \pm $    5.55e-12 \\ 
uvm2 & 55807.1526 & 13.82 $ \pm $ 0.05 & 16.00 &  16.25 $ \pm $  0.73 &    1.36e-10 $ \pm $    6.12e-12 \\ 
uvm2 & 55807.2865 & 13.84 $ \pm $ 0.05 & 16.04 &  16.06 $ \pm $  0.71 &    1.34e-10 $ \pm $    5.90e-12 \\ 
uvm2 & 55807.4205 & 13.78 $ \pm $ 0.05 & 15.99 &  16.95 $ \pm $  0.73 &    1.42e-10 $ \pm $    6.15e-12 \\ 
uvm2 & 55807.6949 & 13.70 $ \pm $ 0.09 & 15.19 &  18.16 $ \pm $  1.54 &    1.52e-10 $ \pm $    1.29e-11 \\ 
uvm2 & 55807.6957 & 13.76 $ \pm $ 0.05 & 15.99 &  17.26 $ \pm $  0.73 &    1.44e-10 $ \pm $    6.13e-12 \\ 
uvm2 & 55807.8277 & 13.64 $ \pm $ 0.04 & 16.10 &  19.20 $ \pm $  0.67 &    1.61e-10 $ \pm $    5.59e-12 \\ 
uvm2 & 55808.0237 & 13.56 $ \pm $ 0.05 & 15.79 &  20.60 $ \pm $  0.88 &    1.73e-10 $ \pm $    7.38e-12 \\ 
uvm2 & 55808.0897 & 13.56 $ \pm $ 0.05 & 15.79 &  20.70 $ \pm $  0.89 &    1.73e-10 $ \pm $    7.43e-12 \\ 
uvm2 & 55808.2228 & 13.57 $ \pm $ 0.05 & 15.82 &  20.50 $ \pm $  0.86 &    1.72e-10 $ \pm $    7.24e-12 \\ 
uvm2 & 55808.7609 & 13.38 $ \pm $ 0.08 & 15.02 &  24.38 $ \pm $  1.80 &    2.05e-10 $ \pm $    1.51e-11 \\ 
uvm2 & 55808.7617 & 13.43 $ \pm $ 0.04 & 15.73 &  23.30 $ \pm $  0.93 &    1.95e-10 $ \pm $    7.80e-12 \\ 
uvm2 & 55808.7718 & 13.48 $ \pm $ 0.04 & 15.92 &  22.28 $ \pm $  0.78 &    1.87e-10 $ \pm $    6.55e-12 \\ 
uvm2 & 55808.9030 & 13.41 $ \pm $ 0.04 & 15.82 &  23.65 $ \pm $  0.86 &    1.98e-10 $ \pm $    7.24e-12 \\ 
uvm2 & 55809.3682 & 13.43 $ \pm $ 0.04 & 15.91 &  23.31 $ \pm $  0.79 &    1.95e-10 $ \pm $    6.60e-12 \\ 
uvm2 & 55809.6429 & 13.33 $ \pm $ 0.04 & 15.78 &  25.69 $ \pm $  0.89 &    2.15e-10 $ \pm $    7.45e-12 \\ 
uvm2 & 55809.7624 & 13.27 $ \pm $ 0.08 & 14.95 &  27.09 $ \pm $  1.92 &    2.27e-10 $ \pm $    1.61e-11 \\ 
uvm2 & 55809.7632 & 13.26 $ \pm $ 0.04 & 15.59 &  27.31 $ \pm $  1.06 &    2.29e-10 $ \pm $    8.94e-12 \\ 
uvm2 & 55810.1145 & 13.26 $ \pm $ 0.04 & 15.74 &  27.21 $ \pm $  0.93 &    2.28e-10 $ \pm $    7.76e-12 \\ 
uvm2 & 55810.3032 & 13.24 $ \pm $ 0.04 & 15.73 &  27.69 $ \pm $  0.94 &    2.32e-10 $ \pm $    7.86e-12 \\ 
uvm2 & 55811.0366 & 13.08 $ \pm $ 0.06 & 14.98 &  32.22 $ \pm $  1.86 &    2.71e-10 $ \pm $    1.57e-11 \\ 
uvm2 & 55811.0377 & 13.18 $ \pm $ 0.04 & 15.57 &  29.40 $ \pm $  1.08 &    2.47e-10 $ \pm $    9.11e-12 \\ 
uvm2 & 55811.6389 & 13.14 $ \pm $ 0.07 & 14.99 &  30.38 $ \pm $  1.85 &    2.55e-10 $ \pm $    1.56e-11 \\ 
uvm2 & 55811.6399 & 13.17 $ \pm $ 0.04 & 15.55 &  29.71 $ \pm $  1.11 &    2.50e-10 $ \pm $    9.29e-12 \\ 
uvm2 & 55812.3767 & 13.03 $ \pm $ 0.06 & 15.00 &  33.68 $ \pm $  1.83 &    2.84e-10 $ \pm $    1.54e-11 \\ 
uvm2 & 55812.3779 & 13.09 $ \pm $ 0.04 & 15.51 &  31.92 $ \pm $  1.15 &    2.69e-10 $ \pm $    9.68e-12 \\ 
uvm2 & 55812.5768 & 13.10 $ \pm $ 0.04 & 15.47 &  31.70 $ \pm $  1.19 &    2.67e-10 $ \pm $    9.99e-12 \\ 
uvm2 & 55813.1202 & 13.08 $ \pm $ 0.06 & 15.01 &  32.26 $ \pm $  1.82 &    2.72e-10 $ \pm $    1.54e-11 \\ 
uvm2 & 55813.1214 & 13.07 $ \pm $ 0.04 & 15.48 &  32.46 $ \pm $  1.18 &    2.73e-10 $ \pm $    9.89e-12 \\ 
uvm2 & 55814.2580 & 13.03 $ \pm $ 0.06 & 15.00 &  33.62 $ \pm $  1.83 &    2.85e-10 $ \pm $    1.55e-11 \\ 
uvm2 & 55814.2592 & 13.03 $ \pm $ 0.04 & 15.45 &  33.82 $ \pm $  1.21 &    2.87e-10 $ \pm $    1.03e-11 \\ 
uvm2 & 55814.3768 & 13.03 $ \pm $ 0.04 & 15.31 &  33.88 $ \pm $  1.38 &    2.87e-10 $ \pm $    1.17e-11 \\ 
uvm2 & 55814.7782 & 13.07 $ \pm $ 0.04 & 15.34 &  32.48 $ \pm $  1.34 &    2.75e-10 $ \pm $    1.13e-11 \\ 
uvm2 & 55814.8448 & 13.03 $ \pm $ 0.04 & 15.31 &  33.79 $ \pm $  1.37 &    2.87e-10 $ \pm $    1.16e-11 \\ 
uvm2 & 55814.9212 & 13.07 $ \pm $ 0.05 & 15.16 &  32.59 $ \pm $  1.57 &    2.76e-10 $ \pm $    1.33e-11 \\ 
uvm2 & 55814.9229 & 13.05 $ \pm $ 0.04 & 15.50 &  33.16 $ \pm $  1.16 &    2.81e-10 $ \pm $    9.83e-12 \\ 
uvm2 & 55815.2586 & 13.13 $ \pm $ 0.05 & 15.20 &  30.61 $ \pm $  1.52 &    2.60e-10 $ \pm $    1.29e-11 \\ 
uvm2 & 55815.2604 & 13.06 $ \pm $ 0.04 & 15.52 &  32.67 $ \pm $  1.14 &    2.78e-10 $ \pm $    9.71e-12 \\ 
uvm2 & 55815.3963 & 13.05 $ \pm $ 0.06 & 15.03 &  33.24 $ \pm $  1.78 &    2.83e-10 $ \pm $    1.52e-11 \\ 
uvm2 & 55815.3976 & 13.10 $ \pm $ 0.04 & 15.52 &  31.49 $ \pm $  1.14 &    2.68e-10 $ \pm $    9.69e-12 \\ 
uvm2 & 55816.3307 & 13.12 $ \pm $ 0.05 & 15.18 &  30.94 $ \pm $  1.55 &    2.64e-10 $ \pm $    1.33e-11 \\ 
uvm2 & 55816.3323 & 13.09 $ \pm $ 0.04 & 15.53 &  31.87 $ \pm $  1.12 &    2.72e-10 $ \pm $    9.58e-12 \\ 
uvm2 & 55817.7987 & 13.20 $ \pm $ 0.04 & 15.66 &  28.86 $ \pm $  0.99 &    2.46e-10 $ \pm $    8.49e-12 \\ 
uvm2 & 55817.8692 & 13.20 $ \pm $ 0.04 & 15.68 &  28.91 $ \pm $  0.98 &    2.47e-10 $ \pm $    8.37e-12 \\ 
uvm2 & 55818.4102 & 13.26 $ \pm $ 0.04 & 15.75 &  27.28 $ \pm $  0.92 &    2.33e-10 $ \pm $    7.86e-12 \\ 
uvm2 & 55819.0688 & 13.26 $ \pm $ 0.06 & 15.22 &  27.38 $ \pm $  1.50 &    2.34e-10 $ \pm $    1.28e-11 \\ 
uvm2 & 55819.0703 & 13.35 $ \pm $ 0.04 & 15.75 &  25.24 $ \pm $  0.92 &    2.15e-10 $ \pm $    7.82e-12 \\ 
uvm2 & 55820.8774 & 13.61 $ \pm $ 0.08 & 15.28 &  19.81 $ \pm $  1.42 &    1.68e-10 $ \pm $    1.21e-11 \\ 
uvm2 & 55820.8785 & 13.57 $ \pm $ 0.04 & 15.89 &  20.56 $ \pm $  0.80 &    1.75e-10 $ \pm $    6.83e-12 \\ 
uvm2 & 55820.9464 & 13.59 $ \pm $ 0.04 & 15.97 &  20.22 $ \pm $  0.75 &    1.72e-10 $ \pm $    6.40e-12 \\ 
uvm2 & 55822.2161 & 13.69 $ \pm $ 0.09 & 15.25 &  18.30 $ \pm $  1.45 &    1.56e-10 $ \pm $    1.23e-11 \\ 
uvm2 & 55822.2170 & 13.79 $ \pm $ 0.04 & 16.05 &  16.77 $ \pm $  0.70 &    1.42e-10 $ \pm $    5.92e-12 \\ 
uvm2 & 55823.0198 & 13.88 $ \pm $ 0.09 & 15.39 &  15.36 $ \pm $  1.27 &    1.30e-10 $ \pm $    1.08e-11 \\ 
uvm2 & 55823.0208 & 13.88 $ \pm $ 0.04 & 16.14 &  15.37 $ \pm $  0.64 &    1.30e-10 $ \pm $    5.43e-12 \\ 
uvm2 & 55823.0867 & 14.02 $ \pm $ 0.10 & 15.37 &  13.59 $ \pm $  1.30 &    1.15e-10 $ \pm $    1.10e-11 \\ 
uvm2 & 55823.0876 & 13.89 $ \pm $ 0.05 & 16.10 &  15.33 $ \pm $  0.67 &    1.30e-10 $ \pm $    5.64e-12 \\ 
uvm2 & 55824.4253 & 14.09 $ \pm $ 0.11 & 15.37 &  12.76 $ \pm $  1.30 &    1.07e-10 $ \pm $    1.10e-11 \\ 
uvm2 & 55824.4262 & 14.03 $ \pm $ 0.05 & 16.19 &  13.48 $ \pm $  0.61 &    1.14e-10 $ \pm $    5.15e-12 \\ 
uvm2 & 55826.9093 & 14.41 $ \pm $ 0.11 & 15.69 &   9.47 $ \pm $  0.97 &    7.91e-11 $ \pm $    8.09e-12 \\ 
uvm2 & 55826.9103 & 14.36 $ \pm $ 0.05 & 16.51 &   9.89 $ \pm $  0.46 &    8.27e-11 $ \pm $    3.82e-12 \\ 
uvm2 & 55826.9728 & 14.45 $ \pm $ 0.13 & 15.59 &   9.13 $ \pm $  1.06 &    7.60e-11 $ \pm $    8.86e-12 \\ 
uvm2 & 55826.9737 & 14.41 $ \pm $ 0.05 & 16.49 &   9.47 $ \pm $  0.46 &    7.89e-11 $ \pm $    3.87e-12 \\ 
uvm2 & 55827.0402 & 14.16 $ \pm $ 0.11 & 15.41 &  11.92 $ \pm $  1.25 &    1.00e-10 $ \pm $    1.05e-11 \\ 
uvm2 & 55827.0410 & 14.41 $ \pm $ 0.06 & 16.47 &   9.44 $ \pm $  0.47 &    7.87e-11 $ \pm $    3.95e-12 \\ 
uvm2 & 55828.1731 & 14.48 $ \pm $ 0.11 & 15.74 &   8.86 $ \pm $  0.93 &    7.39e-11 $ \pm $    7.74e-12 \\ 
uvm2 & 55828.1742 & 14.51 $ \pm $ 0.05 & 16.61 &   8.64 $ \pm $  0.41 &    7.20e-11 $ \pm $    3.46e-12 \\ 
uvm2 & 55829.4458 & 14.79 $ \pm $ 0.12 & 15.95 &   6.64 $ \pm $  0.76 &    5.50e-11 $ \pm $    6.31e-12 \\ 
uvm2 & 55829.4470 & 14.60 $ \pm $ 0.05 & 16.71 &   7.95 $ \pm $  0.38 &    6.63e-11 $ \pm $    3.15e-12 \\ 
uvm2 & 55829.5146 & 14.71 $ \pm $ 0.14 & 15.73 &   7.20 $ \pm $  0.94 &    5.97e-11 $ \pm $    7.78e-12 \\ 
uvm2 & 55829.5154 & 14.77 $ \pm $ 0.06 & 16.72 &   6.78 $ \pm $  0.38 &    5.61e-11 $ \pm $    3.10e-12 \\ 
uvm2 & 55829.8431 & 14.90 $ \pm $ 0.16 & 15.76 &   6.04 $ \pm $  0.91 &    4.98e-11 $ \pm $    7.50e-12 \\ 
uvm2 & 55829.8439 & 14.77 $ \pm $ 0.06 & 16.70 &   6.79 $ \pm $  0.38 &    5.63e-11 $ \pm $    3.19e-12 \\ 
uvm2 & 55830.0419 & 14.81 $ \pm $ 0.07 & 16.64 &   6.54 $ \pm $  0.40 &    5.43e-11 $ \pm $    3.35e-12 \\ 
uvm2 & 55830.3778 & 14.78 $ \pm $ 0.06 & 16.75 &   6.72 $ \pm $  0.37 &    5.58e-11 $ \pm $    3.04e-12 \\ 
uvm2 & 55830.5146 & 14.91 $ \pm $ 0.06 & 16.86 &   5.99 $ \pm $  0.33 &    4.95e-11 $ \pm $    2.72e-12 \\ 
uvm2 & 55831.7954 & 14.91 $ \pm $ 0.14 & 15.98 &   5.96 $ \pm $  0.74 &    4.96e-11 $ \pm $    6.16e-12 \\ 
uvm2 & 55831.7966 & 15.05 $ \pm $ 0.06 & 17.00 &   5.27 $ \pm $  0.29 &    4.36e-11 $ \pm $    2.41e-12 \\ 
uvm2 & 55831.9178 & 15.36 $ \pm $ 0.18 & 16.10 &   3.94 $ \pm $  0.66 &    3.22e-11 $ \pm $    5.42e-12 \\ 
uvm2 & 55831.9189 & 15.02 $ \pm $ 0.06 & 16.94 &   5.39 $ \pm $  0.31 &    4.47e-11 $ \pm $    2.54e-12 \\ 
uvm2 & 55832.9874 & 15.06 $ \pm $ 0.16 & 15.93 &   5.22 $ \pm $  0.78 &    4.33e-11 $ \pm $    6.47e-12 \\ 
uvm2 & 55832.9883 & 15.14 $ \pm $ 0.07 & 16.99 &   4.81 $ \pm $  0.29 &    3.98e-11 $ \pm $    2.42e-12 \\ 
uvm2 & 55833.4602 & 15.10 $ \pm $ 0.12 & 16.30 &   5.01 $ \pm $  0.55 &    4.16e-11 $ \pm $    4.60e-12 \\ 
uvm2 & 55833.4619 & 15.12 $ \pm $ 0.06 & 17.17 &   4.92 $ \pm $  0.25 &    4.08e-11 $ \pm $    2.07e-12 \\ 
uvm2 & 55833.5276 & 15.09 $ \pm $ 0.17 & 15.94 &   5.04 $ \pm $  0.77 &    4.19e-11 $ \pm $    6.40e-12 \\ 
uvm2 & 55833.5285 & 15.18 $ \pm $ 0.07 & 17.01 &   4.66 $ \pm $  0.29 &    3.86e-11 $ \pm $    2.39e-12 \\ 
uvm2 & 55835.3965 & 15.47 $ \pm $ 0.15 & 16.43 &   3.57 $ \pm $  0.49 &    2.94e-11 $ \pm $    4.07e-12 \\ 
uvm2 & 55835.3981 & 15.27 $ \pm $ 0.06 & 17.23 &   4.28 $ \pm $  0.23 &    3.56e-11 $ \pm $    1.95e-12 \\ 
uvm2 & 55835.4644 & 15.57 $ \pm $ 0.19 & 16.27 &   3.25 $ \pm $  0.57 &    2.67e-11 $ \pm $    4.67e-12 \\ 
uvm2 & 55835.4655 & 15.39 $ \pm $ 0.07 & 17.20 &   3.82 $ \pm $  0.24 &    3.16e-11 $ \pm $    2.00e-12 \\ 
uvm2 & 55836.4685 & 15.19 $ \pm $ 0.14 & 16.20 &   4.62 $ \pm $  0.61 &    3.85e-11 $ \pm $    5.08e-12 \\ 
uvm2 & 55836.4698 & 15.46 $ \pm $ 0.07 & 17.28 &   3.61 $ \pm $  0.22 &    2.98e-11 $ \pm $    1.85e-12 \\ 
uvm2 & 55836.5372 & 15.51 $ \pm $ 0.18 & 16.24 &   3.43 $ \pm $  0.58 &    2.82e-11 $ \pm $    4.79e-12 \\ 
uvm2 & 55836.5383 & 15.60 $ \pm $ 0.07 & 17.31 &   3.17 $ \pm $  0.22 &    2.60e-11 $ \pm $    1.79e-12 \\ 
uvm2 & 55837.4015 & 15.71 $ \pm $ 0.19 & 16.40 &   2.85 $ \pm $  0.50 &    2.34e-11 $ \pm $    4.12e-12 \\ 
uvm2 & 55837.4027 & 15.58 $ \pm $ 0.07 & 17.33 &   3.23 $ \pm $  0.21 &    2.66e-11 $ \pm $    1.76e-12 \\ 
uvm2 & 55838.3408 & 15.48 $ \pm $ 0.15 & 16.47 &   3.53 $ \pm $  0.47 &    2.93e-11 $ \pm $    3.94e-12 \\ 
uvm2 & 55838.3424 & 15.53 $ \pm $ 0.06 & 17.40 &   3.38 $ \pm $  0.20 &    2.80e-11 $ \pm $    1.66e-12 \\ 
uvm2 & 55838.9430 & 15.81 $ \pm $ 0.22 & 16.37 &   2.60 $ \pm $  0.52 &    2.13e-11 $ \pm $    4.24e-12 \\ 
uvm2 & 55838.9441 & 15.69 $ \pm $ 0.08 & 17.36 &   2.91 $ \pm $  0.21 &    2.40e-11 $ \pm $    1.72e-12 \\ 
uvm2 & 55839.6137 & 15.87 $ \pm $ 0.22 & 16.43 &   2.46 $ \pm $  0.49 &    2.02e-11 $ \pm $    4.04e-12 \\ 
uvm2 & 55839.6149 & 15.64 $ \pm $ 0.07 & 17.35 &   3.04 $ \pm $  0.21 &    2.52e-11 $ \pm $    1.74e-12 \\ 
uvm2 & 55840.2146 & 15.76 $ \pm $ 0.18 & 16.51 &   2.74 $ \pm $  0.46 &    2.26e-11 $ \pm $    3.78e-12 \\ 
uvm2 & 55840.2160 & 15.76 $ \pm $ 0.07 & 17.49 &   2.72 $ \pm $  0.18 &    2.25e-11 $ \pm $    1.53e-12 \\ 
uvm2 & 55840.3522 & 15.77 $ \pm $ 0.26 & 16.14 &   2.70 $ \pm $  0.64 &    2.23e-11 $ \pm $    5.29e-12 \\ 
uvm2 & 55840.3531 & 15.81 $ \pm $ 0.09 & 17.28 &   2.60 $ \pm $  0.22 &    2.15e-11 $ \pm $    1.85e-12 \\ 
uvm2 & 55841.3469 & 15.77 $ \pm $ 0.20 & 16.41 &   2.69 $ \pm $  0.50 &    2.24e-11 $ \pm $    4.13e-12 \\ 
uvm2 & 55841.3482 & 15.80 $ \pm $ 0.08 & 17.45 &   2.62 $ \pm $  0.19 &    2.17e-11 $ \pm $    1.59e-12 \\ 
uvm2 & 55841.8889 & 16.08 $ \pm $ 0.25 & 16.48 &   2.04 $ \pm $  0.47 &    1.67e-11 $ \pm $    3.82e-12 \\ 
uvm2 & 55841.8900 & 15.77 $ \pm $ 0.08 & 17.38 &   2.70 $ \pm $  0.20 &    2.24e-11 $ \pm $    1.69e-12 \\ 
uvm2 & 55842.0099 & 15.42 $ \pm $ 0.21 & 16.00 &   3.74 $ \pm $  0.73 &    3.15e-11 $ \pm $    6.17e-12 \\ 
uvm2 & 55842.0107 & 15.77 $ \pm $ 0.09 & 17.23 &   2.72 $ \pm $  0.23 &    2.26e-11 $ \pm $    1.95e-12 \\ 
uvm2 & 55842.0773 & 15.79 $ \pm $ 0.10 & 17.19 &   2.66 $ \pm $  0.24 &    2.22e-11 $ \pm $    2.03e-12 \\ 
uvm2 & 55842.1428 & 15.85 $ \pm $ 0.08 & 17.47 &   2.52 $ \pm $  0.19 &    2.09e-11 $ \pm $    1.56e-12 \\ 
uvm2 & 55842.3541 & 15.49 $ \pm $ 0.18 & 16.23 &   3.48 $ \pm $  0.59 &    2.93e-11 $ \pm $    4.94e-12 \\ 
uvm2 & 55842.3553 & 15.88 $ \pm $ 0.09 & 17.44 &   2.45 $ \pm $  0.19 &    2.03e-11 $ \pm $    1.60e-12 \\ 
uvm2 & 55842.5477 & 15.89 $ \pm $ 0.08 & 17.48 &   2.42 $ \pm $  0.19 &    2.01e-11 $ \pm $    1.54e-12 \\ 
uvm2 & 55842.8930 & 15.82 $ \pm $ 0.22 & 16.38 &   2.58 $ \pm $  0.52 &    2.15e-11 $ \pm $    4.29e-12 \\ 
uvm2 & 55842.8941 & 15.76 $ \pm $ 0.08 & 17.38 &   2.74 $ \pm $  0.20 &    2.29e-11 $ \pm $    1.70e-12 \\ 
uvm2 & 55842.9455 & 15.88 $ \pm $ 0.12 & 17.05 &   2.44 $ \pm $  0.28 &    2.03e-11 $ \pm $    2.31e-12 \\ 
uvm2 & 55843.4875 & 15.87 $ \pm $ 0.23 & 16.39 &   2.46 $ \pm $  0.51 &    2.05e-11 $ \pm $    4.24e-12 \\ 
uvm2 & 55843.4886 & 15.93 $ \pm $ 0.09 & 17.46 &   2.33 $ \pm $  0.19 &    1.94e-11 $ \pm $    1.58e-12 \\ 
uvm2 & 55843.7516 & 16.18 $ \pm $ 0.28 & 16.46 &   1.86 $ \pm $  0.48 &    1.53e-11 $ \pm $    3.94e-12 \\ 
uvm2 & 55843.7526 & 15.82 $ \pm $ 0.09 & 17.38 &   2.57 $ \pm $  0.20 &    2.15e-11 $ \pm $    1.71e-12 \\ 
uvm2 & 55844.0205 & 16.15 $ \pm $ 0.26 & 16.52 &   1.91 $ \pm $  0.45 &    1.59e-11 $ \pm $    3.74e-12 \\ 
uvm2 & 55844.0216 & 15.94 $ \pm $ 0.09 & 17.49 &   2.31 $ \pm $  0.18 &    1.93e-11 $ \pm $    1.54e-12 \\ 
uvm2 & 55844.0869 & 15.86 $ \pm $ 0.23 & 16.37 &   2.50 $ \pm $  0.52 &    2.09e-11 $ \pm $    4.32e-12 \\ 
uvm2 & 55844.0880 & 16.01 $ \pm $ 0.09 & 17.49 &   2.17 $ \pm $  0.18 &    1.80e-11 $ \pm $    1.53e-12 \\ 
uvm2 & 55845.4243 & 15.69 $ \pm $ 0.21 & 16.29 &   2.91 $ \pm $  0.56 &    2.46e-11 $ \pm $    4.72e-12 \\ 
uvm2 & 55845.4254 & 15.96 $ \pm $ 0.10 & 17.38 &   2.28 $ \pm $  0.21 &    1.91e-11 $ \pm $    1.73e-12 \\ 
uvm2 & 55845.4903 & 15.90 $ \pm $ 0.25 & 16.29 &   2.40 $ \pm $  0.56 &    2.02e-11 $ \pm $    4.70e-12 \\ 
uvm2 & 55845.4912 & 15.88 $ \pm $ 0.09 & 17.36 &   2.45 $ \pm $  0.21 &    2.07e-11 $ \pm $    1.75e-12 \\ 
uvm2 & 55845.5546 & 15.84 $ \pm $ 0.27 & 16.17 &   2.54 $ \pm $  0.62 &    2.14e-11 $ \pm $    5.26e-12 \\ 
uvm2 & 55845.5554 & 16.10 $ \pm $ 0.11 & 17.38 &   2.00 $ \pm $  0.20 &    1.67e-11 $ \pm $    1.71e-12 \\ 
uvm2 & 55846.7029 & 16.42 $ \pm $ 0.28 & 16.70 &   1.48 $ \pm $  0.38 &    1.23e-11 $ \pm $    3.18e-12 \\ 
uvm2 & 55846.7041 & 16.03 $ \pm $ 0.09 & 17.55 &   2.13 $ \pm $  0.18 &    1.79e-11 $ \pm $    1.48e-12 \\ 
uvm2 & 55847.4392 & 15.85 $ \pm $ 0.21 & 16.45 &   2.52 $ \pm $  0.48 &    2.13e-11 $ \pm $    4.07e-12 \\ 
uvm2 & 55847.4404 & 16.11 $ \pm $ 0.09 & 17.59 &   1.97 $ \pm $  0.17 &    1.65e-11 $ \pm $    1.41e-12 \\ 
uvm2 & 55848.0489 & 16.02 $ \pm $ 0.06 & 17.92 &   2.15 $ \pm $  0.12 &    1.81e-11 $ \pm $    1.04e-12 \\ 
uvm2 & 55849.5163 & 16.13 $ \pm $ 0.07 & 17.98 &   1.94 $ \pm $  0.12 &    1.63e-11 $ \pm $    9.92e-13 \\ 
uvm2 & 55850.7234 & 16.15 $ \pm $ 0.07 & 17.97 &   1.91 $ \pm $  0.12 &    1.61e-11 $ \pm $    9.95e-13 \\ 
uvm2 & 55852.3279 & 16.19 $ \pm $ 0.07 & 18.01 &   1.83 $ \pm $  0.12 &    1.55e-11 $ \pm $    9.72e-13 \\ 
uvm2 & 55853.7232 & 16.35 $ \pm $ 0.07 & 18.08 &   1.58 $ \pm $  0.11 &    1.34e-11 $ \pm $    9.12e-13 \\ 
uvm2 & 55854.8600 & 16.10 $ \pm $ 0.14 & 17.15 &   2.00 $ \pm $  0.25 &    1.70e-11 $ \pm $    2.15e-12 \\ 
uvm2 & 55855.5903 & 16.40 $ \pm $ 0.08 & 18.02 &   1.51 $ \pm $  0.11 &    1.28e-11 $ \pm $    9.55e-13 \\ 
uvm2 & 55855.6605 & 16.37 $ \pm $ 0.08 & 18.02 &   1.56 $ \pm $  0.11 &    1.32e-11 $ \pm $    9.64e-13 \\ 
uvm2 & 55856.3927 & 16.42 $ \pm $ 0.08 & 18.02 &   1.49 $ \pm $  0.11 &    1.26e-11 $ \pm $    9.63e-13 \\ 
uvm2 & 55856.4593 & 16.44 $ \pm $ 0.09 & 18.02 &   1.45 $ \pm $  0.11 &    1.23e-11 $ \pm $    9.55e-13 \\ 
uvm2 & 55857.4638 & 16.36 $ \pm $ 0.08 & 18.03 &   1.56 $ \pm $  0.11 &    1.32e-11 $ \pm $    9.57e-13 \\ 
uvm2 & 55857.5234 & 16.55 $ \pm $ 0.12 & 17.77 &   1.31 $ \pm $  0.14 &    1.11e-11 $ \pm $    1.21e-12 \\ 
uvm2 & 55858.5262 & 16.45 $ \pm $ 0.11 & 17.72 &   1.44 $ \pm $  0.15 &    1.22e-11 $ \pm $    1.27e-12 \\ 
uvm2 & 55859.5371 & 16.55 $ \pm $ 0.09 & 18.07 &   1.32 $ \pm $  0.11 &    1.12e-11 $ \pm $    9.20e-13 \\ 
uvm2 & 55860.0095 & 16.55 $ \pm $ 0.09 & 18.05 &   1.31 $ \pm $  0.11 &    1.11e-11 $ \pm $    9.29e-13 \\ 
uvm2 & 55860.0659 & 16.62 $ \pm $ 0.11 & 17.96 &   1.24 $ \pm $  0.12 &    1.04e-11 $ \pm $    1.01e-12 \\ 
uvm2 & 55861.1430 & 16.75 $ \pm $ 0.09 & 18.21 &   1.10 $ \pm $  0.10 &    9.28e-12 $ \pm $    8.09e-13 \\ 
uvm2 & 55862.2796 & 16.67 $ \pm $ 0.09 & 18.20 &   1.18 $ \pm $  0.10 &    9.99e-12 $ \pm $    8.10e-13 \\ 
uvm2 & 55863.0151 & 16.60 $ \pm $ 0.09 & 18.16 &   1.26 $ \pm $  0.10 &    1.07e-11 $ \pm $    8.37e-13 \\ 
uvm2 & 55864.8893 & 16.68 $ \pm $ 0.09 & 18.20 &   1.17 $ \pm $  0.10 &    9.92e-12 $ \pm $    8.11e-13 \\ 
uvm2 & 55865.2223 & 16.80 $ \pm $ 0.10 & 18.22 &   1.05 $ \pm $  0.09 &    8.84e-12 $ \pm $    7.92e-13 \\ 
uvm2 & 55866.8946 & 16.68 $ \pm $ 0.09 & 18.17 &   1.16 $ \pm $  0.10 &    9.83e-12 $ \pm $    8.36e-13 \\ 
uvm2 & 55867.3608 & 16.91 $ \pm $ 0.12 & 18.06 &   0.95 $ \pm $  0.11 &    7.96e-12 $ \pm $    9.15e-13 \\ 
uvm2 & 55867.9646 & 16.80 $ \pm $ 0.10 & 18.18 &   1.04 $ \pm $  0.10 &    8.78e-12 $ \pm $    8.25e-13 \\ 
uvm2 & 55868.1001 & 16.89 $ \pm $ 0.10 & 18.27 &   0.96 $ \pm $  0.09 &    8.11e-12 $ \pm $    7.56e-13 \\ 
uvm2 & 55868.4922 & 16.83 $ \pm $ 0.12 & 18.03 &   1.02 $ \pm $  0.11 &    8.58e-12 $ \pm $    9.41e-13 \\ 
uvm2 & 55869.1691 & 16.93 $ \pm $ 0.10 & 18.28 &   0.93 $ \pm $  0.09 &    7.82e-12 $ \pm $    7.48e-13 \\ 
uvm2 & 55873.1206 & 17.05 $ \pm $ 0.12 & 18.26 &   0.83 $ \pm $  0.09 &    6.98e-12 $ \pm $    7.64e-13 \\ 
uvm2 & 55875.7255 & 17.32 $ \pm $ 0.16 & 18.23 &   0.65 $ \pm $  0.09 &    5.41e-12 $ \pm $    7.74e-13 \\ 
uvm2 & 55877.9446 & 17.13 $ \pm $ 0.12 & 18.29 &   0.77 $ \pm $  0.09 &    6.49e-12 $ \pm $    7.49e-13 \\ 
uvm2 & 55879.2121 & 17.32 $ \pm $ 0.14 & 18.34 &   0.65 $ \pm $  0.08 &    5.39e-12 $ \pm $    7.00e-13 \\ 
uvm2 & 55881.9593 & 17.36 $ \pm $ 0.15 & 18.34 &   0.63 $ \pm $  0.08 &    5.23e-12 $ \pm $    7.00e-13 \\ 
uvm2 & 55885.9061 & 17.37 $ \pm $ 0.14 & 18.37 &   0.62 $ \pm $  0.08 &    5.15e-12 $ \pm $    6.84e-13 \\ 
uvm2 & 55887.3118 & 17.47 $ \pm $ 0.16 & 18.35 &   0.56 $ \pm $  0.08 &    4.68e-12 $ \pm $    6.98e-13 \\ 
uvm2 & 55889.7862 & 17.38 $ \pm $ 0.17 & 18.23 &   0.61 $ \pm $  0.09 &    5.14e-12 $ \pm $    7.86e-13 \\ 
uvm2 & 55891.8463 & 17.57 $ \pm $ 0.16 & 18.44 &   0.51 $ \pm $  0.08 &    4.28e-12 $ \pm $    6.41e-13 \\ 
uvm2 & 55893.9185 & 17.94 $ \pm $ 0.20 & 18.56 &   0.37 $ \pm $  0.07 &    3.02e-12 $ \pm $    5.67e-13 \\ 
uvm2 & 55895.9232 & 17.98 $ \pm $ 0.21 & 18.57 &   0.35 $ \pm $  0.07 &    2.90e-12 $ \pm $    5.58e-13 \\ 
uvm2 & 55897.4662 & 17.56 $ \pm $ 0.17 & 18.36 &   0.52 $ \pm $  0.08 &    4.36e-12 $ \pm $    6.94e-13 \\ 
uvm2 & 55899.6699 & 17.99 $ \pm $ 0.21 & 18.58 &   0.35 $ \pm $  0.07 &    2.87e-12 $ \pm $    5.59e-13 \\ 
uvm2 & 55901.5438 & 18.53 $ \pm $ 0.31 & 18.70 &   0.21 $ \pm $  0.06 &    1.72e-12 $ \pm $    4.90e-13 \\ 
uvm2 & 55903.7392 &  0.00 $ \pm $ 0.00 & 16.46 &   0.13 $ \pm $  0.37 &    9.91e-13 $ \pm $    2.88e-12 \\ 
uvm2 & 55905.0796 & 18.18 $ \pm $ 0.24 & 18.63 &   0.29 $ \pm $  0.06 &    2.41e-12 $ \pm $    5.24e-13 \\ 
uvm2 & 55909.9591 & 18.28 $ \pm $ 0.26 & 18.65 &   0.27 $ \pm $  0.06 &    2.20e-12 $ \pm $    5.16e-13 \\ 
uvm2 & 55913.9027 & 18.28 $ \pm $ 0.26 & 18.65 &   0.27 $ \pm $  0.06 &    2.21e-12 $ \pm $    5.17e-13 \\ 
uvw1 & 55797.9237 & 17.49 $ \pm $ 0.14 & 18.49 &   0.96 $ \pm $  0.13 &    5.61e-12 $ \pm $    7.45e-13 \\ 
uvw1 & 55797.9906 & 17.23 $ \pm $ 0.13 & 18.36 &   1.22 $ \pm $  0.14 &    7.02e-12 $ \pm $    8.24e-13 \\ 
uvw1 & 55799.0019 & 16.10 $ \pm $ 0.08 & 17.69 &   3.43 $ \pm $  0.27 &    2.03e-11 $ \pm $    1.57e-12 \\ 
uvw1 & 55799.1297 & 15.89 $ \pm $ 0.07 & 17.73 &   4.16 $ \pm $  0.26 &    2.47e-11 $ \pm $    1.52e-12 \\ 
uvw1 & 55799.2073 & 15.95 $ \pm $ 0.07 & 17.78 &   3.96 $ \pm $  0.24 &    2.32e-11 $ \pm $    1.44e-12 \\ 
uvw1 & 55799.3974 & 15.77 $ \pm $ 0.06 & 17.66 &   4.65 $ \pm $  0.27 &    2.77e-11 $ \pm $    1.61e-12 \\ 
uvw1 & 55799.5356 & 15.55 $ \pm $ 0.06 & 17.58 &   5.71 $ \pm $  0.29 &    3.35e-11 $ \pm $    1.72e-12 \\ 
uvw1 & 55800.0650 & 15.31 $ \pm $ 0.05 & 17.39 &   7.11 $ \pm $  0.35 &    4.18e-11 $ \pm $    2.05e-12 \\ 
uvw1 & 55800.2044 & 15.12 $ \pm $ 0.06 & 17.12 &   8.51 $ \pm $  0.45 &    4.99e-11 $ \pm $    2.61e-12 \\ 
uvw1 & 55800.3383 & 15.02 $ \pm $ 0.05 & 17.14 &   9.28 $ \pm $  0.44 &    5.43e-11 $ \pm $    2.56e-12 \\ 
uvw1 & 55800.6089 & 14.80 $ \pm $ 0.04 & 17.09 &  11.34 $ \pm $  0.46 &    6.63e-11 $ \pm $    2.68e-12 \\ 
uvw1 & 55800.7340 & 14.71 $ \pm $ 0.05 & 16.94 &  12.36 $ \pm $  0.53 &    7.25e-11 $ \pm $    3.09e-12 \\ 
uvw1 & 55800.8075 & 14.63 $ \pm $ 0.05 & 16.76 &  13.28 $ \pm $  0.62 &    7.79e-11 $ \pm $    3.67e-12 \\ 
uvw1 & 55800.9344 & 14.65 $ \pm $ 0.05 & 16.72 &  13.02 $ \pm $  0.65 &    7.62e-11 $ \pm $    3.78e-12 \\ 
uvw1 & 55801.0131 & 14.54 $ \pm $ 0.04 & 16.80 &  14.44 $ \pm $  0.60 &    8.48e-11 $ \pm $    3.53e-12 \\ 
uvw1 & 55801.1381 & 14.47 $ \pm $ 0.05 & 16.70 &  15.45 $ \pm $  0.66 &    9.04e-11 $ \pm $    3.85e-12 \\ 
uvw1 & 55801.2182 & 14.40 $ \pm $ 0.04 & 16.69 &  16.41 $ \pm $  0.67 &    9.59e-11 $ \pm $    3.89e-12 \\ 
uvw1 & 55801.2701 & 14.35 $ \pm $ 0.04 & 16.62 &  17.26 $ \pm $  0.71 &    1.00e-10 $ \pm $    4.12e-12 \\ 
uvw1 & 55801.4034 & 14.32 $ \pm $ 0.04 & 16.61 &  17.67 $ \pm $  0.72 &    1.03e-10 $ \pm $    4.21e-12 \\ 
uvw1 & 55801.4856 & 14.27 $ \pm $ 0.04 & 16.58 &  18.58 $ \pm $  0.73 &    1.08e-10 $ \pm $    4.28e-12 \\ 
uvw1 & 55801.5472 & 14.16 $ \pm $ 0.04 & 16.47 &  20.57 $ \pm $  0.81 &    1.20e-10 $ \pm $    4.75e-12 \\ 
uvw1 & 55801.6708 & 14.08 $ \pm $ 0.04 & 16.41 &  22.16 $ \pm $  0.86 &    1.30e-10 $ \pm $    5.06e-12 \\ 
uvw1 & 55801.8049 & 14.03 $ \pm $ 0.04 & 16.36 &  23.06 $ \pm $  0.90 &    1.36e-10 $ \pm $    5.29e-12 \\ 
uvw1 & 55801.9382 & 13.94 $ \pm $ 0.04 & 16.29 &  25.08 $ \pm $  0.96 &    1.48e-10 $ \pm $    5.71e-12 \\ 
uvw1 & 55802.0104 & 13.84 $ \pm $ 0.04 & 16.21 &  27.52 $ \pm $  1.04 &    1.62e-10 $ \pm $    6.10e-12 \\ 
uvw1 & 55802.1542 & 13.75 $ \pm $ 0.04 & 16.14 &  29.91 $ \pm $  1.11 &    1.77e-10 $ \pm $    6.57e-12 \\ 
uvw1 & 55802.2113 & 13.79 $ \pm $ 0.04 & 16.23 &  28.91 $ \pm $  1.02 &    1.70e-10 $ \pm $    6.00e-12 \\ 
uvw1 & 55803.0148 & 13.15 $ \pm $ 0.04 & 15.64 &  52.00 $ \pm $  1.76 &    3.12e-10 $ \pm $    1.06e-11 \\ 
uvw1 & 55804.2943 & 12.40 $ \pm $ 0.04 & 14.90 & 103.84 $ \pm $  3.46 &    6.38e-10 $ \pm $    2.13e-11 \\ 
uvw1 & 55805.3731 & 11.90 $ \pm $ 0.04 & 14.42 & 164.64 $ \pm $  5.38 &    1.03e-09 $ \pm $    3.38e-11 \\ 
uvw1 & 55805.4279 & 11.93 $ \pm $ 0.04 & 14.45 & 160.50 $ \pm $  5.23 &    1.01e-09 $ \pm $    3.29e-11 \\ 
uvw1 & 55806.3700 & 11.59 $ \pm $ 0.04 & 14.12 & 219.09 $ \pm $  7.08 &    1.40e-09 $ \pm $    4.52e-11 \\ 
uvw1 & 55806.7623 & 11.49 $ \pm $ 0.04 & 14.01 & 240.20 $ \pm $  7.84 &    1.53e-09 $ \pm $    5.01e-11 \\ 
uvw1 & 55807.0872 & 11.46 $ \pm $ 0.04 & 13.99 & 247.01 $ \pm $  8.02 &    1.57e-09 $ \pm $    5.11e-11 \\ 
uvw1 & 55807.1537 & 11.45 $ \pm $ 0.04 & 13.98 & 249.63 $ \pm $  8.07 &    1.60e-09 $ \pm $    5.16e-11 \\ 
uvw1 & 55807.4217 & 11.41 $ \pm $ 0.04 & 13.95 & 257.51 $ \pm $  8.31 &    1.64e-09 $ \pm $    5.31e-11 \\ 
uvw1 & 55807.6979 & 11.32 $ \pm $ 0.04 & 13.85 & 279.95 $ \pm $  9.10 &    1.79e-09 $ \pm $    5.81e-11 \\ 
uvw1 & 55808.7639 & 11.17 $ \pm $ 0.04 & 13.70 & 322.98 $ \pm $ 10.46 &    2.07e-09 $ \pm $    6.70e-11 \\ 
uvw1 & 55809.7651 & 11.06 $ \pm $ 0.04 & 13.58 & 357.30 $ \pm $ 11.64 &    2.29e-09 $ \pm $    7.46e-11 \\ 
uvw1 & 55811.0401 & 11.03 $ \pm $ 0.04 & 13.57 & 365.44 $ \pm $ 11.81 &    2.33e-09 $ \pm $    7.53e-11 \\ 
uvw1 & 55811.6423 & 11.04 $ \pm $ 0.04 & 13.57 & 363.55 $ \pm $ 11.77 &    2.31e-09 $ \pm $    7.49e-11 \\ 
uvw1 & 55812.3807 & 11.00 $ \pm $ 0.04 & 13.53 & 377.86 $ \pm $ 12.23 &    2.40e-09 $ \pm $    7.78e-11 \\ 
uvw1 & 55812.5789 & 11.03 $ \pm $ 0.04 & 13.56 & 367.26 $ \pm $ 11.91 &    2.33e-09 $ \pm $    7.57e-11 \\ 
uvw1 & 55813.1241 & 11.02 $ \pm $ 0.04 & 13.54 & 368.93 $ \pm $ 12.05 &    2.35e-09 $ \pm $    7.68e-11 \\ 
uvw1 & 55814.2620 & 11.07 $ \pm $ 0.04 & 13.60 & 351.93 $ \pm $ 11.42 &    2.24e-09 $ \pm $    7.27e-11 \\ 
uvw1 & 55814.9269 & 11.12 $ \pm $ 0.04 & 13.65 & 338.25 $ \pm $ 10.95 &    2.15e-09 $ \pm $    6.97e-11 \\ 
uvw1 & 55815.2642 & 11.14 $ \pm $ 0.04 & 13.67 & 332.19 $ \pm $ 10.73 &    2.11e-09 $ \pm $    6.82e-11 \\ 
uvw1 & 55815.4004 & 11.16 $ \pm $ 0.04 & 13.69 & 323.78 $ \pm $ 10.54 &    2.05e-09 $ \pm $    6.67e-11 \\ 
uvw1 & 55816.3350 & 11.23 $ \pm $ 0.04 & 13.74 & 303.34 $ \pm $ 10.03 &    1.92e-09 $ \pm $    6.36e-11 \\ 
uvw1 & 55817.8582 & 11.43 $ \pm $ 0.04 & 13.96 & 253.74 $ \pm $  8.20 &    1.60e-09 $ \pm $    5.17e-11 \\ 
uvw1 & 55818.3967 & 11.56 $ \pm $ 0.04 & 14.09 & 225.01 $ \pm $  7.29 &    1.41e-09 $ \pm $    4.57e-11 \\ 
uvw1 & 55819.0720 & 11.63 $ \pm $ 0.04 & 14.12 & 211.53 $ \pm $  7.07 &    1.32e-09 $ \pm $    4.42e-11 \\ 
uvw1 & 55819.0735 & 11.58 $ \pm $ 0.04 & 14.11 & 220.81 $ \pm $  7.19 &    1.38e-09 $ \pm $    4.50e-11 \\ 
uvw1 & 55820.8799 & 11.93 $ \pm $ 0.04 & 14.36 & 160.06 $ \pm $  5.69 &    9.88e-10 $ \pm $    3.51e-11 \\ 
uvw1 & 55820.8810 & 11.83 $ \pm $ 0.04 & 14.34 & 175.86 $ \pm $  5.81 &    1.09e-09 $ \pm $    3.59e-11 \\ 
uvw1 & 55820.9484 & 11.87 $ \pm $ 0.04 & 14.34 & 169.72 $ \pm $  5.81 &    1.05e-09 $ \pm $    3.59e-11 \\ 
uvw1 & 55820.9500 & 11.85 $ \pm $ 0.04 & 14.36 & 172.77 $ \pm $  5.67 &    1.07e-09 $ \pm $    3.51e-11 \\ 
uvw1 & 55822.2183 & 12.12 $ \pm $ 0.04 & 14.49 & 134.54 $ \pm $  5.04 &    8.20e-10 $ \pm $    3.07e-11 \\ 
uvw1 & 55822.2193 & 12.00 $ \pm $ 0.04 & 14.50 & 150.17 $ \pm $  5.01 &    9.17e-10 $ \pm $    3.06e-11 \\ 
uvw1 & 55823.0222 & 12.02 $ \pm $ 0.04 & 14.43 & 147.47 $ \pm $  5.35 &    8.99e-10 $ \pm $    3.26e-11 \\ 
uvw1 & 55823.0232 & 12.12 $ \pm $ 0.04 & 14.62 & 134.40 $ \pm $  4.48 &    8.18e-10 $ \pm $    2.73e-11 \\ 
uvw1 & 55823.0889 & 12.09 $ \pm $ 0.04 & 14.46 & 138.00 $ \pm $  5.21 &    8.41e-10 $ \pm $    3.17e-11 \\ 
uvw1 & 55823.0898 & 12.13 $ \pm $ 0.04 & 14.62 & 133.07 $ \pm $  4.49 &    8.10e-10 $ \pm $    2.73e-11 \\ 
uvw1 & 55824.4274 & 12.31 $ \pm $ 0.04 & 14.61 & 112.57 $ \pm $  4.53 &    6.88e-10 $ \pm $    2.77e-11 \\ 
uvw1 & 55824.4282 & 12.31 $ \pm $ 0.04 & 14.80 & 112.30 $ \pm $  3.80 &    6.86e-10 $ \pm $    2.32e-11 \\ 
uvw1 & 55826.9117 & 12.54 $ \pm $ 0.04 & 14.83 &  90.99 $ \pm $  3.69 &    5.59e-10 $ \pm $    2.26e-11 \\ 
uvw1 & 55826.9128 & 12.60 $ \pm $ 0.04 & 15.08 &  86.11 $ \pm $  2.94 &    5.29e-10 $ \pm $    1.80e-11 \\ 
uvw1 & 55826.9750 & 12.66 $ \pm $ 0.05 & 14.86 &  81.98 $ \pm $  3.59 &    5.02e-10 $ \pm $    2.20e-11 \\ 
uvw1 & 55826.9759 & 12.63 $ \pm $ 0.04 & 15.10 &  84.13 $ \pm $  2.89 &    5.16e-10 $ \pm $    1.77e-11 \\ 
uvw1 & 55827.0421 & 12.65 $ \pm $ 0.05 & 14.83 &  82.07 $ \pm $  3.67 &    5.03e-10 $ \pm $    2.25e-11 \\ 
uvw1 & 55827.0424 & 12.53 $ \pm $ 0.09 & 14.04 &  92.36 $ \pm $  7.67 &    5.67e-10 $ \pm $    4.71e-11 \\ 
uvw1 & 55827.1009 & 12.68 $ \pm $ 0.04 & 15.15 &  79.94 $ \pm $  2.75 &    4.89e-10 $ \pm $    1.68e-11 \\ 
uvw1 & 55827.2376 & 12.70 $ \pm $ 0.04 & 15.18 &  78.74 $ \pm $  2.67 &    4.85e-10 $ \pm $    1.65e-11 \\ 
uvw1 & 55827.2999 & 12.73 $ \pm $ 0.04 & 15.02 &  76.28 $ \pm $  3.09 &    4.69e-10 $ \pm $    1.90e-11 \\ 
uvw1 & 55827.4345 & 12.73 $ \pm $ 0.04 & 15.12 &  76.81 $ \pm $  2.82 &    4.73e-10 $ \pm $    1.74e-11 \\ 
uvw1 & 55827.5049 & 12.69 $ \pm $ 0.04 & 15.17 &  79.77 $ \pm $  2.70 &    4.92e-10 $ \pm $    1.67e-11 \\ 
uvw1 & 55827.6445 & 12.72 $ \pm $ 0.04 & 15.20 &  77.34 $ \pm $  2.63 &    4.77e-10 $ \pm $    1.62e-11 \\ 
uvw1 & 55829.4485 & 12.85 $ \pm $ 0.05 & 15.08 &  68.74 $ \pm $  2.93 &    4.26e-10 $ \pm $    1.81e-11 \\ 
uvw1 & 55829.4497 & 12.97 $ \pm $ 0.04 & 15.44 &  61.10 $ \pm $  2.10 &    3.78e-10 $ \pm $    1.30e-11 \\ 
uvw1 & 55829.5166 & 13.05 $ \pm $ 0.05 & 15.11 &  57.08 $ \pm $  2.86 &    3.50e-10 $ \pm $    1.75e-11 \\ 
uvw1 & 55829.5175 & 12.97 $ \pm $ 0.04 & 15.41 &  61.23 $ \pm $  2.16 &    3.76e-10 $ \pm $    1.33e-11 \\ 
uvw1 & 55829.8451 & 13.01 $ \pm $ 0.06 & 15.05 &  59.43 $ \pm $  3.01 &    3.65e-10 $ \pm $    1.85e-11 \\ 
uvw1 & 55831.7981 & 13.21 $ \pm $ 0.05 & 15.30 &  49.19 $ \pm $  2.38 &    3.02e-10 $ \pm $    1.46e-11 \\ 
uvw1 & 55831.7992 & 13.30 $ \pm $ 0.04 & 15.73 &  45.42 $ \pm $  1.61 &    2.79e-10 $ \pm $    9.87e-12 \\ 
uvw1 & 55831.9202 & 13.27 $ \pm $ 0.06 & 15.30 &  46.71 $ \pm $  2.39 &    2.87e-10 $ \pm $    1.47e-11 \\ 
uvw1 & 55831.9213 & 13.29 $ \pm $ 0.04 & 15.72 &  45.69 $ \pm $  1.62 &    2.81e-10 $ \pm $    9.99e-12 \\ 
uvw1 & 55832.9896 & 13.50 $ \pm $ 0.06 & 15.41 &  37.75 $ \pm $  2.17 &    2.31e-10 $ \pm $    1.33e-11 \\ 
uvw1 & 55832.9906 & 13.45 $ \pm $ 0.04 & 15.85 &  39.53 $ \pm $  1.44 &    2.42e-10 $ \pm $    8.81e-12 \\ 
uvw1 & 55833.4640 & 13.40 $ \pm $ 0.05 & 15.57 &  41.23 $ \pm $  1.87 &    2.54e-10 $ \pm $    1.15e-11 \\ 
uvw1 & 55833.4657 & 13.48 $ \pm $ 0.04 & 15.94 &  38.24 $ \pm $  1.33 &    2.35e-10 $ \pm $    8.19e-12 \\ 
uvw1 & 55833.5299 & 13.43 $ \pm $ 0.06 & 15.36 &  40.34 $ \pm $  2.27 &    2.47e-10 $ \pm $    1.39e-11 \\ 
uvw1 & 55833.5308 & 13.50 $ \pm $ 0.04 & 15.89 &  37.58 $ \pm $  1.39 &    2.30e-10 $ \pm $    8.49e-12 \\ 
uvw1 & 55835.4000 & 13.62 $ \pm $ 0.05 & 15.68 &  33.58 $ \pm $  1.69 &    2.06e-10 $ \pm $    1.03e-11 \\ 
uvw1 & 55835.4015 & 13.72 $ \pm $ 0.04 & 16.13 &  30.84 $ \pm $  1.12 &    1.89e-10 $ \pm $    6.83e-12 \\ 
uvw1 & 55835.4670 & 13.76 $ \pm $ 0.06 & 15.64 &  29.57 $ \pm $  1.75 &    1.80e-10 $ \pm $    1.06e-11 \\ 
uvw1 & 55835.4682 & 13.74 $ \pm $ 0.04 & 16.12 &  30.25 $ \pm $  1.12 &    1.84e-10 $ \pm $    6.85e-12 \\ 
uvw1 & 55836.4714 & 13.85 $ \pm $ 0.06 & 15.77 &  27.27 $ \pm $  1.56 &    1.66e-10 $ \pm $    9.47e-12 \\ 
uvw1 & 55836.4728 & 13.84 $ \pm $ 0.04 & 16.23 &  27.55 $ \pm $  1.01 &    1.67e-10 $ \pm $    6.16e-12 \\ 
uvw1 & 55836.5398 & 13.88 $ \pm $ 0.07 & 15.71 &  26.42 $ \pm $  1.63 &    1.59e-10 $ \pm $    9.86e-12 \\ 
uvw1 & 55836.5410 & 13.83 $ \pm $ 0.04 & 16.20 &  27.82 $ \pm $  1.04 &    1.68e-10 $ \pm $    6.28e-12 \\ 
uvw1 & 55837.4043 & 13.96 $ \pm $ 0.07 & 15.80 &  24.62 $ \pm $  1.50 &    1.49e-10 $ \pm $    9.08e-12 \\ 
uvw1 & 55837.4056 & 13.90 $ \pm $ 0.04 & 16.28 &  25.98 $ \pm $  0.97 &    1.57e-10 $ \pm $    5.86e-12 \\ 
uvw1 & 55838.3444 & 14.03 $ \pm $ 0.06 & 15.96 &  23.12 $ \pm $  1.31 &    1.40e-10 $ \pm $    7.94e-12 \\ 
uvw1 & 55838.3460 & 13.97 $ \pm $ 0.04 & 16.37 &  24.33 $ \pm $  0.90 &    1.48e-10 $ \pm $    5.44e-12 \\ 
uvw1 & 55838.9456 & 14.15 $ \pm $ 0.07 & 15.86 &  20.73 $ \pm $  1.43 &    1.25e-10 $ \pm $    8.59e-12 \\ 
uvw1 & 55838.9468 & 14.05 $ \pm $ 0.04 & 16.39 &  22.74 $ \pm $  0.88 &    1.37e-10 $ \pm $    5.31e-12 \\ 
uvw1 & 55839.6164 & 14.02 $ \pm $ 0.07 & 15.82 &  23.24 $ \pm $  1.48 &    1.41e-10 $ \pm $    8.97e-12 \\ 
uvw1 & 55839.6177 & 14.13 $ \pm $ 0.04 & 16.47 &  21.09 $ \pm $  0.81 &    1.28e-10 $ \pm $    4.92e-12 \\ 
uvw1 & 55840.2179 & 14.15 $ \pm $ 0.07 & 15.97 &  20.76 $ \pm $  1.29 &    1.25e-10 $ \pm $    7.74e-12 \\ 
uvw1 & 55840.2193 & 14.15 $ \pm $ 0.04 & 16.51 &  20.64 $ \pm $  0.79 &    1.24e-10 $ \pm $    4.73e-12 \\ 
uvw1 & 55840.3543 & 14.14 $ \pm $ 0.09 & 15.68 &  20.90 $ \pm $  1.69 &    1.26e-10 $ \pm $    1.01e-11 \\ 
uvw1 & 55840.3551 & 14.14 $ \pm $ 0.04 & 16.41 &  20.87 $ \pm $  0.86 &    1.25e-10 $ \pm $    5.17e-12 \\ 
uvw1 & 55841.3498 & 14.22 $ \pm $ 0.07 & 15.96 &  19.38 $ \pm $  1.30 &    1.17e-10 $ \pm $    7.84e-12 \\ 
uvw1 & 55841.3510 & 14.26 $ \pm $ 0.04 & 16.58 &  18.77 $ \pm $  0.73 &    1.13e-10 $ \pm $    4.42e-12 \\ 
uvw1 & 55841.8914 & 14.34 $ \pm $ 0.08 & 15.96 &  17.37 $ \pm $  1.30 &    1.05e-10 $ \pm $    7.86e-12 \\ 
uvw1 & 55841.8926 & 14.27 $ \pm $ 0.04 & 16.56 &  18.60 $ \pm $  0.75 &    1.12e-10 $ \pm $    4.54e-12 \\ 
uvw1 & 55842.0118 & 14.28 $ \pm $ 0.09 & 15.75 &  18.35 $ \pm $  1.58 &    1.11e-10 $ \pm $    9.57e-12 \\ 
uvw1 & 55842.0123 & 14.29 $ \pm $ 0.06 & 16.28 &  18.15 $ \pm $  0.97 &    1.10e-10 $ \pm $    5.85e-12 \\ 
uvw1 & 55842.3568 & 14.16 $ \pm $ 0.07 & 15.87 &  20.50 $ \pm $  1.41 &    1.24e-10 $ \pm $    8.54e-12 \\ 
uvw1 & 55842.3579 & 14.27 $ \pm $ 0.04 & 16.57 &  18.53 $ \pm $  0.74 &    1.12e-10 $ \pm $    4.46e-12 \\ 
uvw1 & 55842.8956 & 14.42 $ \pm $ 0.08 & 16.00 &  16.21 $ \pm $  1.25 &    9.84e-11 $ \pm $    7.62e-12 \\ 
uvw1 & 55842.8968 & 14.34 $ \pm $ 0.04 & 16.62 &  17.34 $ \pm $  0.71 &    1.05e-10 $ \pm $    4.30e-12 \\ 
uvw1 & 55843.4901 & 14.49 $ \pm $ 0.09 & 16.05 &  15.16 $ \pm $  1.20 &    9.16e-11 $ \pm $    7.28e-12 \\ 
uvw1 & 55843.4912 & 14.41 $ \pm $ 0.04 & 16.69 &  16.32 $ \pm $  0.67 &    9.88e-11 $ \pm $    4.03e-12 \\ 
uvw1 & 55843.7540 & 14.40 $ \pm $ 0.09 & 15.94 &  16.44 $ \pm $  1.33 &    1.00e-10 $ \pm $    8.13e-12 \\ 
uvw1 & 55843.7550 & 14.33 $ \pm $ 0.04 & 16.60 &  17.60 $ \pm $  0.72 &    1.07e-10 $ \pm $    4.39e-12 \\ 
uvw1 & 55844.0231 & 14.36 $ \pm $ 0.08 & 15.98 &  17.01 $ \pm $  1.28 &    1.03e-10 $ \pm $    7.76e-12 \\ 
uvw1 & 55844.0243 & 14.44 $ \pm $ 0.04 & 16.71 &  15.90 $ \pm $  0.65 &    9.64e-11 $ \pm $    3.96e-12 \\ 
uvw1 & 55844.0894 & 14.38 $ \pm $ 0.09 & 15.95 &  16.82 $ \pm $  1.31 &    1.02e-10 $ \pm $    7.94e-12 \\ 
uvw1 & 55844.0905 & 14.41 $ \pm $ 0.04 & 16.67 &  16.35 $ \pm $  0.68 &    9.89e-11 $ \pm $    4.08e-12 \\ 
uvw1 & 55845.4268 & 14.52 $ \pm $ 0.09 & 16.04 &  14.73 $ \pm $  1.22 &    9.02e-11 $ \pm $    7.45e-12 \\ 
uvw1 & 55845.4279 & 14.49 $ \pm $ 0.04 & 16.75 &  15.09 $ \pm $  0.63 &    9.25e-11 $ \pm $    3.87e-12 \\ 
uvw1 & 55845.4925 & 14.47 $ \pm $ 0.09 & 15.93 &  15.48 $ \pm $  1.34 &    9.54e-11 $ \pm $    8.23e-12 \\ 
uvw1 & 55845.4934 & 14.46 $ \pm $ 0.05 & 16.69 &  15.51 $ \pm $  0.66 &    9.56e-11 $ \pm $    4.09e-12 \\ 
uvw1 & 55846.7057 & 14.53 $ \pm $ 0.09 & 16.10 &  14.54 $ \pm $  1.15 &    8.95e-11 $ \pm $    7.04e-12 \\ 
uvw1 & 55846.7069 & 14.56 $ \pm $ 0.04 & 16.82 &  14.17 $ \pm $  0.59 &    8.71e-11 $ \pm $    3.63e-12 \\ 
uvw1 & 55847.4420 & 14.62 $ \pm $ 0.09 & 16.17 &  13.45 $ \pm $  1.07 &    8.26e-11 $ \pm $    6.58e-12 \\ 
uvw1 & 55847.4433 & 14.64 $ \pm $ 0.05 & 16.88 &  13.23 $ \pm $  0.56 &    8.12e-11 $ \pm $    3.44e-12 \\ 
uvw1 & 55848.0349 & 14.68 $ \pm $ 0.04 & 17.00 &  12.71 $ \pm $  0.50 &    7.87e-11 $ \pm $    3.10e-12 \\ 
uvw1 & 55849.5023 & 14.64 $ \pm $ 0.04 & 16.97 &  13.15 $ \pm $  0.52 &    8.17e-11 $ \pm $    3.20e-12 \\ 
uvw1 & 55850.7109 & 14.70 $ \pm $ 0.04 & 17.00 &  12.46 $ \pm $  0.50 &    7.76e-11 $ \pm $    3.13e-12 \\ 
uvw1 & 55851.7247 & 14.77 $ \pm $ 0.04 & 17.05 &  11.72 $ \pm $  0.48 &    7.30e-11 $ \pm $    2.98e-12 \\ 
uvw1 & 55852.3145 & 14.80 $ \pm $ 0.04 & 17.09 &  11.35 $ \pm $  0.46 &    7.07e-11 $ \pm $    2.87e-12 \\ 
uvw1 & 55853.7100 & 14.83 $ \pm $ 0.04 & 17.10 &  11.10 $ \pm $  0.46 &    6.90e-11 $ \pm $    2.84e-12 \\ 
uvw1 & 55854.7900 & 14.92 $ \pm $ 0.05 & 17.11 &  10.19 $ \pm $  0.45 &    6.42e-11 $ \pm $    2.85e-12 \\ 
uvw1 & 55854.8540 & 14.94 $ \pm $ 0.05 & 17.09 &  10.01 $ \pm $  0.46 &    6.31e-11 $ \pm $    2.89e-12 \\ 
uvw1 & 55855.5813 & 14.94 $ \pm $ 0.05 & 17.13 &   9.96 $ \pm $  0.45 &    6.19e-11 $ \pm $    2.76e-12 \\ 
uvw1 & 55855.6514 & 14.92 $ \pm $ 0.05 & 17.11 &  10.20 $ \pm $  0.45 &    6.34e-11 $ \pm $    2.81e-12 \\ 
uvw1 & 55856.3842 & 14.94 $ \pm $ 0.05 & 17.11 &  10.02 $ \pm $  0.45 &    6.21e-11 $ \pm $    2.81e-12 \\ 
uvw1 & 55856.4512 & 14.93 $ \pm $ 0.05 & 17.09 &  10.14 $ \pm $  0.46 &    6.30e-11 $ \pm $    2.87e-12 \\ 
uvw1 & 55857.4537 & 14.93 $ \pm $ 0.05 & 17.13 &  10.12 $ \pm $  0.44 &    6.30e-11 $ \pm $    2.75e-12 \\ 
uvw1 & 55857.5196 & 14.92 $ \pm $ 0.06 & 16.89 &  10.16 $ \pm $  0.56 &    6.29e-11 $ \pm $    3.44e-12 \\ 
uvw1 & 55858.5225 & 15.01 $ \pm $ 0.06 & 16.94 &   9.39 $ \pm $  0.53 &    5.85e-11 $ \pm $    3.29e-12 \\ 
uvw1 & 55859.5290 & 14.98 $ \pm $ 0.05 & 17.10 &   9.65 $ \pm $  0.46 &    5.97e-11 $ \pm $    2.81e-12 \\ 
uvw1 & 55860.0020 & 15.06 $ \pm $ 0.05 & 17.16 &   8.98 $ \pm $  0.43 &    5.55e-11 $ \pm $    2.67e-12 \\ 
uvw1 & 55861.1305 & 15.21 $ \pm $ 0.05 & 17.39 &   7.83 $ \pm $  0.35 &    4.82e-11 $ \pm $    2.15e-12 \\ 
uvw1 & 55862.2672 & 15.09 $ \pm $ 0.05 & 17.29 &   8.68 $ \pm $  0.38 &    5.36e-11 $ \pm $    2.36e-12 \\ 
uvw1 & 55863.0028 & 15.13 $ \pm $ 0.05 & 17.32 &   8.36 $ \pm $  0.37 &    5.20e-11 $ \pm $    2.31e-12 \\ 
uvw1 & 55864.8766 & 15.21 $ \pm $ 0.05 & 17.38 &   7.82 $ \pm $  0.35 &    4.84e-11 $ \pm $    2.17e-12 \\ 
uvw1 & 55865.2097 & 15.18 $ \pm $ 0.05 & 17.36 &   8.01 $ \pm $  0.36 &    4.94e-11 $ \pm $    2.20e-12 \\ 
uvw1 & 55866.8826 & 15.24 $ \pm $ 0.05 & 17.40 &   7.57 $ \pm $  0.34 &    4.69e-11 $ \pm $    2.14e-12 \\ 
uvw1 & 55867.3552 & 15.32 $ \pm $ 0.06 & 17.24 &   7.03 $ \pm $  0.40 &    4.30e-11 $ \pm $    2.45e-12 \\ 
uvw1 & 55867.9550 & 15.32 $ \pm $ 0.05 & 17.40 &   7.05 $ \pm $  0.35 &    4.34e-11 $ \pm $    2.13e-12 \\ 
uvw1 & 55868.0862 & 15.28 $ \pm $ 0.05 & 17.46 &   7.32 $ \pm $  0.33 &    4.50e-11 $ \pm $    2.01e-12 \\ 
uvw1 & 55868.4872 & 15.30 $ \pm $ 0.06 & 17.19 &   7.16 $ \pm $  0.42 &    4.40e-11 $ \pm $    2.58e-12 \\ 
uvw1 & 55869.1567 & 15.30 $ \pm $ 0.05 & 17.44 &   7.17 $ \pm $  0.33 &    4.40e-11 $ \pm $    2.05e-12 \\ 
uvw1 & 55873.1088 & 15.43 $ \pm $ 0.05 & 17.51 &   6.38 $ \pm $  0.31 &    3.91e-11 $ \pm $    1.90e-12 \\ 
uvw1 & 55875.7203 & 15.98 $ \pm $ 0.10 & 17.43 &   3.85 $ \pm $  0.34 &    2.30e-11 $ \pm $    2.02e-12 \\ 
uvw1 & 55877.9327 & 15.59 $ \pm $ 0.06 & 17.61 &   5.49 $ \pm $  0.29 &    3.37e-11 $ \pm $    1.76e-12 \\ 
uvw1 & 55879.2004 & 15.67 $ \pm $ 0.06 & 17.64 &   5.12 $ \pm $  0.28 &    3.11e-11 $ \pm $    1.67e-12 \\ 
uvw1 & 55881.9471 & 15.62 $ \pm $ 0.06 & 17.64 &   5.32 $ \pm $  0.28 &    3.24e-11 $ \pm $    1.68e-12 \\ 
uvw1 & 55883.0332 & 15.66 $ \pm $ 0.06 & 17.56 &   5.15 $ \pm $  0.30 &    3.14e-11 $ \pm $    1.81e-12 \\ 
uvw1 & 55885.8934 & 15.77 $ \pm $ 0.06 & 17.75 &   4.68 $ \pm $  0.25 &    2.85e-11 $ \pm $    1.54e-12 \\ 
uvw1 & 55887.3015 & 15.79 $ \pm $ 0.06 & 17.73 &   4.58 $ \pm $  0.25 &    2.79e-11 $ \pm $    1.55e-12 \\ 
uvw1 & 55889.7761 & 15.84 $ \pm $ 0.06 & 17.79 &   4.37 $ \pm $  0.24 &    2.67e-11 $ \pm $    1.48e-12 \\ 
uvw1 & 55891.8345 & 15.89 $ \pm $ 0.06 & 17.80 &   4.17 $ \pm $  0.24 &    2.54e-11 $ \pm $    1.46e-12 \\ 
uvw1 & 55893.9067 & 15.97 $ \pm $ 0.06 & 17.86 &   3.86 $ \pm $  0.23 &    2.31e-11 $ \pm $    1.36e-12 \\ 
uvw1 & 55895.9116 & 16.00 $ \pm $ 0.07 & 17.87 &   3.77 $ \pm $  0.23 &    2.26e-11 $ \pm $    1.35e-12 \\ 
uvw1 & 55897.4596 & 15.97 $ \pm $ 0.07 & 17.68 &   3.87 $ \pm $  0.27 &    2.37e-11 $ \pm $    1.64e-12 \\ 
uvw1 & 55899.6575 & 16.09 $ \pm $ 0.07 & 17.93 &   3.47 $ \pm $  0.21 &    2.08e-11 $ \pm $    1.27e-12 \\ 
uvw1 & 55901.5315 & 16.11 $ \pm $ 0.07 & 17.95 &   3.40 $ \pm $  0.21 &    2.00e-11 $ \pm $    1.23e-12 \\ 
uvw1 & 55903.7306 & 16.16 $ \pm $ 0.07 & 17.97 &   3.27 $ \pm $  0.20 &    1.88e-11 $ \pm $    1.18e-12 \\ 
uvw1 & 55905.0668 & 16.23 $ \pm $ 0.07 & 18.02 &   3.04 $ \pm $  0.20 &    1.82e-11 $ \pm $    1.17e-12 \\ 
uvw1 & 55909.9472 & 16.25 $ \pm $ 0.07 & 18.02 &   2.98 $ \pm $  0.20 &    1.79e-11 $ \pm $    1.18e-12 \\ 
uvw1 & 55913.8905 & 16.46 $ \pm $ 0.08 & 18.12 &   2.47 $ \pm $  0.18 &    1.49e-11 $ \pm $    1.07e-12 \\ 
u & 55797.9252 & 15.78 $ \pm $ 0.07 & 17.57 &  10.58 $ \pm $  0.68 &    5.92e-11 $ \pm $    3.79e-12 \\ 
u & 55797.9921 & 15.65 $ \pm $ 0.07 & 17.51 &  11.87 $ \pm $  0.71 &    6.63e-11 $ \pm $    3.99e-12 \\ 
u & 55799.0028 & 14.33 $ \pm $ 0.05 & 16.55 &  40.07 $ \pm $  1.74 &    2.24e-10 $ \pm $    9.71e-12 \\ 
u & 55799.1311 & 14.20 $ \pm $ 0.04 & 16.49 &  45.18 $ \pm $  1.83 &    2.53e-10 $ \pm $    1.02e-11 \\ 
u & 55799.2087 & 14.20 $ \pm $ 0.04 & 16.54 &  45.20 $ \pm $  1.75 &    2.52e-10 $ \pm $    9.78e-12 \\ 
u & 55799.3988 & 14.00 $ \pm $ 0.04 & 16.35 &  54.60 $ \pm $  2.08 &    3.05e-10 $ \pm $    1.16e-11 \\ 
u & 55799.5373 & 13.88 $ \pm $ 0.04 & 16.28 &  60.71 $ \pm $  2.22 &    3.39e-10 $ \pm $    1.24e-11 \\ 
u & 55800.0665 & 13.49 $ \pm $ 0.04 & 15.92 &  87.24 $ \pm $  3.10 &    4.87e-10 $ \pm $    1.73e-11 \\ 
u & 55800.2053 & 13.35 $ \pm $ 0.04 & 15.76 &  98.82 $ \pm $  3.58 &    5.51e-10 $ \pm $    2.00e-11 \\ 
u & 55800.3395 & 13.27 $ \pm $ 0.04 & 15.73 & 106.58 $ \pm $  3.70 &    5.95e-10 $ \pm $    2.06e-11 \\ 
u & 55800.6110 & 13.07 $ \pm $ 0.04 & 15.57 & 128.49 $ \pm $  4.29 &    7.17e-10 $ \pm $    2.39e-11 \\ 
u & 55800.7353 & 13.00 $ \pm $ 0.04 & 15.49 & 136.22 $ \pm $  4.62 &    7.60e-10 $ \pm $    2.58e-11 \\ 
u & 55800.8082 & 12.99 $ \pm $ 0.04 & 15.46 & 137.45 $ \pm $  4.75 &    7.67e-10 $ \pm $    2.65e-11 \\ 
u & 55800.9350 & 12.84 $ \pm $ 0.04 & 15.30 & 158.63 $ \pm $  5.48 &    8.85e-10 $ \pm $    3.06e-11 \\ 
u & 55801.1391 & 12.68 $ \pm $ 0.04 & 15.18 & 183.93 $ \pm $  6.14 &    1.03e-09 $ \pm $    3.43e-11 \\ 
u & 55801.2194 & 12.61 $ \pm $ 0.04 & 15.12 & 196.32 $ \pm $  6.45 &    1.09e-09 $ \pm $    3.60e-11 \\ 
u & 55801.4868 & 12.50 $ \pm $ 0.04 & 15.02 & 217.00 $ \pm $  7.12 &    1.21e-09 $ \pm $    3.97e-11 \\ 
u & 55801.5368 & 12.50 $ \pm $ 0.04 & 14.96 & 217.46 $ \pm $  7.49 &    1.21e-09 $ \pm $    4.17e-11 \\ 
u & 55801.5376 & 12.44 $ \pm $ 0.04 & 14.95 & 229.24 $ \pm $  7.55 &    1.28e-09 $ \pm $    4.20e-11 \\ 
u & 55828.1791 & 11.26 $ \pm $ 0.04 & 13.78 & 682.43 $ \pm $ 22.16 &    3.81e-09 $ \pm $    1.24e-10 \\ 
u & 55829.4524 & 11.44 $ \pm $ 0.04 & 13.97 & 578.36 $ \pm $ 18.66 &    3.23e-09 $ \pm $    1.04e-10 \\ 
u & 55829.5195 & 11.44 $ \pm $ 0.04 & 13.96 & 577.42 $ \pm $ 18.80 &    3.22e-09 $ \pm $    1.05e-10 \\ 
u & 55831.8015 & 11.76 $ \pm $ 0.04 & 14.28 & 430.60 $ \pm $ 14.05 &    2.40e-09 $ \pm $    7.84e-11 \\ 
u & 55831.9232 & 11.78 $ \pm $ 0.04 & 14.31 & 420.89 $ \pm $ 13.68 &    2.35e-09 $ \pm $    7.63e-11 \\ 
u & 55832.9926 & 11.92 $ \pm $ 0.04 & 14.45 & 369.47 $ \pm $ 12.04 &    2.06e-09 $ \pm $    6.71e-11 \\ 
u & 55833.4695 & 11.99 $ \pm $ 0.04 & 14.52 & 347.73 $ \pm $ 11.25 &    1.94e-09 $ \pm $    6.27e-11 \\ 
u & 55833.5325 & 12.01 $ \pm $ 0.04 & 14.50 & 340.32 $ \pm $ 11.50 &    1.90e-09 $ \pm $    6.40e-11 \\ 
u & 55835.4035 & 12.34 $ \pm $ 0.04 & 14.85 & 250.44 $ \pm $  8.26 &    1.39e-09 $ \pm $    4.60e-11 \\ 
u & 55835.4050 & 12.24 $ \pm $ 0.04 & 14.77 & 275.47 $ \pm $  8.95 &    1.53e-09 $ \pm $    4.98e-11 \\ 
u & 55835.4697 & 12.36 $ \pm $ 0.04 & 14.85 & 247.09 $ \pm $  8.28 &    1.37e-09 $ \pm $    4.60e-11 \\ 
u & 55835.4708 & 12.25 $ \pm $ 0.04 & 14.77 & 273.83 $ \pm $  8.96 &    1.52e-09 $ \pm $    4.98e-11 \\ 
u & 55836.4744 & 12.38 $ \pm $ 0.04 & 14.88 & 241.92 $ \pm $  8.05 &    1.34e-09 $ \pm $    4.48e-11 \\ 
u & 55836.4755 & 12.35 $ \pm $ 0.04 & 14.87 & 248.25 $ \pm $  8.12 &    1.38e-09 $ \pm $    4.51e-11 \\ 
u & 55836.5425 & 12.40 $ \pm $ 0.04 & 14.89 & 236.98 $ \pm $  7.96 &    1.32e-09 $ \pm $    4.42e-11 \\ 
u & 55836.5432 & 12.36 $ \pm $ 0.04 & 14.87 & 246.77 $ \pm $  8.14 &    1.37e-09 $ \pm $    4.52e-11 \\ 
u & 55836.6693 & 12.45 $ \pm $ 0.04 & 14.97 & 227.63 $ \pm $  7.40 &    1.26e-09 $ \pm $    4.11e-11 \\ 
u & 55836.7276 & 12.49 $ \pm $ 0.04 & 15.01 & 218.54 $ \pm $  7.15 &    1.21e-09 $ \pm $    3.97e-11 \\ 
u & 55836.7942 & 12.46 $ \pm $ 0.04 & 14.98 & 224.84 $ \pm $  7.33 &    1.25e-09 $ \pm $    4.07e-11 \\ 
u & 55836.8609 & 12.51 $ \pm $ 0.04 & 15.04 & 214.34 $ \pm $  7.00 &    1.19e-09 $ \pm $    3.89e-11 \\ 
u & 55836.9283 & 12.48 $ \pm $ 0.04 & 15.01 & 219.86 $ \pm $  7.14 &    1.22e-09 $ \pm $    3.97e-11 \\ 
u & 55836.9949 & 12.46 $ \pm $ 0.04 & 14.99 & 224.64 $ \pm $  7.32 &    1.25e-09 $ \pm $    4.06e-11 \\ 
u & 55838.3480 & 12.55 $ \pm $ 0.04 & 15.04 & 206.47 $ \pm $  6.97 &    1.15e-09 $ \pm $    3.87e-11 \\ 
u & 55838.3496 & 12.55 $ \pm $ 0.04 & 15.06 & 207.83 $ \pm $  6.85 &    1.15e-09 $ \pm $    3.80e-11 \\ 
u & 55838.9482 & 12.63 $ \pm $ 0.04 & 15.09 & 192.52 $ \pm $  6.62 &    1.07e-09 $ \pm $    3.67e-11 \\ 
u & 55838.9494 & 12.62 $ \pm $ 0.04 & 15.13 & 194.23 $ \pm $  6.40 &    1.08e-09 $ \pm $    3.55e-11 \\ 
u & 55839.6192 & 12.66 $ \pm $ 0.04 & 15.13 & 186.99 $ \pm $  6.44 &    1.04e-09 $ \pm $    3.57e-11 \\ 
u & 55839.6204 & 12.67 $ \pm $ 0.04 & 15.18 & 185.29 $ \pm $  6.11 &    1.03e-09 $ \pm $    3.39e-11 \\ 
u & 55840.2212 & 12.77 $ \pm $ 0.04 & 15.22 & 169.58 $ \pm $  5.89 &    9.40e-10 $ \pm $    3.26e-11 \\ 
u & 55840.2226 & 12.75 $ \pm $ 0.04 & 15.26 & 171.95 $ \pm $  5.71 &    9.53e-10 $ \pm $    3.16e-11 \\ 
u & 55840.3563 & 12.81 $ \pm $ 0.04 & 15.21 & 162.21 $ \pm $  5.98 &    8.99e-10 $ \pm $    3.31e-11 \\ 
u & 55840.3571 & 12.72 $ \pm $ 0.04 & 15.21 & 176.59 $ \pm $  5.93 &    9.78e-10 $ \pm $    3.28e-11 \\ 
u & 55841.3526 & 12.84 $ \pm $ 0.04 & 15.29 & 157.95 $ \pm $  5.52 &    8.75e-10 $ \pm $    3.06e-11 \\ 
u & 55841.3539 & 12.83 $ \pm $ 0.04 & 15.35 & 159.43 $ \pm $  5.25 &    8.83e-10 $ \pm $    2.91e-11 \\ 
u & 55841.8940 & 12.78 $ \pm $ 0.04 & 15.21 & 167.64 $ \pm $  5.95 &    9.29e-10 $ \pm $    3.30e-11 \\ 
u & 55841.8952 & 12.85 $ \pm $ 0.04 & 15.34 & 157.71 $ \pm $  5.30 &    8.74e-10 $ \pm $    2.94e-11 \\ 
u & 55842.3594 & 12.89 $ \pm $ 0.04 & 15.31 & 151.56 $ \pm $  5.41 &    8.40e-10 $ \pm $    3.00e-11 \\ 
u & 55842.3604 & 12.88 $ \pm $ 0.04 & 15.38 & 152.95 $ \pm $  5.10 &    8.47e-10 $ \pm $    2.83e-11 \\ 
u & 55842.8982 & 12.87 $ \pm $ 0.04 & 15.29 & 153.57 $ \pm $  5.53 &    8.51e-10 $ \pm $    3.07e-11 \\ 
u & 55842.8994 & 12.93 $ \pm $ 0.04 & 15.42 & 145.80 $ \pm $  4.91 &    8.08e-10 $ \pm $    2.72e-11 \\ 
u & 55843.4927 & 12.97 $ \pm $ 0.04 & 15.39 & 139.90 $ \pm $  5.02 &    7.75e-10 $ \pm $    2.78e-11 \\ 
u & 55843.4937 & 12.99 $ \pm $ 0.04 & 15.49 & 137.99 $ \pm $  4.58 &    7.65e-10 $ \pm $    2.54e-11 \\ 
u & 55843.7564 & 12.96 $ \pm $ 0.04 & 15.36 & 142.37 $ \pm $  5.20 &    7.89e-10 $ \pm $    2.88e-11 \\ 
u & 55843.7571 & 13.00 $ \pm $ 0.04 & 15.48 & 137.09 $ \pm $  4.62 &    7.60e-10 $ \pm $    2.56e-11 \\ 
u & 55844.0258 & 13.05 $ \pm $ 0.04 & 15.44 & 130.82 $ \pm $  4.81 &    7.25e-10 $ \pm $    2.66e-11 \\ 
u & 55844.0262 & 13.02 $ \pm $ 0.04 & 15.45 & 133.86 $ \pm $  4.79 &    7.42e-10 $ \pm $    2.66e-11 \\ 
u & 55844.0920 & 12.94 $ \pm $ 0.04 & 15.35 & 144.52 $ \pm $  5.24 &    8.01e-10 $ \pm $    2.90e-11 \\ 
u & 55844.0923 & 13.02 $ \pm $ 0.04 & 15.32 & 134.48 $ \pm $  5.36 &    7.45e-10 $ \pm $    2.97e-11 \\ 
u & 55845.4294 & 13.12 $ \pm $ 0.04 & 15.50 & 122.19 $ \pm $  4.57 &    6.78e-10 $ \pm $    2.54e-11 \\ 
u & 55845.4304 & 13.11 $ \pm $ 0.04 & 15.61 & 123.28 $ \pm $  4.12 &    6.84e-10 $ \pm $    2.29e-11 \\ 
u & 55845.4947 & 13.12 $ \pm $ 0.04 & 15.47 & 122.10 $ \pm $  4.67 &    6.78e-10 $ \pm $    2.59e-11 \\ 
u & 55845.4954 & 13.13 $ \pm $ 0.04 & 15.60 & 121.64 $ \pm $  4.16 &    6.75e-10 $ \pm $    2.31e-11 \\ 
u & 55846.7084 & 13.25 $ \pm $ 0.04 & 15.61 & 109.08 $ \pm $  4.13 &    6.05e-10 $ \pm $    2.29e-11 \\ 
u & 55846.7096 & 13.17 $ \pm $ 0.04 & 15.66 & 116.84 $ \pm $  3.92 &    6.48e-10 $ \pm $    2.17e-11 \\ 
u & 55847.4449 & 13.27 $ \pm $ 0.04 & 15.63 & 106.42 $ \pm $  4.03 &    5.91e-10 $ \pm $    2.23e-11 \\ 
u & 55847.4461 & 13.20 $ \pm $ 0.04 & 15.69 & 113.71 $ \pm $  3.82 &    6.31e-10 $ \pm $    2.12e-11 \\ 
u & 55848.0370 & 13.25 $ \pm $ 0.04 & 15.74 & 108.54 $ \pm $  3.64 &    6.03e-10 $ \pm $    2.02e-11 \\ 
u & 55848.5079 & 13.31 $ \pm $ 0.04 & 15.57 & 103.16 $ \pm $  4.27 &    5.73e-10 $ \pm $    2.37e-11 \\ 
u & 55848.5087 & 13.27 $ \pm $ 0.04 & 15.74 & 107.05 $ \pm $  3.66 &    5.95e-10 $ \pm $    2.03e-11 \\ 
u & 55849.5045 & 13.30 $ \pm $ 0.04 & 15.79 & 103.66 $ \pm $  3.50 &    5.76e-10 $ \pm $    1.94e-11 \\ 
u & 55850.7128 & 13.38 $ \pm $ 0.04 & 15.86 &  96.38 $ \pm $  3.28 &    5.36e-10 $ \pm $    1.82e-11 \\ 
u & 55851.6550 & 13.42 $ \pm $ 0.05 & 15.65 &  92.75 $ \pm $  3.99 &    5.15e-10 $ \pm $    2.22e-11 \\ 
u & 55851.6558 & 13.40 $ \pm $ 0.04 & 15.86 &  94.73 $ \pm $  3.28 &    5.26e-10 $ \pm $    1.82e-11 \\ 
u & 55851.7265 & 13.36 $ \pm $ 0.04 & 15.83 &  97.78 $ \pm $  3.36 &    5.43e-10 $ \pm $    1.87e-11 \\ 
u & 55852.2378 & 13.49 $ \pm $ 0.05 & 15.69 &  86.92 $ \pm $  3.82 &    4.83e-10 $ \pm $    2.12e-11 \\ 
u & 55852.2386 & 13.40 $ \pm $ 0.04 & 15.86 &  94.34 $ \pm $  3.27 &    5.24e-10 $ \pm $    1.81e-11 \\ 
u & 55852.3165 & 13.45 $ \pm $ 0.04 & 15.92 &  90.31 $ \pm $  3.09 &    5.02e-10 $ \pm $    1.71e-11 \\ 
u & 55853.3079 & 13.56 $ \pm $ 0.05 & 15.72 &  81.86 $ \pm $  3.71 &    4.55e-10 $ \pm $    2.06e-11 \\ 
u & 55853.3088 & 13.46 $ \pm $ 0.04 & 15.90 &  89.86 $ \pm $  3.14 &    4.99e-10 $ \pm $    1.75e-11 \\ 
u & 55853.7120 & 13.47 $ \pm $ 0.04 & 15.93 &  88.32 $ \pm $  3.07 &    4.90e-10 $ \pm $    1.70e-11 \\ 
u & 55854.7913 & 13.47 $ \pm $ 0.04 & 15.91 &  89.03 $ \pm $  3.12 &    4.95e-10 $ \pm $    1.73e-11 \\ 
u & 55854.8552 & 13.50 $ \pm $ 0.04 & 15.94 &  86.11 $ \pm $  3.06 &    4.79e-10 $ \pm $    1.70e-11 \\ 
u & 55855.5826 & 13.52 $ \pm $ 0.04 & 15.96 &  84.58 $ \pm $  2.98 &    4.69e-10 $ \pm $    1.65e-11 \\ 
u & 55855.6527 & 13.51 $ \pm $ 0.04 & 15.96 &  85.33 $ \pm $  3.00 &    4.74e-10 $ \pm $    1.66e-11 \\ 
u & 55856.3854 & 13.57 $ \pm $ 0.04 & 15.99 &  80.67 $ \pm $  2.89 &    4.48e-10 $ \pm $    1.60e-11 \\ 
u & 55856.4524 & 13.59 $ \pm $ 0.04 & 16.00 &  79.52 $ \pm $  2.86 &    4.41e-10 $ \pm $    1.59e-11 \\ 
u & 55857.4552 & 13.59 $ \pm $ 0.04 & 16.02 &  79.49 $ \pm $  2.82 &    4.41e-10 $ \pm $    1.56e-11 \\ 
u & 55857.5202 & 13.61 $ \pm $ 0.04 & 15.94 &  78.35 $ \pm $  3.05 &    4.35e-10 $ \pm $    1.69e-11 \\ 
u & 55857.5246 & 13.65 $ \pm $ 0.05 & 15.79 &  75.12 $ \pm $  3.50 &    4.17e-10 $ \pm $    1.94e-11 \\ 
u & 55857.5254 & 13.66 $ \pm $ 0.04 & 16.10 &  74.14 $ \pm $  2.63 &    4.11e-10 $ \pm $    1.46e-11 \\ 
u & 55858.5231 & 13.62 $ \pm $ 0.04 & 15.95 &  77.54 $ \pm $  3.02 &    4.30e-10 $ \pm $    1.68e-11 \\ 
u & 55858.5274 & 13.56 $ \pm $ 0.05 & 15.73 &  81.73 $ \pm $  3.69 &    4.54e-10 $ \pm $    2.05e-11 \\ 
u & 55858.5282 & 13.63 $ \pm $ 0.04 & 16.06 &  76.57 $ \pm $  2.71 &    4.25e-10 $ \pm $    1.50e-11 \\ 
u & 55859.5302 & 13.63 $ \pm $ 0.04 & 16.04 &  76.29 $ \pm $  2.77 &    4.23e-10 $ \pm $    1.54e-11 \\ 
u & 55860.0031 & 13.66 $ \pm $ 0.04 & 16.06 &  74.56 $ \pm $  2.73 &    4.14e-10 $ \pm $    1.51e-11 \\ 
u & 55860.0617 & 13.62 $ \pm $ 0.04 & 15.98 &  76.92 $ \pm $  2.92 &    4.27e-10 $ \pm $    1.62e-11 \\ 
u & 55860.0677 & 13.61 $ \pm $ 0.05 & 15.76 &  77.92 $ \pm $  3.58 &    4.32e-10 $ \pm $    1.98e-11 \\ 
u & 55860.0685 & 13.67 $ \pm $ 0.04 & 16.10 &  73.91 $ \pm $  2.63 &    4.10e-10 $ \pm $    1.46e-11 \\ 
u & 55861.1324 & 13.77 $ \pm $ 0.04 & 16.21 &  67.26 $ \pm $  2.38 &    3.73e-10 $ \pm $    1.32e-11 \\ 
u & 55861.5986 & 13.70 $ \pm $ 0.05 & 15.83 &  72.04 $ \pm $  3.38 &    4.00e-10 $ \pm $    1.87e-11 \\ 
u & 55861.5994 & 13.69 $ \pm $ 0.04 & 16.13 &  72.58 $ \pm $  2.56 &    4.03e-10 $ \pm $    1.42e-11 \\ 
u & 55862.2690 & 13.72 $ \pm $ 0.04 & 16.16 &  70.63 $ \pm $  2.48 &    3.92e-10 $ \pm $    1.38e-11 \\ 
u & 55862.7339 & 13.77 $ \pm $ 0.05 & 15.87 &  67.23 $ \pm $  3.23 &    3.74e-10 $ \pm $    1.79e-11 \\ 
u & 55862.7347 & 13.73 $ \pm $ 0.04 & 16.17 &  69.80 $ \pm $  2.46 &    3.88e-10 $ \pm $    1.37e-11 \\ 
u & 55863.0046 & 13.76 $ \pm $ 0.04 & 16.19 &  68.02 $ \pm $  2.41 &    3.78e-10 $ \pm $    1.34e-11 \\ 
u & 55864.1387 & 13.69 $ \pm $ 0.05 & 15.82 &  72.26 $ \pm $  3.39 &    4.02e-10 $ \pm $    1.88e-11 \\ 
u & 55864.1395 & 13.72 $ \pm $ 0.04 & 16.16 &  70.39 $ \pm $  2.49 &    3.91e-10 $ \pm $    1.38e-11 \\ 
u & 55864.8785 & 13.80 $ \pm $ 0.04 & 16.23 &  65.73 $ \pm $  2.33 &    3.66e-10 $ \pm $    1.30e-11 \\ 
u & 55865.0077 & 13.85 $ \pm $ 0.05 & 15.92 &  62.55 $ \pm $  3.10 &    3.48e-10 $ \pm $    1.72e-11 \\ 
u & 55865.0085 & 13.76 $ \pm $ 0.04 & 16.20 &  67.97 $ \pm $  2.40 &    3.78e-10 $ \pm $    1.33e-11 \\ 
u & 55865.2117 & 13.79 $ \pm $ 0.04 & 16.23 &  65.87 $ \pm $  2.33 &    3.66e-10 $ \pm $    1.29e-11 \\ 
u & 55866.6131 & 13.80 $ \pm $ 0.05 & 15.89 &  65.57 $ \pm $  3.18 &    3.65e-10 $ \pm $    1.77e-11 \\ 
u & 55866.6139 & 13.89 $ \pm $ 0.04 & 16.32 &  59.99 $ \pm $  2.15 &    3.34e-10 $ \pm $    1.19e-11 \\ 
u & 55866.8844 & 13.80 $ \pm $ 0.04 & 16.24 &  65.26 $ \pm $  2.31 &    3.63e-10 $ \pm $    1.28e-11 \\ 
u & 55867.2152 & 13.76 $ \pm $ 0.05 & 15.87 &  67.99 $ \pm $  3.24 &    3.78e-10 $ \pm $    1.80e-11 \\ 
u & 55867.2160 & 13.82 $ \pm $ 0.04 & 16.25 &  64.34 $ \pm $  2.28 &    3.58e-10 $ \pm $    1.27e-11 \\ 
u & 55867.3560 & 13.81 $ \pm $ 0.04 & 16.14 &  64.86 $ \pm $  2.52 &    3.61e-10 $ \pm $    1.40e-11 \\ 
u & 55867.9564 & 13.77 $ \pm $ 0.04 & 16.18 &  67.09 $ \pm $  2.45 &    3.73e-10 $ \pm $    1.36e-11 \\ 
u & 55868.0188 & 13.88 $ \pm $ 0.05 & 15.95 &  60.85 $ \pm $  3.02 &    3.39e-10 $ \pm $    1.68e-11 \\ 
u & 55868.0196 & 13.85 $ \pm $ 0.04 & 16.28 &  62.79 $ \pm $  2.22 &    3.49e-10 $ \pm $    1.24e-11 \\ 
u & 55868.0883 & 13.83 $ \pm $ 0.04 & 16.26 &  63.70 $ \pm $  2.26 &    3.54e-10 $ \pm $    1.26e-11 \\ 
u & 55868.4879 & 13.85 $ \pm $ 0.04 & 16.16 &  62.75 $ \pm $  2.48 &    3.49e-10 $ \pm $    1.38e-11 \\ 
u & 55869.0223 & 13.90 $ \pm $ 0.06 & 15.95 &  59.79 $ \pm $  3.03 &    3.33e-10 $ \pm $    1.68e-11 \\ 
u & 55869.0231 & 13.91 $ \pm $ 0.04 & 16.32 &  59.30 $ \pm $  2.14 &    3.30e-10 $ \pm $    1.19e-11 \\ 
u & 55869.1585 & 13.87 $ \pm $ 0.04 & 16.29 &  61.13 $ \pm $  2.20 &    3.40e-10 $ \pm $    1.22e-11 \\ 
u & 55873.1106 & 13.96 $ \pm $ 0.04 & 16.34 &  56.53 $ \pm $  2.10 &    3.15e-10 $ \pm $    1.17e-11 \\ 
u & 55875.7211 & 14.03 $ \pm $ 0.05 & 16.28 &  53.13 $ \pm $  2.23 &    2.96e-10 $ \pm $    1.24e-11 \\ 
u & 55877.9345 & 14.14 $ \pm $ 0.04 & 16.48 &  47.79 $ \pm $  1.85 &    2.67e-10 $ \pm $    1.03e-11 \\ 
u & 55879.2022 & 14.12 $ \pm $ 0.04 & 16.46 &  48.82 $ \pm $  1.89 &    2.72e-10 $ \pm $    1.05e-11 \\ 
u & 55881.9490 & 14.20 $ \pm $ 0.04 & 16.55 &  45.27 $ \pm $  1.74 &    2.53e-10 $ \pm $    9.70e-12 \\ 
u & 55885.8953 & 14.26 $ \pm $ 0.04 & 16.61 &  42.71 $ \pm $  1.65 &    2.38e-10 $ \pm $    9.19e-12 \\ 
u & 55887.3032 & 14.27 $ \pm $ 0.04 & 16.61 &  42.39 $ \pm $  1.64 &    2.37e-10 $ \pm $    9.16e-12 \\ 
u & 55889.7779 & 14.33 $ \pm $ 0.04 & 16.66 &  40.22 $ \pm $  1.56 &    2.25e-10 $ \pm $    8.73e-12 \\ 
u & 55891.8364 & 14.44 $ \pm $ 0.04 & 16.75 &  36.24 $ \pm $  1.44 &    2.02e-10 $ \pm $    8.06e-12 \\ 
u & 55893.9086 & 14.54 $ \pm $ 0.04 & 16.82 &  33.22 $ \pm $  1.35 &    1.85e-10 $ \pm $    7.50e-12 \\ 
u & 55895.9133 & 14.46 $ \pm $ 0.04 & 16.77 &  35.47 $ \pm $  1.41 &    1.98e-10 $ \pm $    7.87e-12 \\ 
u & 55897.4606 & 14.57 $ \pm $ 0.05 & 16.76 &  32.22 $ \pm $  1.43 &    1.80e-10 $ \pm $    8.01e-12 \\ 
u & 55899.6593 & 14.61 $ \pm $ 0.04 & 16.90 &  31.14 $ \pm $  1.26 &    1.74e-10 $ \pm $    7.01e-12 \\ 
u & 55901.5333 & 14.68 $ \pm $ 0.04 & 16.95 &  29.04 $ \pm $  1.20 &    1.62e-10 $ \pm $    6.65e-12 \\ 
u & 55903.7324 & 14.71 $ \pm $ 0.04 & 16.98 &  28.39 $ \pm $  1.17 &    1.58e-10 $ \pm $    6.51e-12 \\ 
u & 55905.0687 & 14.75 $ \pm $ 0.04 & 17.02 &  27.24 $ \pm $  1.13 &    1.52e-10 $ \pm $    6.29e-12 \\ 
u & 55909.9490 & 14.79 $ \pm $ 0.04 & 17.04 &  26.33 $ \pm $  1.10 &    1.47e-10 $ \pm $    6.14e-12 \\ 
u & 55913.8923 & 14.95 $ \pm $ 0.05 & 17.17 &  22.63 $ \pm $  0.98 &    1.26e-10 $ \pm $    5.48e-12 \\ 
b & 55797.9261 & 15.66 $ \pm $ 0.06 & 17.70 &  23.92 $ \pm $  1.22 &    1.10e-10 $ \pm $    5.59e-12 \\ 
b & 55797.9930 & 15.50 $ \pm $ 0.05 & 17.61 &  27.78 $ \pm $  1.32 &    1.27e-10 $ \pm $    6.06e-12 \\ 
b & 55799.0032 & 14.18 $ \pm $ 0.04 & 16.58 &  93.67 $ \pm $  3.44 &    4.29e-10 $ \pm $    1.58e-11 \\ 
b & 55799.1318 & 14.12 $ \pm $ 0.04 & 16.53 &  99.37 $ \pm $  3.60 &    4.55e-10 $ \pm $    1.65e-11 \\ 
b & 55799.2094 & 14.04 $ \pm $ 0.04 & 16.50 & 106.18 $ \pm $  3.70 &    4.86e-10 $ \pm $    1.70e-11 \\ 
b & 55799.3995 & 13.88 $ \pm $ 0.04 & 16.33 & 123.39 $ \pm $  4.30 &    5.66e-10 $ \pm $    1.97e-11 \\ 
b & 55799.5382 & 13.79 $ \pm $ 0.04 & 16.27 & 134.55 $ \pm $  4.57 &    6.17e-10 $ \pm $    2.09e-11 \\ 
b & 55800.0673 & 13.36 $ \pm $ 0.04 & 15.85 & 198.82 $ \pm $  6.71 &    9.11e-10 $ \pm $    3.08e-11 \\ 
b & 55800.2058 & 13.25 $ \pm $ 0.04 & 15.74 & 221.58 $ \pm $  7.41 &    1.02e-09 $ \pm $    3.40e-11 \\ 
b & 55800.3401 & 13.13 $ \pm $ 0.04 & 15.64 & 247.51 $ \pm $  8.12 &    1.14e-09 $ \pm $    3.73e-11 \\ 
b & 55801.5396 & 12.44 $ \pm $ 0.04 & 14.97 & 466.37 $ \pm $ 15.15 &    2.14e-09 $ \pm $    6.96e-11 \\ 
b & 55848.5106 & 12.90 $ \pm $ 0.04 & 15.42 & 304.90 $ \pm $  9.99 &    1.38e-09 $ \pm $    4.52e-11 \\ 
b & 55851.6578 & 13.03 $ \pm $ 0.04 & 15.54 & 270.33 $ \pm $  8.94 &    1.22e-09 $ \pm $    4.04e-11 \\ 
b & 55852.2398 & 13.18 $ \pm $ 0.04 & 15.64 & 236.14 $ \pm $  8.15 &    1.07e-09 $ \pm $    3.69e-11 \\ 
b & 55852.2406 & 13.05 $ \pm $ 0.04 & 15.55 & 266.37 $ \pm $  8.82 &    1.21e-09 $ \pm $    4.00e-11 \\ 
b & 55853.3107 & 13.07 $ \pm $ 0.04 & 15.58 & 259.45 $ \pm $  8.62 &    1.17e-09 $ \pm $    3.90e-11 \\ 
b & 55853.7130 & 13.13 $ \pm $ 0.04 & 15.65 & 245.57 $ \pm $  8.10 &    1.11e-09 $ \pm $    3.67e-11 \\ 
b & 55854.7920 & 13.15 $ \pm $ 0.04 & 15.66 & 243.02 $ \pm $  8.01 &    1.10e-09 $ \pm $    3.63e-11 \\ 
b & 55854.8558 & 13.17 $ \pm $ 0.04 & 15.68 & 237.64 $ \pm $  7.85 &    1.08e-09 $ \pm $    3.56e-11 \\ 
b & 55855.5833 & 13.20 $ \pm $ 0.04 & 15.71 & 230.28 $ \pm $  7.63 &    1.04e-09 $ \pm $    3.46e-11 \\ 
b & 55855.6534 & 13.20 $ \pm $ 0.04 & 15.71 & 231.44 $ \pm $  7.63 &    1.05e-09 $ \pm $    3.46e-11 \\ 
b & 55856.3861 & 13.19 $ \pm $ 0.04 & 15.70 & 232.47 $ \pm $  7.73 &    1.05e-09 $ \pm $    3.50e-11 \\ 
b & 55856.4530 & 13.22 $ \pm $ 0.04 & 15.72 & 226.98 $ \pm $  7.53 &    1.03e-09 $ \pm $    3.41e-11 \\ 
b & 55857.4560 & 13.19 $ \pm $ 0.04 & 15.70 & 232.80 $ \pm $  7.69 &    1.06e-09 $ \pm $    3.48e-11 \\ 
b & 55857.5205 & 13.24 $ \pm $ 0.04 & 15.74 & 221.88 $ \pm $  7.45 &    1.01e-09 $ \pm $    3.38e-11 \\ 
b & 55857.5266 & 13.30 $ \pm $ 0.04 & 15.75 & 211.23 $ \pm $  7.36 &    9.57e-10 $ \pm $    3.34e-11 \\ 
b & 55857.5274 & 13.24 $ \pm $ 0.04 & 15.75 & 222.21 $ \pm $  7.37 &    1.01e-09 $ \pm $    3.34e-11 \\ 
b & 55858.5234 & 13.31 $ \pm $ 0.04 & 15.79 & 209.69 $ \pm $  7.08 &    9.50e-10 $ \pm $    3.21e-11 \\ 
b & 55859.5308 & 13.27 $ \pm $ 0.04 & 15.77 & 217.16 $ \pm $  7.21 &    9.83e-10 $ \pm $    3.26e-11 \\ 
b & 55860.0037 & 13.28 $ \pm $ 0.04 & 15.79 & 214.36 $ \pm $  7.11 &    9.71e-10 $ \pm $    3.22e-11 \\ 
b & 55860.0620 & 13.29 $ \pm $ 0.04 & 15.79 & 212.97 $ \pm $  7.12 &    9.65e-10 $ \pm $    3.23e-11 \\ 
b & 55860.0697 & 13.27 $ \pm $ 0.04 & 15.72 & 216.64 $ \pm $  7.53 &    9.81e-10 $ \pm $    3.41e-11 \\ 
b & 55860.0705 & 13.25 $ \pm $ 0.04 & 15.75 & 221.02 $ \pm $  7.35 &    1.00e-09 $ \pm $    3.33e-11 \\ 
b & 55861.1334 & 13.42 $ \pm $ 0.04 & 15.93 & 188.38 $ \pm $  6.26 &    8.53e-10 $ \pm $    2.83e-11 \\ 
b & 55861.6006 & 13.22 $ \pm $ 0.04 & 15.68 & 226.99 $ \pm $  7.82 &    1.03e-09 $ \pm $    3.54e-11 \\ 
b & 55861.6014 & 13.28 $ \pm $ 0.04 & 15.78 & 215.12 $ \pm $  7.16 &    9.73e-10 $ \pm $    3.24e-11 \\ 
b & 55862.2699 & 13.37 $ \pm $ 0.04 & 15.88 & 197.99 $ \pm $  6.54 &    8.96e-10 $ \pm $    2.96e-11 \\ 
b & 55862.7359 & 13.37 $ \pm $ 0.04 & 15.81 & 197.03 $ \pm $  6.96 &    8.91e-10 $ \pm $    3.15e-11 \\ 
b & 55862.7367 & 13.29 $ \pm $ 0.04 & 15.79 & 212.57 $ \pm $  7.07 &    9.61e-10 $ \pm $    3.20e-11 \\ 
b & 55863.0056 & 13.39 $ \pm $ 0.04 & 15.89 & 194.25 $ \pm $  6.44 &    8.79e-10 $ \pm $    2.92e-11 \\ 
b & 55864.1407 & 13.34 $ \pm $ 0.04 & 15.79 & 202.54 $ \pm $  7.13 &    9.17e-10 $ \pm $    3.23e-11 \\ 
b & 55864.1415 & 13.32 $ \pm $ 0.04 & 15.82 & 206.43 $ \pm $  6.89 &    9.35e-10 $ \pm $    3.12e-11 \\ 
b & 55864.8794 & 13.40 $ \pm $ 0.04 & 15.90 & 192.55 $ \pm $  6.39 &    8.70e-10 $ \pm $    2.89e-11 \\ 
b & 55865.0097 & 13.46 $ \pm $ 0.04 & 15.88 & 182.15 $ \pm $  6.53 &    8.23e-10 $ \pm $    2.95e-11 \\ 
b & 55865.0105 & 13.36 $ \pm $ 0.04 & 15.86 & 199.95 $ \pm $  6.67 &    9.04e-10 $ \pm $    3.02e-11 \\ 
b & 55865.2126 & 13.43 $ \pm $ 0.04 & 15.93 & 187.62 $ \pm $  6.22 &    8.48e-10 $ \pm $    2.81e-11 \\ 
b & 55866.6151 & 13.39 $ \pm $ 0.04 & 15.83 & 193.77 $ \pm $  6.86 &    8.74e-10 $ \pm $    3.09e-11 \\ 
b & 55866.6159 & 13.38 $ \pm $ 0.04 & 15.88 & 194.91 $ \pm $  6.51 &    8.79e-10 $ \pm $    2.94e-11 \\ 
b & 55866.8853 & 13.42 $ \pm $ 0.04 & 15.92 & 188.57 $ \pm $  6.30 &    8.52e-10 $ \pm $    2.85e-11 \\ 
b & 55867.2171 & 13.42 $ \pm $ 0.04 & 15.85 & 189.12 $ \pm $  6.72 &    8.54e-10 $ \pm $    3.03e-11 \\ 
b & 55867.2180 & 13.39 $ \pm $ 0.04 & 15.89 & 193.55 $ \pm $  6.46 &    8.74e-10 $ \pm $    2.92e-11 \\ 
b & 55867.3564 & 13.43 $ \pm $ 0.04 & 15.91 & 186.99 $ \pm $  6.35 &    8.44e-10 $ \pm $    2.86e-11 \\ 
b & 55867.9572 & 13.44 $ \pm $ 0.04 & 15.92 & 186.17 $ \pm $  6.29 &    8.40e-10 $ \pm $    2.84e-11 \\ 
b & 55868.0208 & 13.42 $ \pm $ 0.04 & 15.85 & 188.84 $ \pm $  6.74 &    8.52e-10 $ \pm $    3.04e-11 \\ 
b & 55868.0216 & 13.38 $ \pm $ 0.04 & 15.88 & 195.58 $ \pm $  6.56 &    8.83e-10 $ \pm $    2.96e-11 \\ 
b & 55868.0893 & 13.46 $ \pm $ 0.04 & 15.95 & 182.80 $ \pm $  6.12 &    8.25e-10 $ \pm $    2.76e-11 \\ 
b & 55868.4883 & 13.37 $ \pm $ 0.04 & 15.86 & 197.24 $ \pm $  6.63 &    8.90e-10 $ \pm $    2.99e-11 \\ 
b & 55869.0242 & 13.49 $ \pm $ 0.04 & 15.90 & 177.25 $ \pm $  6.43 &    7.99e-10 $ \pm $    2.90e-11 \\ 
b & 55869.0250 & 13.40 $ \pm $ 0.04 & 15.89 & 191.65 $ \pm $  6.46 &    8.65e-10 $ \pm $    2.91e-11 \\ 
b & 55869.1595 & 13.50 $ \pm $ 0.04 & 16.00 & 175.46 $ \pm $  5.87 &    7.91e-10 $ \pm $    2.65e-11 \\ 
b & 55873.1116 & 13.56 $ \pm $ 0.04 & 16.03 & 166.61 $ \pm $  5.67 &    7.50e-10 $ \pm $    2.55e-11 \\ 
b & 55875.7215 & 13.58 $ \pm $ 0.04 & 16.02 & 163.41 $ \pm $  5.72 &    7.34e-10 $ \pm $    2.57e-11 \\ 
b & 55877.9354 & 13.66 $ \pm $ 0.04 & 16.12 & 151.14 $ \pm $  5.21 &    6.79e-10 $ \pm $    2.34e-11 \\ 
b & 55879.2031 & 13.61 $ \pm $ 0.04 & 16.08 & 158.84 $ \pm $  5.43 &    7.14e-10 $ \pm $    2.44e-11 \\ 
b & 55881.9499 & 13.62 $ \pm $ 0.04 & 16.10 & 157.71 $ \pm $  5.35 &    7.08e-10 $ \pm $    2.40e-11 \\ 
b & 55885.8963 & 13.68 $ \pm $ 0.04 & 16.16 & 148.32 $ \pm $  5.05 &    6.66e-10 $ \pm $    2.27e-11 \\ 
b & 55887.3041 & 13.72 $ \pm $ 0.04 & 16.20 & 143.30 $ \pm $  4.87 &    6.44e-10 $ \pm $    2.19e-11 \\ 
b & 55889.7789 & 13.75 $ \pm $ 0.04 & 16.22 & 139.65 $ \pm $  4.77 &    6.27e-10 $ \pm $    2.14e-11 \\ 
b & 55891.8373 & 13.83 $ \pm $ 0.04 & 16.30 & 129.59 $ \pm $  4.43 &    5.82e-10 $ \pm $    1.99e-11 \\ 
b & 55893.9095 & 13.83 $ \pm $ 0.04 & 16.30 & 129.63 $ \pm $  4.42 &    5.82e-10 $ \pm $    1.98e-11 \\ 
b & 55895.9142 & 13.87 $ \pm $ 0.04 & 16.35 & 124.35 $ \pm $  4.24 &    5.59e-10 $ \pm $    1.90e-11 \\ 
b & 55897.4611 & 13.85 $ \pm $ 0.04 & 16.30 & 127.25 $ \pm $  4.43 &    5.72e-10 $ \pm $    1.99e-11 \\ 
b & 55899.6602 & 13.88 $ \pm $ 0.04 & 16.36 & 123.14 $ \pm $  4.18 &    5.53e-10 $ \pm $    1.88e-11 \\ 
b & 55901.5343 & 13.97 $ \pm $ 0.04 & 16.44 & 113.99 $ \pm $  3.90 &    5.12e-10 $ \pm $    1.75e-11 \\ 
b & 55903.7334 & 13.92 $ \pm $ 0.04 & 16.40 & 118.78 $ \pm $  4.04 &    5.33e-10 $ \pm $    1.81e-11 \\ 
b & 55905.0697 & 13.99 $ \pm $ 0.04 & 16.46 & 111.43 $ \pm $  3.81 &    5.00e-10 $ \pm $    1.71e-11 \\ 
b & 55909.9499 & 14.04 $ \pm $ 0.04 & 16.51 & 106.66 $ \pm $  3.66 &    4.79e-10 $ \pm $    1.64e-11 \\ 
b & 55913.8933 & 14.06 $ \pm $ 0.04 & 16.53 & 104.42 $ \pm $  3.58 &    4.69e-10 $ \pm $    1.61e-11 \\ 
v & 55797.9309 & 15.27 $ \pm $ 0.06 & 17.18 &  11.12 $ \pm $  0.64 &    4.08e-11 $ \pm $    2.34e-12 \\ 
v & 55797.9978 & 15.10 $ \pm $ 0.06 & 17.09 &  13.12 $ \pm $  0.70 &    4.81e-11 $ \pm $    2.56e-12 \\ 
v & 55799.0058 & 13.93 $ \pm $ 0.05 & 16.14 &  38.48 $ \pm $  1.67 &    1.41e-10 $ \pm $    6.11e-12 \\ 
v & 55799.1360 & 13.79 $ \pm $ 0.04 & 16.11 &  43.45 $ \pm $  1.72 &    1.59e-10 $ \pm $    6.29e-12 \\ 
v & 55799.2135 & 13.75 $ \pm $ 0.04 & 16.09 &  45.33 $ \pm $  1.75 &    1.66e-10 $ \pm $    6.41e-12 \\ 
v & 55799.4037 & 13.65 $ \pm $ 0.04 & 16.00 &  49.86 $ \pm $  1.90 &    1.83e-10 $ \pm $    6.96e-12 \\ 
v & 55799.5432 & 13.49 $ \pm $ 0.04 & 15.90 &  57.34 $ \pm $  2.09 &    2.10e-10 $ \pm $    7.67e-12 \\ 
v & 55800.0719 & 13.12 $ \pm $ 0.04 & 15.56 &  80.99 $ \pm $  2.84 &    2.97e-10 $ \pm $    1.04e-11 \\ 
v & 55800.2084 & 13.04 $ \pm $ 0.04 & 15.44 &  86.91 $ \pm $  3.19 &    3.19e-10 $ \pm $    1.17e-11 \\ 
v & 55800.3436 & 12.99 $ \pm $ 0.04 & 15.44 &  90.81 $ \pm $  3.19 &    3.34e-10 $ \pm $    1.17e-11 \\ 
v & 55800.6183 & 12.82 $ \pm $ 0.04 & 15.31 & 107.03 $ \pm $  3.60 &    3.94e-10 $ \pm $    1.32e-11 \\ 
v & 55800.7400 & 12.76 $ \pm $ 0.04 & 15.23 & 112.91 $ \pm $  3.85 &    4.15e-10 $ \pm $    1.42e-11 \\ 
v & 55800.8107 & 12.72 $ \pm $ 0.04 & 15.16 & 116.50 $ \pm $  4.11 &    4.29e-10 $ \pm $    1.51e-11 \\ 
v & 55800.9372 & 12.69 $ \pm $ 0.04 & 15.12 & 120.46 $ \pm $  4.29 &    4.44e-10 $ \pm $    1.58e-11 \\ 
v & 55801.1424 & 12.53 $ \pm $ 0.04 & 15.01 & 139.60 $ \pm $  4.75 &    5.14e-10 $ \pm $    1.75e-11 \\ 
v & 55801.2235 & 12.46 $ \pm $ 0.04 & 14.96 & 147.92 $ \pm $  4.94 &    5.45e-10 $ \pm $    1.82e-11 \\ 
v & 55801.4908 & 12.44 $ \pm $ 0.04 & 14.94 & 151.06 $ \pm $  5.05 &    5.57e-10 $ \pm $    1.86e-11 \\ 
v & 55801.5407 & 12.40 $ \pm $ 0.04 & 14.80 & 156.82 $ \pm $  5.75 &    5.78e-10 $ \pm $    2.12e-11 \\ 
v & 55801.5424 & 12.38 $ \pm $ 0.04 & 14.89 & 160.63 $ \pm $  5.26 &    5.92e-10 $ \pm $    1.94e-11 \\ 
v & 55802.1588 & 12.31 $ \pm $ 0.04 & 14.82 & 169.82 $ \pm $  5.64 &    6.28e-10 $ \pm $    2.09e-11 \\ 
v & 55802.2205 & 12.16 $ \pm $ 0.04 & 14.68 & 196.20 $ \pm $  6.42 &    7.25e-10 $ \pm $    2.37e-11 \\ 
v & 55804.5012 & 11.32 $ \pm $ 0.04 & 13.86 & 422.96 $ \pm $ 13.66 &    1.56e-09 $ \pm $    5.04e-11 \\ 
v & 55805.4342 & 11.11 $ \pm $ 0.04 & 13.65 & 516.36 $ \pm $ 16.56 &    1.91e-09 $ \pm $    6.11e-11 \\ 
v & 55806.7679 & 10.85 $ \pm $ 0.04 & 13.39 & 657.82 $ \pm $ 21.04 &    2.43e-09 $ \pm $    7.77e-11 \\ 
v & 55807.0237 & 10.82 $ \pm $ 0.04 & 13.36 & 675.25 $ \pm $ 21.67 &    2.50e-09 $ \pm $    8.01e-11 \\ 
v & 55831.7940 & 10.89 $ \pm $ 0.04 & 13.42 & 632.60 $ \pm $ 20.48 &    2.31e-09 $ \pm $    7.49e-11 \\ 
v & 55831.9165 & 10.89 $ \pm $ 0.04 & 13.43 & 630.87 $ \pm $ 20.30 &    2.31e-09 $ \pm $    7.43e-11 \\ 
v & 55832.9861 & 10.93 $ \pm $ 0.04 & 13.47 & 608.77 $ \pm $ 19.59 &    2.22e-09 $ \pm $    7.15e-11 \\ 
v & 55833.4582 & 10.96 $ \pm $ 0.04 & 13.50 & 588.74 $ \pm $ 18.97 &    2.15e-09 $ \pm $    6.92e-11 \\ 
v & 55833.5263 & 10.94 $ \pm $ 0.04 & 13.46 & 602.82 $ \pm $ 19.66 &    2.20e-09 $ \pm $    7.17e-11 \\ 
v & 55835.3946 & 11.04 $ \pm $ 0.04 & 13.57 & 551.42 $ \pm $ 17.76 &    2.01e-09 $ \pm $    6.46e-11 \\ 
v & 55835.4629 & 11.06 $ \pm $ 0.04 & 13.59 & 539.87 $ \pm $ 17.52 &    1.97e-09 $ \pm $    6.38e-11 \\ 
v & 55836.4668 & 11.12 $ \pm $ 0.04 & 13.65 & 512.75 $ \pm $ 16.58 &    1.86e-09 $ \pm $    6.03e-11 \\ 
v & 55836.5357 & 11.13 $ \pm $ 0.04 & 13.66 & 506.02 $ \pm $ 16.38 &    1.84e-09 $ \pm $    5.96e-11 \\ 
v & 55838.3388 & 11.21 $ \pm $ 0.04 & 13.74 & 469.26 $ \pm $ 15.24 &    1.71e-09 $ \pm $    5.54e-11 \\ 
v & 55838.9415 & 11.23 $ \pm $ 0.04 & 13.76 & 461.16 $ \pm $ 14.90 &    1.68e-09 $ \pm $    5.42e-11 \\ 
v & 55839.6121 & 11.27 $ \pm $ 0.04 & 13.79 & 446.84 $ \pm $ 14.48 &    1.63e-09 $ \pm $    5.27e-11 \\ 
v & 55840.2128 & 11.30 $ \pm $ 0.04 & 13.83 & 430.67 $ \pm $ 14.02 &    1.57e-09 $ \pm $    5.10e-11 \\ 
v & 55840.3511 & 11.31 $ \pm $ 0.04 & 13.83 & 429.07 $ \pm $ 13.98 &    1.56e-09 $ \pm $    5.08e-11 \\ 
v & 55841.3453 & 11.39 $ \pm $ 0.04 & 13.92 & 399.72 $ \pm $ 12.86 &    1.45e-09 $ \pm $    4.67e-11 \\ 
v & 55841.8874 & 11.38 $ \pm $ 0.04 & 13.90 & 400.50 $ \pm $ 13.12 &    1.46e-09 $ \pm $    4.77e-11 \\ 
v & 55842.3527 & 11.43 $ \pm $ 0.04 & 13.96 & 385.27 $ \pm $ 12.50 &    1.40e-09 $ \pm $    4.54e-11 \\ 
v & 55842.8915 & 11.44 $ \pm $ 0.04 & 13.96 & 379.46 $ \pm $ 12.41 &    1.38e-09 $ \pm $    4.51e-11 \\ 
v & 55843.4860 & 11.51 $ \pm $ 0.04 & 14.05 & 357.00 $ \pm $ 11.48 &    1.30e-09 $ \pm $    4.17e-11 \\ 
v & 55843.7502 & 11.51 $ \pm $ 0.04 & 14.04 & 357.77 $ \pm $ 11.59 &    1.30e-09 $ \pm $    4.21e-11 \\ 
v & 55844.0190 & 11.53 $ \pm $ 0.04 & 14.05 & 351.44 $ \pm $ 11.40 &    1.28e-09 $ \pm $    4.14e-11 \\ 
v & 55844.0855 & 11.55 $ \pm $ 0.04 & 14.08 & 343.43 $ \pm $ 11.13 &    1.25e-09 $ \pm $    4.04e-11 \\ 
v & 55845.4229 & 11.63 $ \pm $ 0.04 & 14.16 & 319.59 $ \pm $ 10.35 &    1.16e-09 $ \pm $    3.76e-11 \\ 
v & 55845.4890 & 11.62 $ \pm $ 0.04 & 14.15 & 322.24 $ \pm $ 10.46 &    1.17e-09 $ \pm $    3.80e-11 \\ 
v & 55846.7014 & 11.71 $ \pm $ 0.04 & 14.24 & 296.84 $ \pm $  9.60 &    1.08e-09 $ \pm $    3.49e-11 \\ 
v & 55847.4376 & 11.76 $ \pm $ 0.04 & 14.30 & 281.99 $ \pm $  9.13 &    1.02e-09 $ \pm $    3.32e-11 \\ 
v & 55848.5118 & 11.90 $ \pm $ 0.04 & 14.38 & 249.81 $ \pm $  8.42 &    9.08e-10 $ \pm $    3.06e-11 \\ 
v & 55848.5164 & 11.85 $ \pm $ 0.04 & 14.38 & 260.61 $ \pm $  8.41 &    9.47e-10 $ \pm $    3.06e-11 \\ 
v & 55849.5119 & 11.94 $ \pm $ 0.04 & 14.48 & 239.57 $ \pm $  7.74 &    8.71e-10 $ \pm $    2.81e-11 \\ 
v & 55851.6590 & 12.00 $ \pm $ 0.04 & 14.47 & 227.17 $ \pm $  7.76 &    8.26e-10 $ \pm $    2.82e-11 \\ 
v & 55851.6609 & 12.01 $ \pm $ 0.04 & 14.54 & 225.36 $ \pm $  7.32 &    8.19e-10 $ \pm $    2.66e-11 \\ 
v & 55852.2417 & 12.07 $ \pm $ 0.04 & 14.53 & 213.32 $ \pm $  7.33 &    7.76e-10 $ \pm $    2.67e-11 \\ 
v & 55852.2429 & 12.02 $ \pm $ 0.04 & 14.55 & 223.11 $ \pm $  7.24 &    8.11e-10 $ \pm $    2.63e-11 \\ 
v & 55852.3234 & 12.04 $ \pm $ 0.04 & 14.57 & 218.35 $ \pm $  7.09 &    7.94e-10 $ \pm $    2.58e-11 \\ 
v & 55853.3119 & 12.07 $ \pm $ 0.04 & 14.53 & 212.70 $ \pm $  7.35 &    7.73e-10 $ \pm $    2.67e-11 \\ 
v & 55853.3140 & 12.06 $ \pm $ 0.04 & 14.58 & 215.56 $ \pm $  7.00 &    7.84e-10 $ \pm $    2.54e-11 \\ 
v & 55853.7188 & 12.12 $ \pm $ 0.04 & 14.65 & 202.43 $ \pm $  6.61 &    7.36e-10 $ \pm $    2.40e-11 \\ 
v & 55854.8593 & 12.14 $ \pm $ 0.04 & 14.66 & 199.77 $ \pm $  6.54 &    7.26e-10 $ \pm $    2.38e-11 \\ 
v & 55855.5873 & 12.18 $ \pm $ 0.04 & 14.70 & 192.88 $ \pm $  6.29 &    7.01e-10 $ \pm $    2.29e-11 \\ 
v & 55855.6574 & 12.16 $ \pm $ 0.04 & 14.68 & 196.04 $ \pm $  6.39 &    7.13e-10 $ \pm $    2.32e-11 \\ 
v & 55856.3898 & 12.20 $ \pm $ 0.04 & 14.71 & 188.87 $ \pm $  6.21 &    6.87e-10 $ \pm $    2.26e-11 \\ 
v & 55856.4565 & 12.24 $ \pm $ 0.04 & 14.75 & 181.86 $ \pm $  6.00 &    6.62e-10 $ \pm $    2.18e-11 \\ 
v & 55857.4606 & 12.23 $ \pm $ 0.04 & 14.74 & 184.05 $ \pm $  6.05 &    6.69e-10 $ \pm $    2.20e-11 \\ 
v & 55857.5222 & 12.30 $ \pm $ 0.04 & 14.78 & 171.83 $ \pm $  5.82 &    6.25e-10 $ \pm $    2.12e-11 \\ 
v & 55857.5286 & 12.25 $ \pm $ 0.04 & 14.68 & 180.54 $ \pm $  6.42 &    6.57e-10 $ \pm $    2.33e-11 \\ 
v & 55857.5311 & 12.25 $ \pm $ 0.04 & 14.78 & 180.18 $ \pm $  5.86 &    6.55e-10 $ \pm $    2.13e-11 \\ 
v & 55858.5251 & 12.30 $ \pm $ 0.04 & 14.78 & 172.20 $ \pm $  5.83 &    6.27e-10 $ \pm $    2.12e-11 \\ 
v & 55859.5343 & 12.27 $ \pm $ 0.04 & 14.78 & 176.98 $ \pm $  5.85 &    6.44e-10 $ \pm $    2.13e-11 \\ 
v & 55860.0070 & 12.29 $ \pm $ 0.04 & 14.80 & 173.87 $ \pm $  5.76 &    6.33e-10 $ \pm $    2.10e-11 \\ 
v & 55860.0641 & 12.31 $ \pm $ 0.04 & 14.80 & 170.78 $ \pm $  5.76 &    6.22e-10 $ \pm $    2.10e-11 \\ 
v & 55860.0716 & 12.33 $ \pm $ 0.04 & 14.74 & 166.83 $ \pm $  6.04 &    6.07e-10 $ \pm $    2.20e-11 \\ 
v & 55860.0734 & 12.30 $ \pm $ 0.04 & 14.83 & 171.46 $ \pm $  5.60 &    6.24e-10 $ \pm $    2.04e-11 \\ 
v & 55861.1390 & 12.41 $ \pm $ 0.04 & 14.93 & 154.86 $ \pm $  5.08 &    5.64e-10 $ \pm $    1.85e-11 \\ 
v & 55861.6025 & 12.36 $ \pm $ 0.04 & 14.77 & 163.25 $ \pm $  5.90 &    5.95e-10 $ \pm $    2.15e-11 \\ 
v & 55861.6035 & 12.34 $ \pm $ 0.04 & 14.85 & 166.43 $ \pm $  5.48 &    6.06e-10 $ \pm $    2.00e-11 \\ 
v & 55862.2753 & 12.40 $ \pm $ 0.04 & 14.91 & 157.62 $ \pm $  5.16 &    5.74e-10 $ \pm $    1.88e-11 \\ 
v & 55862.7379 & 12.36 $ \pm $ 0.04 & 14.77 & 163.62 $ \pm $  5.91 &    5.96e-10 $ \pm $    2.15e-11 \\ 
v & 55862.7395 & 12.37 $ \pm $ 0.04 & 14.90 & 161.14 $ \pm $  5.25 &    5.87e-10 $ \pm $    1.91e-11 \\ 
v & 55863.0110 & 12.44 $ \pm $ 0.04 & 14.95 & 151.28 $ \pm $  4.98 &    5.51e-10 $ \pm $    1.81e-11 \\ 
v & 55864.1426 & 12.53 $ \pm $ 0.04 & 14.89 & 139.58 $ \pm $  5.27 &    5.09e-10 $ \pm $    1.92e-11 \\ 
v & 55864.1440 & 12.42 $ \pm $ 0.04 & 14.94 & 153.75 $ \pm $  5.06 &    5.60e-10 $ \pm $    1.84e-11 \\ 
v & 55864.8850 & 12.47 $ \pm $ 0.04 & 14.98 & 147.02 $ \pm $  4.85 &    5.36e-10 $ \pm $    1.77e-11 \\ 
v & 55865.0116 & 12.48 $ \pm $ 0.04 & 14.86 & 145.62 $ \pm $  5.41 &    5.31e-10 $ \pm $    1.97e-11 \\ 
v & 55865.0132 & 12.44 $ \pm $ 0.04 & 14.96 & 150.82 $ \pm $  4.93 &    5.50e-10 $ \pm $    1.80e-11 \\ 
v & 55865.2183 & 12.50 $ \pm $ 0.04 & 15.01 & 143.53 $ \pm $  4.75 &    5.23e-10 $ \pm $    1.73e-11 \\ 
v & 55866.6170 & 12.46 $ \pm $ 0.04 & 14.85 & 149.12 $ \pm $  5.51 &    5.43e-10 $ \pm $    2.01e-11 \\ 
v & 55866.6187 & 12.49 $ \pm $ 0.04 & 15.01 & 144.54 $ \pm $  4.72 &    5.27e-10 $ \pm $    1.72e-11 \\ 
v & 55866.8907 & 12.52 $ \pm $ 0.04 & 15.04 & 140.10 $ \pm $  4.61 &    5.11e-10 $ \pm $    1.68e-11 \\ 
v & 55867.2191 & 12.58 $ \pm $ 0.04 & 14.94 & 133.29 $ \pm $  5.07 &    4.86e-10 $ \pm $    1.85e-11 \\ 
v & 55867.2208 & 12.52 $ \pm $ 0.04 & 15.04 & 140.74 $ \pm $  4.61 &    5.13e-10 $ \pm $    1.68e-11 \\ 
v & 55867.3589 & 12.53 $ \pm $ 0.04 & 15.00 & 139.87 $ \pm $  4.77 &    5.10e-10 $ \pm $    1.74e-11 \\ 
v & 55867.9613 & 12.54 $ \pm $ 0.04 & 15.03 & 138.02 $ \pm $  4.63 &    5.04e-10 $ \pm $    1.69e-11 \\ 
v & 55868.0228 & 12.56 $ \pm $ 0.04 & 14.93 & 135.77 $ \pm $  5.11 &    4.95e-10 $ \pm $    1.86e-11 \\ 
v & 55868.0240 & 12.55 $ \pm $ 0.04 & 15.06 & 137.20 $ \pm $  4.50 &    5.01e-10 $ \pm $    1.64e-11 \\ 
v & 55868.0956 & 12.57 $ \pm $ 0.04 & 15.07 & 134.43 $ \pm $  4.49 &    4.90e-10 $ \pm $    1.64e-11 \\ 
v & 55868.4904 & 12.57 $ \pm $ 0.04 & 15.03 & 134.50 $ \pm $  4.63 &    4.91e-10 $ \pm $    1.69e-11 \\ 
v & 55869.0262 & 12.61 $ \pm $ 0.04 & 14.95 & 130.03 $ \pm $  5.00 &    4.75e-10 $ \pm $    1.83e-11 \\ 
v & 55869.0275 & 12.58 $ \pm $ 0.04 & 15.08 & 132.98 $ \pm $  4.43 &    4.85e-10 $ \pm $    1.62e-11 \\ 
v & 55869.1649 & 12.60 $ \pm $ 0.04 & 15.10 & 131.03 $ \pm $  4.36 &    4.78e-10 $ \pm $    1.59e-11 \\ 
v & 55873.1170 & 12.67 $ \pm $ 0.04 & 15.16 & 122.54 $ \pm $  4.13 &    4.48e-10 $ \pm $    1.51e-11 \\ 
v & 55875.7238 & 12.67 $ \pm $ 0.04 & 15.12 & 122.50 $ \pm $  4.29 &    4.48e-10 $ \pm $    1.57e-11 \\ 
v & 55877.9408 & 12.84 $ \pm $ 0.04 & 15.31 & 104.97 $ \pm $  3.57 &    3.84e-10 $ \pm $    1.31e-11 \\ 
v & 55879.2084 & 12.87 $ \pm $ 0.04 & 15.34 & 101.68 $ \pm $  3.50 &    3.72e-10 $ \pm $    1.28e-11 \\ 
v & 55881.9555 & 12.94 $ \pm $ 0.04 & 15.40 &  95.35 $ \pm $  3.29 &    3.49e-10 $ \pm $    1.21e-11 \\ 
v & 55885.9020 & 13.03 $ \pm $ 0.04 & 15.49 &  88.07 $ \pm $  3.03 &    3.23e-10 $ \pm $    1.11e-11 \\ 
v & 55887.3093 & 13.09 $ \pm $ 0.04 & 15.54 &  83.08 $ \pm $  2.89 &    3.05e-10 $ \pm $    1.06e-11 \\ 
v & 55889.7843 & 13.10 $ \pm $ 0.04 & 15.56 &  82.46 $ \pm $  2.85 &    3.02e-10 $ \pm $    1.04e-11 \\ 
v & 55891.8427 & 13.20 $ \pm $ 0.04 & 15.65 &  75.24 $ \pm $  2.62 &    2.76e-10 $ \pm $    9.62e-12 \\ 
v & 55893.9149 & 13.25 $ \pm $ 0.04 & 15.70 &  71.57 $ \pm $  2.50 &    2.62e-10 $ \pm $    9.18e-12 \\ 
v & 55895.9195 & 13.27 $ \pm $ 0.04 & 15.71 &  70.35 $ \pm $  2.47 &    2.58e-10 $ \pm $    9.07e-12 \\ 
v & 55897.4641 & 13.33 $ \pm $ 0.04 & 15.71 &  66.41 $ \pm $  2.48 &    2.43e-10 $ \pm $    9.07e-12 \\ 
v & 55899.6657 & 13.34 $ \pm $ 0.04 & 15.78 &  66.34 $ \pm $  2.34 &    2.43e-10 $ \pm $    8.57e-12 \\ 
v & 55901.5399 & 13.45 $ \pm $ 0.04 & 15.87 &  59.60 $ \pm $  2.13 &    2.19e-10 $ \pm $    7.83e-12 \\ 
v & 55903.7387 & 13.50 $ \pm $ 0.04 & 15.91 &  57.19 $ \pm $  2.06 &    2.10e-10 $ \pm $    7.55e-12 \\ 
v & 55905.0753 & 13.53 $ \pm $ 0.04 & 15.95 &  55.60 $ \pm $  2.00 &    2.04e-10 $ \pm $    7.32e-12 \\ 
v & 55909.9551 & 13.61 $ \pm $ 0.04 & 16.02 &  51.57 $ \pm $  1.87 &    1.89e-10 $ \pm $    6.86e-12 \\ 
v & 55913.8987 & 13.66 $ \pm $ 0.04 & 16.06 &  49.33 $ \pm $  1.80 &    1.81e-10 $ \pm $    6.61e-12 \\ 


==> tab2.tex <==
uvw2 &  -15.0 &  5.875 \\
uvw2 &  -14.9 &  5.793 \\
uvw2 &  -14.8 &  5.712 \\
uvw2 &  -14.7 &  5.632 \\
uvw2 &  -14.6 &  5.553 \\
uvw2 &  -14.5 &  5.474 \\
uvw2 &  -14.4 &  5.397 \\
uvw2 &  -14.3 &  5.320 \\
uvw2 &  -14.2 &  5.244 \\
uvw2 &  -14.1 &  5.169 \\
uvw2 &  -14.0 &  5.094 \\
uvw2 &  -13.9 &  5.019 \\
uvw2 &  -13.8 &  4.945 \\
uvw2 &  -13.7 &  4.872 \\
uvw2 &  -13.6 &  4.799 \\
uvw2 &  -13.5 &  4.726 \\
uvw2 &  -13.4 &  4.654 \\
uvw2 &  -13.3 &  4.582 \\
uvw2 &  -13.2 &  4.510 \\
uvw2 &  -13.1 &  4.438 \\
uvw2 &  -13.0 &  4.367 \\
uvw2 &  -12.9 &  4.296 \\
uvw2 &  -12.8 &  4.225 \\
uvw2 &  -12.7 &  4.155 \\
uvw2 &  -12.6 &  4.084 \\
uvw2 &  -12.5 &  4.014 \\
uvw2 &  -12.4 &  3.944 \\
uvw2 &  -12.3 &  3.874 \\
uvw2 &  -12.2 &  3.805 \\
uvw2 &  -12.1 &  3.736 \\
uvw2 &  -12.0 &  3.667 \\
uvw2 &  -11.9 &  3.598 \\
uvw2 &  -11.8 &  3.529 \\
uvw2 &  -11.7 &  3.461 \\
uvw2 &  -11.6 &  3.393 \\
uvw2 &  -11.5 &  3.325 \\
uvw2 &  -11.4 &  3.258 \\
uvw2 &  -11.3 &  3.191 \\
uvw2 &  -11.2 &  3.124 \\
uvw2 &  -11.1 &  3.058 \\
uvw2 &  -11.0 &  2.992 \\
uvw2 &  -10.9 &  2.926 \\
uvw2 &  -10.8 &  2.861 \\
uvw2 &  -10.7 &  2.796 \\
uvw2 &  -10.6 &  2.732 \\
uvw2 &  -10.5 &  2.668 \\
uvw2 &  -10.4 &  2.605 \\
uvw2 &  -10.3 &  2.542 \\
uvw2 &  -10.2 &  2.479 \\
uvw2 &  -10.1 &  2.418 \\
uvw2 &  -10.0 &  2.357 \\
uvw2 &   -9.9 &  2.296 \\
uvw2 &   -9.8 &  2.236 \\
uvw2 &   -9.7 &  2.177 \\
uvw2 &   -9.6 &  2.118 \\
uvw2 &   -9.5 &  2.061 \\
uvw2 &   -9.4 &  2.003 \\
uvw2 &   -9.3 &  1.947 \\
uvw2 &   -9.2 &  1.891 \\
uvw2 &   -9.1 &  1.836 \\
uvw2 &   -9.0 &  1.782 \\
uvw2 &   -8.9 &  1.729 \\
uvw2 &   -8.8 &  1.676 \\
uvw2 &   -8.7 &  1.625 \\
uvw2 &   -8.6 &  1.574 \\
uvw2 &   -8.5 &  1.524 \\
uvw2 &   -8.4 &  1.475 \\
uvw2 &   -8.3 &  1.427 \\
uvw2 &   -8.2 &  1.380 \\
uvw2 &   -8.1 &  1.333 \\
uvw2 &   -8.0 &  1.288 \\
uvw2 &   -7.9 &  1.244 \\
uvw2 &   -7.8 &  1.200 \\
uvw2 &   -7.7 &  1.158 \\
uvw2 &   -7.6 &  1.116 \\
uvw2 &   -7.5 &  1.076 \\
uvw2 &   -7.4 &  1.036 \\
uvw2 &   -7.3 &  0.997 \\
uvw2 &   -7.2 &  0.960 \\
uvw2 &   -7.1 &  0.923 \\
uvw2 &   -7.0 &  0.887 \\
uvw2 &   -6.9 &  0.853 \\
uvw2 &   -6.8 &  0.819 \\
uvw2 &   -6.7 &  0.786 \\
uvw2 &   -6.6 &  0.755 \\
uvw2 &   -6.5 &  0.724 \\
uvw2 &   -6.4 &  0.694 \\
uvw2 &   -6.3 &  0.665 \\
uvw2 &   -6.2 &  0.637 \\
uvw2 &   -6.1 &  0.610 \\
uvw2 &   -6.0 &  0.584 \\
uvw2 &   -5.9 &  0.559 \\
uvw2 &   -5.8 &  0.534 \\
uvw2 &   -5.7 &  0.511 \\
uvw2 &   -5.6 &  0.488 \\
uvw2 &   -5.5 &  0.467 \\
uvw2 &   -5.4 &  0.446 \\
uvw2 &   -5.3 &  0.426 \\
uvw2 &   -5.2 &  0.406 \\
uvw2 &   -5.1 &  0.388 \\
uvw2 &   -5.0 &  0.370 \\
uvw2 &   -4.9 &  0.353 \\
uvw2 &   -4.8 &  0.337 \\
uvw2 &   -4.7 &  0.321 \\
uvw2 &   -4.6 &  0.306 \\
uvw2 &   -4.5 &  0.292 \\
uvw2 &   -4.4 &  0.278 \\
uvw2 &   -4.3 &  0.265 \\
uvw2 &   -4.2 &  0.253 \\
uvw2 &   -4.1 &  0.241 \\
uvw2 &   -4.0 &  0.230 \\
uvw2 &   -3.9 &  0.219 \\
uvw2 &   -3.8 &  0.209 \\
uvw2 &   -3.7 &  0.199 \\
uvw2 &   -3.6 &  0.189 \\
uvw2 &   -3.5 &  0.180 \\
uvw2 &   -3.4 &  0.171 \\
uvw2 &   -3.3 &  0.163 \\
uvw2 &   -3.2 &  0.155 \\
uvw2 &   -3.1 &  0.145 \\
uvw2 &   -3.0 &  0.132 \\
uvw2 &   -2.9 &  0.123 \\
uvw2 &   -2.8 &  0.114 \\
uvw2 &   -2.7 &  0.106 \\
uvw2 &   -2.6 &  0.098 \\
uvw2 &   -2.5 &  0.090 \\
uvw2 &   -2.4 &  0.083 \\
uvw2 &   -2.3 &  0.076 \\
uvw2 &   -2.2 &  0.069 \\
uvw2 &   -2.1 &  0.062 \\
uvw2 &   -2.0 &  0.056 \\
uvw2 &   -1.9 &  0.051 \\
uvw2 &   -1.8 &  0.045 \\
uvw2 &   -1.7 &  0.040 \\
uvw2 &   -1.6 &  0.036 \\
uvw2 &   -1.5 &  0.031 \\
uvw2 &   -1.4 &  0.027 \\
uvw2 &   -1.3 &  0.023 \\
uvw2 &   -1.2 &  0.020 \\
uvw2 &   -1.1 &  0.017 \\
uvw2 &   -1.0 &  0.014 \\
uvw2 &   -0.9 &  0.011 \\
uvw2 &   -0.8 &  0.009 \\
uvw2 &   -0.7 &  0.007 \\
uvw2 &   -0.6 &  0.005 \\
uvw2 &   -0.5 &  0.003 \\
uvw2 &   -0.4 &  0.002 \\
uvw2 &   -0.3 &  0.001 \\
uvw2 &   -0.2 &  0.001 \\
uvw2 &   -0.1 &  0.000 \\
uvw2 &    0.0 &  0.000 \\
uvw2 &    0.1 &  0.000 \\
uvw2 &    0.2 &  0.001 \\
uvw2 &    0.3 &  0.001 \\
uvw2 &    0.4 &  0.002 \\
uvw2 &    0.5 &  0.003 \\
uvw2 &    0.6 &  0.005 \\
uvw2 &    0.7 &  0.006 \\
uvw2 &    0.8 &  0.008 \\
uvw2 &    0.9 &  0.010 \\
uvw2 &    1.0 &  0.013 \\
uvw2 &    1.1 &  0.015 \\
uvw2 &    1.2 &  0.018 \\
uvw2 &    1.3 &  0.021 \\
uvw2 &    1.4 &  0.024 \\
uvw2 &    1.5 &  0.027 \\
uvw2 &    1.6 &  0.031 \\
uvw2 &    1.7 &  0.035 \\
uvw2 &    1.8 &  0.039 \\
uvw2 &    1.9 &  0.043 \\
uvw2 &    2.0 &  0.047 \\
uvw2 &    2.0 &  0.047 \\
uvw2 &    2.1 &  0.052 \\
uvw2 &    2.2 &  0.057 \\
uvw2 &    2.3 &  0.062 \\
uvw2 &    2.4 &  0.068 \\
uvw2 &    2.5 &  0.074 \\
uvw2 &    2.6 &  0.080 \\
uvw2 &    2.7 &  0.086 \\
uvw2 &    2.8 &  0.092 \\
uvw2 &    2.9 &  0.099 \\
uvw2 &    3.0 &  0.106 \\
uvw2 &    3.1 &  0.113 \\
uvw2 &    3.2 &  0.120 \\
uvw2 &    3.3 &  0.127 \\
uvw2 &    3.4 &  0.135 \\
uvw2 &    3.5 &  0.142 \\
uvw2 &    3.6 &  0.150 \\
uvw2 &    3.7 &  0.158 \\
uvw2 &    3.8 &  0.166 \\
uvw2 &    3.9 &  0.174 \\
uvw2 &    4.0 &  0.183 \\
uvw2 &    4.1 &  0.192 \\
uvw2 &    4.2 &  0.200 \\
uvw2 &    4.3 &  0.209 \\
uvw2 &    4.4 &  0.218 \\
uvw2 &    4.5 &  0.227 \\
uvw2 &    4.6 &  0.237 \\
uvw2 &    4.7 &  0.246 \\
uvw2 &    4.8 &  0.256 \\
uvw2 &    4.9 &  0.265 \\
uvw2 &    5.0 &  0.275 \\
uvw2 &    5.1 &  0.285 \\
uvw2 &    5.2 &  0.295 \\
uvw2 &    5.3 &  0.305 \\
uvw2 &    5.4 &  0.315 \\
uvw2 &    5.5 &  0.326 \\
uvw2 &    5.6 &  0.336 \\
uvw2 &    5.7 &  0.347 \\
uvw2 &    5.8 &  0.358 \\
uvw2 &    5.9 &  0.368 \\
uvw2 &    6.0 &  0.379 \\
uvw2 &    6.1 &  0.390 \\
uvw2 &    6.2 &  0.401 \\
uvw2 &    6.3 &  0.413 \\
uvw2 &    6.4 &  0.424 \\
uvw2 &    6.5 &  0.435 \\
uvw2 &    6.6 &  0.447 \\
uvw2 &    6.7 &  0.458 \\
uvw2 &    6.8 &  0.470 \\
uvw2 &    6.9 &  0.482 \\
uvw2 &    7.0 &  0.493 \\
uvw2 &    7.1 &  0.505 \\
uvw2 &    7.2 &  0.517 \\
uvw2 &    7.3 &  0.529 \\
uvw2 &    7.4 &  0.541 \\
uvw2 &    7.5 &  0.553 \\
uvw2 &    7.6 &  0.565 \\
uvw2 &    7.7 &  0.578 \\
uvw2 &    7.8 &  0.590 \\
uvw2 &    7.9 &  0.602 \\
uvw2 &    8.0 &  0.615 \\
uvw2 &    8.1 &  0.627 \\
uvw2 &    8.2 &  0.640 \\
uvw2 &    8.3 &  0.652 \\
uvw2 &    8.4 &  0.665 \\
uvw2 &    8.5 &  0.677 \\
uvw2 &    8.6 &  0.690 \\
uvw2 &    8.7 &  0.703 \\
uvw2 &    8.8 &  0.716 \\
uvw2 &    8.9 &  0.728 \\
uvw2 &    9.0 &  0.741 \\
uvw2 &    9.1 &  0.754 \\
uvw2 &    9.2 &  0.767 \\
uvw2 &    9.3 &  0.780 \\
uvw2 &    9.4 &  0.793 \\
uvw2 &    9.5 &  0.806 \\
uvw2 &    9.6 &  0.819 \\
uvw2 &    9.7 &  0.832 \\
uvw2 &    9.8 &  0.845 \\
uvw2 &    9.9 &  0.858 \\
uvw2 &   10.0 &  0.871 \\
uvw2 &   10.1 &  0.885 \\
uvw2 &   10.2 &  0.898 \\
uvw2 &   10.3 &  0.911 \\
uvw2 &   10.4 &  0.924 \\
uvw2 &   10.5 &  0.937 \\
uvw2 &   10.6 &  0.951 \\
uvw2 &   10.7 &  0.964 \\
uvw2 &   10.8 &  0.977 \\
uvw2 &   10.9 &  0.990 \\
uvw2 &   11.0 &  1.004 \\
uvw2 &   11.1 &  1.017 \\
uvw2 &   11.2 &  1.030 \\
uvw2 &   11.3 &  1.044 \\
uvw2 &   11.4 &  1.057 \\
uvw2 &   11.5 &  1.070 \\
uvw2 &   11.6 &  1.083 \\
uvw2 &   11.7 &  1.097 \\
uvw2 &   11.8 &  1.110 \\
uvw2 &   11.9 &  1.123 \\
uvw2 &   12.0 &  1.137 \\
uvw2 &   12.1 &  1.150 \\
uvw2 &   12.2 &  1.163 \\
uvw2 &   12.3 &  1.176 \\
uvw2 &   12.4 &  1.190 \\
uvw2 &   12.5 &  1.203 \\
uvw2 &   12.6 &  1.216 \\
uvw2 &   12.7 &  1.229 \\
uvw2 &   12.8 &  1.243 \\
uvw2 &   12.9 &  1.256 \\
uvw2 &   13.0 &  1.269 \\
uvw2 &   13.1 &  1.282 \\
uvw2 &   13.2 &  1.295 \\
uvw2 &   13.3 &  1.308 \\
uvw2 &   13.4 &  1.322 \\
uvw2 &   13.5 &  1.335 \\
uvw2 &   13.6 &  1.348 \\
uvw2 &   13.7 &  1.361 \\
uvw2 &   13.8 &  1.374 \\
uvw2 &   13.9 &  1.387 \\
uvw2 &   14.0 &  1.400 \\
uvw2 &   14.1 &  1.413 \\
uvw2 &   14.2 &  1.426 \\
uvw2 &   14.3 &  1.439 \\
uvw2 &   14.4 &  1.452 \\
uvw2 &   14.5 &  1.465 \\
uvw2 &   14.6 &  1.477 \\
uvw2 &   14.7 &  1.490 \\
uvw2 &   14.8 &  1.503 \\
uvw2 &   14.9 &  1.516 \\
uvw2 &   15.0 &  1.529 \\
uvw2 &   15.1 &  1.541 \\
uvw2 &   15.2 &  1.554 \\
uvw2 &   15.3 &  1.567 \\
uvw2 &   15.4 &  1.579 \\
uvw2 &   15.5 &  1.592 \\
uvw2 &   15.6 &  1.604 \\
uvw2 &   15.7 &  1.617 \\
uvw2 &   15.8 &  1.629 \\
uvw2 &   15.9 &  1.642 \\
uvw2 &   16.0 &  1.654 \\
uvw2 &   16.1 &  1.666 \\
uvw2 &   16.2 &  1.679 \\
uvw2 &   16.3 &  1.691 \\
uvw2 &   16.4 &  1.703 \\
uvw2 &   16.5 &  1.716 \\
uvw2 &   16.6 &  1.728 \\
uvw2 &   16.7 &  1.740 \\
uvw2 &   16.8 &  1.752 \\
uvw2 &   16.9 &  1.764 \\
uvw2 &   17.0 &  1.776 \\
uvw2 &   17.1 &  1.788 \\
uvw2 &   17.2 &  1.800 \\
uvw2 &   17.3 &  1.812 \\
uvw2 &   17.4 &  1.824 \\
uvw2 &   17.5 &  1.836 \\
uvw2 &   17.6 &  1.847 \\
uvw2 &   17.7 &  1.859 \\
uvw2 &   17.8 &  1.871 \\
uvw2 &   17.9 &  1.883 \\
uvw2 &   18.0 &  1.894 \\
uvw2 &   18.1 &  1.906 \\
uvw2 &   18.2 &  1.917 \\
uvw2 &   18.3 &  1.929 \\
uvw2 &   18.4 &  1.940 \\
uvw2 &   18.5 &  1.951 \\
uvw2 &   18.6 &  1.963 \\
uvw2 &   18.7 &  1.974 \\
uvw2 &   18.8 &  1.985 \\
uvw2 &   18.9 &  1.997 \\
uvw2 &   19.0 &  2.008 \\
uvw2 &   19.1 &  2.019 \\
uvw2 &   19.2 &  2.030 \\
uvw2 &   19.3 &  2.041 \\
uvw2 &   19.4 &  2.052 \\
uvw2 &   19.5 &  2.063 \\
uvw2 &   19.6 &  2.074 \\
uvw2 &   19.7 &  2.085 \\
uvw2 &   19.8 &  2.095 \\
uvw2 &   19.9 &  2.106 \\
uvw2 &   20.0 &  2.117 \\
uvw2 &   20.1 &  2.127 \\
uvw2 &   20.2 &  2.138 \\
uvw2 &   20.3 &  2.149 \\
uvw2 &   20.4 &  2.159 \\
uvw2 &   20.5 &  2.170 \\
uvw2 &   20.6 &  2.180 \\
uvw2 &   20.7 &  2.190 \\
uvw2 &   20.8 &  2.201 \\
uvw2 &   20.9 &  2.211 \\
uvw2 &   21.0 &  2.221 \\
uvw2 &   21.1 &  2.231 \\
uvw2 &   21.2 &  2.241 \\
uvw2 &   21.3 &  2.251 \\
uvw2 &   21.4 &  2.261 \\
uvw2 &   21.5 &  2.271 \\
uvw2 &   21.6 &  2.281 \\
uvw2 &   21.7 &  2.291 \\
uvw2 &   21.8 &  2.301 \\
uvw2 &   21.9 &  2.311 \\
uvw2 &   22.0 &  2.321 \\
uvw2 &   22.1 &  2.330 \\
uvw2 &   22.2 &  2.340 \\
uvw2 &   22.3 &  2.349 \\
uvw2 &   22.4 &  2.359 \\
uvw2 &   22.5 &  2.368 \\
uvw2 &   22.6 &  2.378 \\
uvw2 &   22.7 &  2.387 \\
uvw2 &   22.8 &  2.397 \\
uvw2 &   22.9 &  2.406 \\
uvw2 &   23.0 &  2.415 \\
uvw2 &   23.1 &  2.424 \\
uvw2 &   23.2 &  2.433 \\
uvw2 &   23.3 &  2.442 \\
uvw2 &   23.4 &  2.452 \\
uvw2 &   23.5 &  2.461 \\
uvw2 &   23.6 &  2.469 \\
uvw2 &   23.7 &  2.478 \\
uvw2 &   23.8 &  2.487 \\
uvw2 &   23.9 &  2.496 \\
uvw2 &   24.0 &  2.505 \\
uvw2 &   24.1 &  2.513 \\
uvw2 &   24.2 &  2.522 \\
uvw2 &   24.3 &  2.531 \\
uvw2 &   24.4 &  2.539 \\
uvw2 &   24.5 &  2.548 \\
uvw2 &   24.6 &  2.556 \\
uvw2 &   24.7 &  2.565 \\
uvw2 &   24.8 &  2.573 \\
uvw2 &   24.9 &  2.581 \\
uvw2 &   25.0 &  2.590 \\
uvw2 &   25.1 &  2.598 \\
uvw2 &   25.2 &  2.606 \\
uvw2 &   25.3 &  2.614 \\
uvw2 &   25.4 &  2.622 \\
uvw2 &   25.5 &  2.630 \\
uvw2 &   25.6 &  2.638 \\
uvw2 &   25.7 &  2.646 \\
uvw2 &   25.8 &  2.654 \\
uvw2 &   25.9 &  2.662 \\
uvw2 &   26.0 &  2.670 \\
uvw2 &   26.1 &  2.678 \\
uvw2 &   26.2 &  2.685 \\
uvw2 &   26.3 &  2.693 \\
uvw2 &   26.4 &  2.701 \\
uvw2 &   26.5 &  2.708 \\
uvw2 &   26.6 &  2.716 \\
uvw2 &   26.7 &  2.723 \\
uvw2 &   26.8 &  2.731 \\
uvw2 &   26.9 &  2.738 \\
uvw2 &   27.0 &  2.746 \\
uvw2 &   27.1 &  2.753 \\
uvw2 &   27.2 &  2.760 \\
uvw2 &   27.3 &  2.767 \\
uvw2 &   27.4 &  2.775 \\
uvw2 &   27.5 &  2.782 \\
uvw2 &   27.6 &  2.789 \\
uvw2 &   27.7 &  2.796 \\
uvw2 &   27.8 &  2.803 \\
uvw2 &   27.9 &  2.810 \\
uvw2 &   28.0 &  2.817 \\
uvw2 &   28.1 &  2.824 \\
uvw2 &   28.2 &  2.831 \\
uvw2 &   28.3 &  2.838 \\
uvw2 &   28.4 &  2.844 \\
uvw2 &   28.5 &  2.851 \\
uvw2 &   28.6 &  2.858 \\
uvw2 &   28.7 &  2.864 \\
uvw2 &   28.8 &  2.871 \\
uvw2 &   28.9 &  2.878 \\
uvw2 &   29.0 &  2.884 \\
uvw2 &   29.1 &  2.891 \\
uvw2 &   29.2 &  2.897 \\
uvw2 &   29.3 &  2.903 \\
uvw2 &   29.4 &  2.910 \\
uvw2 &   29.5 &  2.916 \\
uvw2 &   29.6 &  2.922 \\
uvw2 &   29.7 &  2.929 \\
uvw2 &   29.8 &  2.935 \\
uvw2 &   29.9 &  2.941 \\
uvw2 &   30.0 &  2.947 \\
uvw2 &   30.1 &  2.953 \\
uvw2 &   30.2 &  2.959 \\
uvw2 &   30.3 &  2.965 \\
uvw2 &   30.4 &  2.971 \\
uvw2 &   30.5 &  2.977 \\
uvw2 &   30.6 &  2.983 \\
uvw2 &   30.7 &  2.989 \\
uvw2 &   30.8 &  2.995 \\
uvw2 &   30.9 &  3.001 \\
uvw2 &   31.0 &  3.007 \\
uvw2 &   31.1 &  3.012 \\
uvw2 &   31.2 &  3.018 \\
uvw2 &   31.3 &  3.024 \\
uvw2 &   31.4 &  3.029 \\
uvw2 &   31.5 &  3.035 \\
uvw2 &   31.6 &  3.040 \\
uvw2 &   31.7 &  3.046 \\
uvw2 &   31.8 &  3.051 \\
uvw2 &   31.9 &  3.057 \\
uvw2 &   32.0 &  3.062 \\
uvw2 &   32.1 &  3.068 \\
uvw2 &   32.2 &  3.073 \\
uvw2 &   32.3 &  3.078 \\
uvw2 &   32.4 &  3.084 \\
uvw2 &   32.5 &  3.089 \\
uvw2 &   32.6 &  3.094 \\
uvw2 &   32.7 &  3.099 \\
uvw2 &   32.8 &  3.105 \\
uvw2 &   32.9 &  3.110 \\
uvw2 &   33.0 &  3.115 \\
uvw2 &   33.1 &  3.120 \\
uvw2 &   33.2 &  3.125 \\
uvw2 &   33.3 &  3.130 \\
uvw2 &   33.4 &  3.135 \\
uvw2 &   33.5 &  3.140 \\
uvw2 &   33.6 &  3.145 \\
uvw2 &   33.7 &  3.150 \\
uvw2 &   33.8 &  3.154 \\
uvw2 &   33.9 &  3.159 \\
uvw2 &   34.0 &  3.164 \\
uvw2 &   34.1 &  3.169 \\
uvw2 &   34.2 &  3.173 \\
uvw2 &   34.3 &  3.178 \\
uvw2 &   34.4 &  3.183 \\
uvw2 &   34.5 &  3.188 \\
uvw2 &   34.6 &  3.192 \\
uvw2 &   34.7 &  3.197 \\
uvw2 &   34.8 &  3.201 \\
uvw2 &   34.9 &  3.206 \\
uvw2 &   35.0 &  3.210 \\
uvw2 &   35.1 &  3.215 \\
uvw2 &   35.2 &  3.219 \\
uvw2 &   35.3 &  3.224 \\
uvw2 &   35.4 &  3.228 \\
uvw2 &   35.5 &  3.232 \\
uvw2 &   35.6 &  3.237 \\
uvw2 &   35.7 &  3.241 \\
uvw2 &   35.8 &  3.245 \\
uvw2 &   35.9 &  3.250 \\
uvw2 &   36.0 &  3.254 \\
uvw2 &   36.1 &  3.258 \\
uvw2 &   36.2 &  3.262 \\
uvw2 &   36.3 &  3.266 \\
uvw2 &   36.4 &  3.271 \\
uvw2 &   36.5 &  3.275 \\
uvw2 &   36.6 &  3.279 \\
uvw2 &   36.7 &  3.283 \\
uvw2 &   36.8 &  3.287 \\
uvw2 &   36.9 &  3.291 \\
uvw2 &   37.0 &  3.295 \\
uvw2 &   37.1 &  3.299 \\
uvw2 &   37.2 &  3.303 \\
uvw2 &   37.3 &  3.307 \\
uvw2 &   37.4 &  3.311 \\
uvw2 &   37.5 &  3.315 \\
uvw2 &   37.6 &  3.318 \\
uvw2 &   37.7 &  3.322 \\
uvw2 &   37.8 &  3.326 \\
uvw2 &   37.9 &  3.330 \\
uvw2 &   38.0 &  3.334 \\
uvw2 &   38.1 &  3.337 \\
uvw2 &   38.2 &  3.341 \\
uvw2 &   38.3 &  3.345 \\
uvw2 &   38.4 &  3.349 \\
uvw2 &   38.5 &  3.352 \\
uvw2 &   38.6 &  3.356 \\
uvw2 &   38.7 &  3.359 \\
uvw2 &   38.8 &  3.363 \\
uvw2 &   38.9 &  3.367 \\
uvw2 &   39.0 &  3.370 \\
uvw2 &   39.1 &  3.374 \\
uvw2 &   39.2 &  3.377 \\
uvw2 &   39.3 &  3.381 \\
uvw2 &   39.4 &  3.384 \\
uvw2 &   39.5 &  3.388 \\
uvw2 &   39.6 &  3.391 \\
uvw2 &   39.7 &  3.395 \\
uvw2 &   39.8 &  3.398 \\
uvw2 &   39.9 &  3.402 \\
uvw2 &   40.0 &  3.405 \\
uvw2 &   40.1 &  3.408 \\
uvw2 &   40.2 &  3.412 \\
uvw2 &   40.3 &  3.415 \\
uvw2 &   40.4 &  3.418 \\
uvw2 &   40.5 &  3.422 \\
uvw2 &   40.6 &  3.425 \\
uvw2 &   40.7 &  3.428 \\
uvw2 &   40.8 &  3.431 \\
uvw2 &   40.9 &  3.435 \\
uvw2 &   41.0 &  3.438 \\
uvw2 &   41.1 &  3.441 \\
uvw2 &   41.2 &  3.444 \\
uvw2 &   41.3 &  3.447 \\
uvw2 &   41.4 &  3.451 \\
uvw2 &   41.5 &  3.454 \\
uvw2 &   41.6 &  3.457 \\
uvw2 &   41.7 &  3.460 \\
uvw2 &   41.8 &  3.463 \\
uvw2 &   41.9 &  3.466 \\
uvw2 &   42.0 &  3.469 \\
uvw2 &   42.1 &  3.472 \\
uvw2 &   42.2 &  3.475 \\
uvw2 &   42.3 &  3.479 \\
uvw2 &   42.4 &  3.482 \\
uvw2 &   42.5 &  3.485 \\
uvw2 &   42.6 &  3.488 \\
uvw2 &   42.7 &  3.491 \\
uvw2 &   42.8 &  3.494 \\
uvw2 &   42.9 &  3.497 \\
uvw2 &   43.0 &  3.499 \\
uvw2 &   43.1 &  3.502 \\
uvw2 &   43.2 &  3.505 \\
uvw2 &   43.3 &  3.508 \\
uvw2 &   43.4 &  3.511 \\
uvw2 &   43.5 &  3.514 \\
uvw2 &   43.6 &  3.517 \\
uvw2 &   43.7 &  3.520 \\
uvw2 &   43.8 &  3.523 \\
uvw2 &   43.9 &  3.526 \\
uvw2 &   44.0 &  3.529 \\
uvw2 &   44.1 &  3.531 \\
uvw2 &   44.2 &  3.534 \\
uvw2 &   44.3 &  3.537 \\
uvw2 &   44.4 &  3.540 \\
uvw2 &   44.5 &  3.543 \\
uvw2 &   44.6 &  3.546 \\
uvw2 &   44.7 &  3.548 \\
uvw2 &   44.8 &  3.551 \\
uvw2 &   44.9 &  3.554 \\
uvw2 &   45.0 &  3.557 \\
uvw2 &   45.1 &  3.560 \\
uvw2 &   45.2 &  3.563 \\
uvw2 &   45.3 &  3.565 \\
uvw2 &   45.4 &  3.568 \\
uvw2 &   45.5 &  3.571 \\
uvw2 &   45.6 &  3.574 \\
uvw2 &   45.7 &  3.576 \\
uvw2 &   45.8 &  3.579 \\
uvw2 &   45.9 &  3.582 \\
uvw2 &   46.0 &  3.585 \\
uvw2 &   46.1 &  3.587 \\
uvw2 &   46.2 &  3.590 \\
uvw2 &   46.3 &  3.593 \\
uvw2 &   46.4 &  3.596 \\
uvw2 &   46.5 &  3.598 \\
uvw2 &   46.6 &  3.601 \\
uvw2 &   46.7 &  3.604 \\
uvw2 &   46.8 &  3.607 \\
uvw2 &   46.9 &  3.609 \\
uvw2 &   47.0 &  3.612 \\
uvw2 &   47.1 &  3.615 \\
uvw2 &   47.2 &  3.618 \\
uvw2 &   47.3 &  3.620 \\
uvw2 &   47.4 &  3.623 \\
uvw2 &   47.5 &  3.626 \\
uvw2 &   47.6 &  3.629 \\
uvw2 &   47.7 &  3.632 \\
uvw2 &   47.8 &  3.634 \\
uvw2 &   47.9 &  3.637 \\
uvw2 &   48.0 &  3.640 \\
uvw2 &   48.1 &  3.643 \\
uvw2 &   48.2 &  3.645 \\
uvw2 &   48.3 &  3.648 \\
uvw2 &   48.4 &  3.651 \\
uvw2 &   48.5 &  3.654 \\
uvw2 &   48.6 &  3.657 \\
uvw2 &   48.7 &  3.659 \\
uvw2 &   48.8 &  3.662 \\
uvw2 &   48.9 &  3.665 \\
uvw2 &   49.0 &  3.668 \\
uvw2 &   49.1 &  3.671 \\
uvw2 &   49.2 &  3.674 \\
uvw2 &   49.3 &  3.677 \\
uvw2 &   49.4 &  3.679 \\
uvw2 &   49.5 &  3.682 \\
uvw2 &   49.6 &  3.685 \\
uvw2 &   49.7 &  3.688 \\
uvw2 &   49.8 &  3.691 \\
uvw2 &   49.9 &  3.694 \\
uvw2 &   50.0 &  3.697 \\
uvm2 &  -15.0 &  5.819 \\
uvm2 &  -14.9 &  5.768 \\
uvm2 &  -14.8 &  5.716 \\
uvm2 &  -14.7 &  5.662 \\
uvm2 &  -14.6 &  5.607 \\
uvm2 &  -14.5 &  5.550 \\
uvm2 &  -14.4 &  5.492 \\
uvm2 &  -14.3 &  5.433 \\
uvm2 &  -14.2 &  5.373 \\
uvm2 &  -14.1 &  5.311 \\
uvm2 &  -14.0 &  5.248 \\
uvm2 &  -13.9 &  5.185 \\
uvm2 &  -13.8 &  5.120 \\
uvm2 &  -13.7 &  5.054 \\
uvm2 &  -13.6 &  4.988 \\
uvm2 &  -13.5 &  4.920 \\
uvm2 &  -13.4 &  4.852 \\
uvm2 &  -13.3 &  4.783 \\
uvm2 &  -13.2 &  4.714 \\
uvm2 &  -13.1 &  4.644 \\
uvm2 &  -13.0 &  4.573 \\
uvm2 &  -12.9 &  4.502 \\
uvm2 &  -12.8 &  4.431 \\
uvm2 &  -12.7 &  4.359 \\
uvm2 &  -12.6 &  4.287 \\
uvm2 &  -12.5 &  4.214 \\
uvm2 &  -12.4 &  4.141 \\
uvm2 &  -12.3 &  4.068 \\
uvm2 &  -12.2 &  3.995 \\
uvm2 &  -12.1 &  3.922 \\
uvm2 &  -12.0 &  3.849 \\
uvm2 &  -11.9 &  3.776 \\
uvm2 &  -11.8 &  3.703 \\
uvm2 &  -11.7 &  3.630 \\
uvm2 &  -11.6 &  3.557 \\
uvm2 &  -11.5 &  3.485 \\
uvm2 &  -11.4 &  3.412 \\
uvm2 &  -11.3 &  3.340 \\
uvm2 &  -11.2 &  3.268 \\
uvm2 &  -11.1 &  3.197 \\
uvm2 &  -11.0 &  3.126 \\
uvm2 &  -10.9 &  3.055 \\
uvm2 &  -10.8 &  2.985 \\
uvm2 &  -10.7 &  2.916 \\
uvm2 &  -10.6 &  2.847 \\
uvm2 &  -10.5 &  2.778 \\
uvm2 &  -10.4 &  2.710 \\
uvm2 &  -10.3 &  2.643 \\
uvm2 &  -10.2 &  2.576 \\
uvm2 &  -10.1 &  2.511 \\
uvm2 &  -10.0 &  2.445 \\
uvm2 &   -9.9 &  2.381 \\
uvm2 &   -9.8 &  2.317 \\
uvm2 &   -9.7 &  2.255 \\
uvm2 &   -9.6 &  2.193 \\
uvm2 &   -9.5 &  2.132 \\
uvm2 &   -9.4 &  2.071 \\
uvm2 &   -9.3 &  2.012 \\
uvm2 &   -9.2 &  1.953 \\
uvm2 &   -9.1 &  1.896 \\
uvm2 &   -9.0 &  1.839 \\
uvm2 &   -8.9 &  1.784 \\
uvm2 &   -8.8 &  1.729 \\
uvm2 &   -8.7 &  1.675 \\
uvm2 &   -8.6 &  1.622 \\
uvm2 &   -8.5 &  1.571 \\
uvm2 &   -8.4 &  1.520 \\
uvm2 &   -8.3 &  1.470 \\
uvm2 &   -8.2 &  1.422 \\
uvm2 &   -8.1 &  1.374 \\
uvm2 &   -8.0 &  1.327 \\
uvm2 &   -7.9 &  1.282 \\
uvm2 &   -7.8 &  1.237 \\
uvm2 &   -7.7 &  1.194 \\
uvm2 &   -7.6 &  1.151 \\
uvm2 &   -7.5 &  1.110 \\
uvm2 &   -7.4 &  1.069 \\
uvm2 &   -7.3 &  1.030 \\
uvm2 &   -7.2 &  0.992 \\
uvm2 &   -7.1 &  0.954 \\
uvm2 &   -7.0 &  0.918 \\
uvm2 &   -6.9 &  0.883 \\
uvm2 &   -6.8 &  0.848 \\
uvm2 &   -6.7 &  0.815 \\
uvm2 &   -6.6 &  0.783 \\
uvm2 &   -6.5 &  0.752 \\
uvm2 &   -6.4 &  0.721 \\
uvm2 &   -6.3 &  0.692 \\
uvm2 &   -6.2 &  0.663 \\
uvm2 &   -6.1 &  0.636 \\
uvm2 &   -6.0 &  0.609 \\
uvm2 &   -5.9 &  0.583 \\
uvm2 &   -5.8 &  0.558 \\
uvm2 &   -5.7 &  0.534 \\
uvm2 &   -5.6 &  0.511 \\
uvm2 &   -5.5 &  0.489 \\
uvm2 &   -5.4 &  0.467 \\
uvm2 &   -5.3 &  0.447 \\
uvm2 &   -5.2 &  0.427 \\
uvm2 &   -5.1 &  0.407 \\
uvm2 &   -5.0 &  0.389 \\
uvm2 &   -4.9 &  0.371 \\
uvm2 &   -4.8 &  0.354 \\
uvm2 &   -4.7 &  0.338 \\
uvm2 &   -4.6 &  0.322 \\
uvm2 &   -4.5 &  0.307 \\
uvm2 &   -4.4 &  0.292 \\
uvm2 &   -4.3 &  0.278 \\
uvm2 &   -4.2 &  0.265 \\
uvm2 &   -4.1 &  0.252 \\
uvm2 &   -4.0 &  0.240 \\
uvm2 &   -3.9 &  0.228 \\
uvm2 &   -3.8 &  0.217 \\
uvm2 &   -3.7 &  0.206 \\
uvm2 &   -3.6 &  0.195 \\
uvm2 &   -3.5 &  0.185 \\
uvm2 &   -3.4 &  0.176 \\
uvm2 &   -3.3 &  0.166 \\
uvm2 &   -3.3 &  0.166 \\
uvm2 &   -3.2 &  0.155 \\
uvm2 &   -3.1 &  0.145 \\
uvm2 &   -3.0 &  0.135 \\
uvm2 &   -2.9 &  0.126 \\
uvm2 &   -2.8 &  0.117 \\
uvm2 &   -2.7 &  0.108 \\
uvm2 &   -2.6 &  0.100 \\
uvm2 &   -2.5 &  0.092 \\
uvm2 &   -2.4 &  0.084 \\
uvm2 &   -2.3 &  0.077 \\
uvm2 &   -2.2 &  0.070 \\
uvm2 &   -2.1 &  0.063 \\
uvm2 &   -2.0 &  0.057 \\
uvm2 &   -1.9 &  0.051 \\
uvm2 &   -1.8 &  0.046 \\
uvm2 &   -1.7 &  0.041 \\
uvm2 &   -1.6 &  0.036 \\
uvm2 &   -1.5 &  0.031 \\
uvm2 &   -1.4 &  0.027 \\
uvm2 &   -1.3 &  0.023 \\
uvm2 &   -1.2 &  0.020 \\
uvm2 &   -1.1 &  0.017 \\
uvm2 &   -1.0 &  0.014 \\
uvm2 &   -0.9 &  0.011 \\
uvm2 &   -0.8 &  0.009 \\
uvm2 &   -0.7 &  0.007 \\
uvm2 &   -0.6 &  0.005 \\
uvm2 &   -0.5 &  0.003 \\
uvm2 &   -0.4 &  0.002 \\
uvm2 &   -0.3 &  0.001 \\
uvm2 &   -0.2 &  0.001 \\
uvm2 &   -0.1 &  0.000 \\
uvm2 &    0.0 &  0.000 \\
uvm2 &    0.1 &  0.000 \\
uvm2 &    0.2 &  0.001 \\
uvm2 &    0.3 &  0.001 \\
uvm2 &    0.4 &  0.002 \\
uvm2 &    0.5 &  0.003 \\
uvm2 &    0.6 &  0.005 \\
uvm2 &    0.7 &  0.006 \\
uvm2 &    0.8 &  0.008 \\
uvm2 &    0.9 &  0.010 \\
uvm2 &    1.0 &  0.012 \\
uvm2 &    1.1 &  0.015 \\
uvm2 &    1.2 &  0.017 \\
uvm2 &    1.3 &  0.020 \\
uvm2 &    1.4 &  0.023 \\
uvm2 &    1.5 &  0.027 \\
uvm2 &    1.6 &  0.030 \\
uvm2 &    1.7 &  0.034 \\
uvm2 &    1.8 &  0.037 \\
uvm2 &    1.9 &  0.041 \\
uvm2 &    2.0 &  0.046 \\
uvm2 &    2.1 &  0.050 \\
uvm2 &    2.2 &  0.054 \\
uvm2 &    2.3 &  0.059 \\
uvm2 &    2.4 &  0.064 \\
uvm2 &    2.5 &  0.069 \\
uvm2 &    2.6 &  0.074 \\
uvm2 &    2.7 &  0.079 \\
uvm2 &    2.8 &  0.085 \\
uvm2 &    2.9 &  0.092 \\
uvm2 &    3.0 &  0.099 \\
uvm2 &    3.1 &  0.106 \\
uvm2 &    3.2 &  0.114 \\
uvm2 &    3.3 &  0.121 \\
uvm2 &    3.4 &  0.129 \\
uvm2 &    3.5 &  0.137 \\
uvm2 &    3.6 &  0.145 \\
uvm2 &    3.7 &  0.154 \\
uvm2 &    3.8 &  0.162 \\
uvm2 &    3.9 &  0.171 \\
uvm2 &    4.0 &  0.180 \\
uvm2 &    4.1 &  0.189 \\
uvm2 &    4.2 &  0.198 \\
uvm2 &    4.3 &  0.208 \\
uvm2 &    4.4 &  0.217 \\
uvm2 &    4.5 &  0.227 \\
uvm2 &    4.6 &  0.237 \\
uvm2 &    4.7 &  0.247 \\
uvm2 &    4.8 &  0.257 \\
uvm2 &    4.9 &  0.267 \\
uvm2 &    5.0 &  0.278 \\
uvm2 &    5.1 &  0.288 \\
uvm2 &    5.2 &  0.299 \\
uvm2 &    5.3 &  0.310 \\
uvm2 &    5.4 &  0.321 \\
uvm2 &    5.5 &  0.332 \\
uvm2 &    5.6 &  0.343 \\
uvm2 &    5.7 &  0.354 \\
uvm2 &    5.8 &  0.366 \\
uvm2 &    5.9 &  0.377 \\
uvm2 &    6.0 &  0.389 \\
uvm2 &    6.1 &  0.401 \\
uvm2 &    6.2 &  0.412 \\
uvm2 &    6.3 &  0.424 \\
uvm2 &    6.4 &  0.436 \\
uvm2 &    6.5 &  0.449 \\
uvm2 &    6.6 &  0.461 \\
uvm2 &    6.7 &  0.473 \\
uvm2 &    6.8 &  0.485 \\
uvm2 &    6.9 &  0.498 \\
uvm2 &    7.0 &  0.511 \\
uvm2 &    7.1 &  0.523 \\
uvm2 &    7.2 &  0.536 \\
uvm2 &    7.3 &  0.549 \\
uvm2 &    7.4 &  0.562 \\
uvm2 &    7.5 &  0.574 \\
uvm2 &    7.6 &  0.587 \\
uvm2 &    7.7 &  0.600 \\
uvm2 &    7.8 &  0.614 \\
uvm2 &    7.9 &  0.627 \\
uvm2 &    8.0 &  0.640 \\
uvm2 &    8.1 &  0.653 \\
uvm2 &    8.2 &  0.667 \\
uvm2 &    8.3 &  0.680 \\
uvm2 &    8.4 &  0.693 \\
uvm2 &    8.5 &  0.707 \\
uvm2 &    8.6 &  0.720 \\
uvm2 &    8.7 &  0.734 \\
uvm2 &    8.8 &  0.748 \\
uvm2 &    8.9 &  0.761 \\
uvm2 &    9.0 &  0.775 \\
uvm2 &    9.1 &  0.789 \\
uvm2 &    9.2 &  0.802 \\
uvm2 &    9.3 &  0.816 \\
uvm2 &    9.4 &  0.830 \\
uvm2 &    9.5 &  0.844 \\
uvm2 &    9.6 &  0.858 \\
uvm2 &    9.7 &  0.872 \\
uvm2 &    9.8 &  0.885 \\
uvm2 &    9.9 &  0.899 \\
uvm2 &   10.0 &  0.913 \\
uvm2 &   10.1 &  0.927 \\
uvm2 &   10.2 &  0.941 \\
uvm2 &   10.3 &  0.955 \\
uvm2 &   10.4 &  0.969 \\
uvm2 &   10.5 &  0.983 \\
uvm2 &   10.6 &  0.997 \\
uvm2 &   10.7 &  1.011 \\
uvm2 &   10.8 &  1.025 \\
uvm2 &   10.9 &  1.039 \\
uvm2 &   11.0 &  1.053 \\
uvm2 &   11.1 &  1.067 \\
uvm2 &   11.2 &  1.081 \\
uvm2 &   11.3 &  1.095 \\
uvm2 &   11.4 &  1.109 \\
uvm2 &   11.5 &  1.123 \\
uvm2 &   11.6 &  1.137 \\
uvm2 &   11.7 &  1.151 \\
uvm2 &   11.8 &  1.165 \\
uvm2 &   11.9 &  1.179 \\
uvm2 &   12.0 &  1.193 \\
uvm2 &   12.1 &  1.207 \\
uvm2 &   12.2 &  1.220 \\
uvm2 &   12.3 &  1.234 \\
uvm2 &   12.4 &  1.248 \\
uvm2 &   12.5 &  1.262 \\
uvm2 &   12.6 &  1.276 \\
uvm2 &   12.7 &  1.289 \\
uvm2 &   12.8 &  1.303 \\
uvm2 &   12.9 &  1.317 \\
uvm2 &   13.0 &  1.331 \\
uvm2 &   13.1 &  1.344 \\
uvm2 &   13.2 &  1.358 \\
uvm2 &   13.3 &  1.372 \\
uvm2 &   13.4 &  1.385 \\
uvm2 &   13.5 &  1.399 \\
uvm2 &   13.6 &  1.412 \\
uvm2 &   13.7 &  1.426 \\
uvm2 &   13.8 &  1.439 \\
uvm2 &   13.9 &  1.452 \\
uvm2 &   14.0 &  1.466 \\
uvm2 &   14.1 &  1.479 \\
uvm2 &   14.2 &  1.492 \\
uvm2 &   14.3 &  1.506 \\
uvm2 &   14.4 &  1.519 \\
uvm2 &   14.5 &  1.532 \\
uvm2 &   14.6 &  1.545 \\
uvm2 &   14.7 &  1.558 \\
uvm2 &   14.8 &  1.571 \\
uvm2 &   14.9 &  1.584 \\
uvm2 &   15.0 &  1.597 \\
uvm2 &   15.1 &  1.610 \\
uvm2 &   15.2 &  1.623 \\
uvm2 &   15.3 &  1.636 \\
uvm2 &   15.4 &  1.648 \\
uvm2 &   15.5 &  1.661 \\
uvm2 &   15.6 &  1.674 \\
uvm2 &   15.7 &  1.686 \\
uvm2 &   15.8 &  1.699 \\
uvm2 &   15.9 &  1.711 \\
uvm2 &   16.0 &  1.724 \\
uvm2 &   16.1 &  1.736 \\
uvm2 &   16.2 &  1.749 \\
uvm2 &   16.3 &  1.761 \\
uvm2 &   16.4 &  1.773 \\
uvm2 &   16.5 &  1.785 \\
uvm2 &   16.6 &  1.797 \\
uvm2 &   16.7 &  1.809 \\
uvm2 &   16.8 &  1.821 \\
uvm2 &   16.9 &  1.833 \\
uvm2 &   17.0 &  1.845 \\
uvm2 &   17.1 &  1.857 \\
uvm2 &   17.2 &  1.869 \\
uvm2 &   17.3 &  1.880 \\
uvm2 &   17.4 &  1.892 \\
uvm2 &   17.5 &  1.904 \\
uvm2 &   17.6 &  1.915 \\
uvm2 &   17.7 &  1.927 \\
uvm2 &   17.8 &  1.938 \\
uvm2 &   17.9 &  1.949 \\
uvm2 &   18.0 &  1.961 \\
uvm2 &   18.1 &  1.972 \\
uvm2 &   18.2 &  1.983 \\
uvm2 &   18.3 &  1.994 \\
uvm2 &   18.4 &  2.005 \\
uvm2 &   18.5 &  2.016 \\
uvm2 &   18.6 &  2.027 \\
uvm2 &   18.7 &  2.038 \\
uvm2 &   18.8 &  2.048 \\
uvm2 &   18.9 &  2.059 \\
uvm2 &   19.0 &  2.070 \\
uvm2 &   19.1 &  2.080 \\
uvm2 &   19.2 &  2.091 \\
uvm2 &   19.3 &  2.101 \\
uvm2 &   19.4 &  2.112 \\
uvm2 &   19.5 &  2.122 \\
uvm2 &   19.6 &  2.132 \\
uvm2 &   19.7 &  2.142 \\
uvm2 &   19.8 &  2.152 \\
uvm2 &   19.9 &  2.162 \\
uvm2 &   20.0 &  2.172 \\
uvm2 &   20.1 &  2.182 \\
uvm2 &   20.2 &  2.192 \\
uvm2 &   20.3 &  2.202 \\
uvm2 &   20.4 &  2.212 \\
uvm2 &   20.5 &  2.221 \\
uvm2 &   20.6 &  2.231 \\
uvm2 &   20.7 &  2.240 \\
uvm2 &   20.8 &  2.250 \\
uvm2 &   20.9 &  2.259 \\
uvm2 &   21.0 &  2.268 \\
uvm2 &   21.1 &  2.278 \\
uvm2 &   21.2 &  2.287 \\
uvm2 &   21.3 &  2.296 \\
uvm2 &   21.4 &  2.305 \\
uvm2 &   21.5 &  2.314 \\
uvm2 &   21.6 &  2.323 \\
uvm2 &   21.7 &  2.332 \\
uvm2 &   21.8 &  2.341 \\
uvm2 &   21.9 &  2.349 \\
uvm2 &   22.0 &  2.358 \\
uvm2 &   22.1 &  2.366 \\
uvm2 &   22.2 &  2.375 \\
uvm2 &   22.3 &  2.383 \\
uvm2 &   22.4 &  2.392 \\
uvm2 &   22.5 &  2.400 \\
uvm2 &   22.6 &  2.408 \\
uvm2 &   22.7 &  2.417 \\
uvm2 &   22.8 &  2.425 \\
uvm2 &   22.9 &  2.433 \\
uvm2 &   23.0 &  2.441 \\
uvm2 &   23.1 &  2.449 \\
uvm2 &   23.2 &  2.457 \\
uvm2 &   23.3 &  2.465 \\
uvm2 &   23.4 &  2.472 \\
uvm2 &   23.5 &  2.480 \\
uvm2 &   23.6 &  2.488 \\
uvm2 &   23.7 &  2.495 \\
uvm2 &   23.8 &  2.503 \\
uvm2 &   23.9 &  2.510 \\
uvm2 &   24.0 &  2.518 \\
uvm2 &   24.1 &  2.525 \\
uvm2 &   24.2 &  2.532 \\
uvm2 &   24.3 &  2.539 \\
uvm2 &   24.4 &  2.547 \\
uvm2 &   24.5 &  2.554 \\
uvm2 &   24.6 &  2.561 \\
uvm2 &   24.7 &  2.568 \\
uvm2 &   24.8 &  2.575 \\
uvm2 &   24.9 &  2.581 \\
uvm2 &   25.0 &  2.588 \\
uvm2 &   25.1 &  2.595 \\
uvm2 &   25.2 &  2.602 \\
uvm2 &   25.3 &  2.608 \\
uvm2 &   25.4 &  2.615 \\
uvm2 &   25.5 &  2.622 \\
uvm2 &   25.6 &  2.628 \\
uvm2 &   25.7 &  2.634 \\
uvm2 &   25.8 &  2.641 \\
uvm2 &   25.9 &  2.647 \\
uvm2 &   26.0 &  2.653 \\
uvm2 &   26.1 &  2.660 \\
uvm2 &   26.2 &  2.666 \\
uvm2 &   26.3 &  2.672 \\
uvm2 &   26.4 &  2.678 \\
uvm2 &   26.5 &  2.684 \\
uvm2 &   26.6 &  2.690 \\
uvm2 &   26.7 &  2.696 \\
uvm2 &   26.8 &  2.702 \\
uvm2 &   26.9 &  2.707 \\
uvm2 &   27.0 &  2.713 \\
uvm2 &   27.1 &  2.719 \\
uvm2 &   27.2 &  2.725 \\
uvm2 &   27.3 &  2.730 \\
uvm2 &   27.4 &  2.736 \\
uvm2 &   27.5 &  2.741 \\
uvm2 &   27.6 &  2.747 \\
uvm2 &   27.7 &  2.752 \\
uvm2 &   27.8 &  2.758 \\
uvm2 &   27.9 &  2.763 \\
uvm2 &   28.0 &  2.768 \\
uvm2 &   28.1 &  2.773 \\
uvm2 &   28.2 &  2.779 \\
uvm2 &   28.3 &  2.784 \\
uvm2 &   28.4 &  2.789 \\
uvm2 &   28.5 &  2.794 \\
uvm2 &   28.6 &  2.799 \\
uvm2 &   28.7 &  2.804 \\
uvm2 &   28.8 &  2.809 \\
uvm2 &   28.9 &  2.814 \\
uvm2 &   29.0 &  2.819 \\
uvm2 &   29.1 &  2.824 \\
uvm2 &   29.2 &  2.829 \\
uvm2 &   29.3 &  2.833 \\
uvm2 &   29.4 &  2.838 \\
uvm2 &   29.5 &  2.843 \\
uvm2 &   29.6 &  2.848 \\
uvm2 &   29.7 &  2.852 \\
uvm2 &   29.8 &  2.857 \\
uvm2 &   29.9 &  2.861 \\
uvm2 &   30.0 &  2.866 \\
uvm2 &   30.1 &  2.871 \\
uvm2 &   30.2 &  2.875 \\
uvm2 &   30.3 &  2.879 \\
uvm2 &   30.4 &  2.884 \\
uvm2 &   30.5 &  2.888 \\
uvm2 &   30.6 &  2.893 \\
uvm2 &   30.7 &  2.897 \\
uvm2 &   30.8 &  2.901 \\
uvm2 &   30.9 &  2.906 \\
uvm2 &   31.0 &  2.910 \\
uvm2 &   31.1 &  2.914 \\
uvm2 &   31.2 &  2.918 \\
uvm2 &   31.3 &  2.922 \\
uvm2 &   31.4 &  2.927 \\
uvm2 &   31.5 &  2.931 \\
uvm2 &   31.6 &  2.935 \\
uvm2 &   31.7 &  2.939 \\
uvm2 &   31.8 &  2.943 \\
uvm2 &   31.9 &  2.947 \\
uvm2 &   32.0 &  2.951 \\
uvm2 &   32.1 &  2.955 \\
uvm2 &   32.2 &  2.959 \\
uvm2 &   32.3 &  2.963 \\
uvm2 &   32.4 &  2.967 \\
uvm2 &   32.5 &  2.971 \\
uvm2 &   32.6 &  2.975 \\
uvm2 &   32.7 &  2.979 \\
uvm2 &   32.8 &  2.982 \\
uvm2 &   32.9 &  2.986 \\
uvm2 &   33.0 &  2.990 \\
uvm2 &   33.1 &  2.994 \\
uvm2 &   33.2 &  2.998 \\
uvm2 &   33.3 &  3.001 \\
uvm2 &   33.4 &  3.005 \\
uvm2 &   33.5 &  3.009 \\
uvm2 &   33.6 &  3.013 \\
uvm2 &   33.7 &  3.016 \\
uvm2 &   33.8 &  3.020 \\
uvm2 &   33.9 &  3.024 \\
uvm2 &   34.0 &  3.028 \\
uvm2 &   34.1 &  3.031 \\
uvm2 &   34.2 &  3.035 \\
uvm2 &   34.3 &  3.039 \\
uvm2 &   34.4 &  3.042 \\
uvm2 &   34.5 &  3.046 \\
uvm2 &   34.6 &  3.050 \\
uvm2 &   34.7 &  3.053 \\
uvm2 &   34.8 &  3.057 \\
uvm2 &   34.9 &  3.060 \\
uvm2 &   35.0 &  3.064 \\
uvm2 &   35.1 &  3.068 \\
uvm2 &   35.2 &  3.071 \\
uvm2 &   35.3 &  3.075 \\
uvm2 &   35.4 &  3.079 \\
uvm2 &   35.5 &  3.082 \\
uvm2 &   35.6 &  3.086 \\
uvm2 &   35.7 &  3.089 \\
uvm2 &   35.8 &  3.093 \\
uvm2 &   35.9 &  3.096 \\
uvm2 &   36.0 &  3.100 \\
uvm2 &   36.1 &  3.104 \\
uvm2 &   36.2 &  3.107 \\
uvm2 &   36.3 &  3.111 \\
uvm2 &   36.4 &  3.114 \\
uvm2 &   36.5 &  3.118 \\
uvm2 &   36.6 &  3.122 \\
uvm2 &   36.7 &  3.125 \\
uvm2 &   36.8 &  3.129 \\
uvm2 &   36.9 &  3.132 \\
uvm2 &   37.0 &  3.136 \\
uvm2 &   37.1 &  3.140 \\
uvm2 &   37.2 &  3.143 \\
uvm2 &   37.3 &  3.147 \\
uvm2 &   37.4 &  3.150 \\
uvm2 &   37.5 &  3.154 \\
uvm2 &   37.6 &  3.158 \\
uvm2 &   37.7 &  3.161 \\
uvm2 &   37.8 &  3.165 \\
uvm2 &   37.9 &  3.169 \\
uvm2 &   38.0 &  3.172 \\
uvm2 &   38.1 &  3.176 \\
uvm2 &   38.2 &  3.179 \\
uvm2 &   38.3 &  3.183 \\
uvm2 &   38.4 &  3.187 \\
uvm2 &   38.5 &  3.190 \\
uvm2 &   38.6 &  3.194 \\
uvm2 &   38.7 &  3.198 \\
uvm2 &   38.8 &  3.202 \\
uvm2 &   38.9 &  3.205 \\
uvm2 &   39.0 &  3.209 \\
uvm2 &   39.1 &  3.213 \\
uvm2 &   39.2 &  3.216 \\
uvm2 &   39.3 &  3.220 \\
uvm2 &   39.4 &  3.224 \\
uvm2 &   39.5 &  3.228 \\
uvm2 &   39.6 &  3.232 \\
uvm2 &   39.7 &  3.235 \\
uvm2 &   39.8 &  3.239 \\
uvm2 &   39.9 &  3.243 \\
uvm2 &   40.0 &  3.247 \\
uvm2 &   40.1 &  3.251 \\
uvm2 &   40.2 &  3.254 \\
uvm2 &   40.3 &  3.258 \\
uvm2 &   40.4 &  3.262 \\
uvm2 &   40.5 &  3.266 \\
uvm2 &   40.6 &  3.270 \\
uvm2 &   40.7 &  3.274 \\
uvm2 &   40.8 &  3.278 \\
uvm2 &   40.9 &  3.282 \\
uvm2 &   41.0 &  3.286 \\
uvm2 &   41.1 &  3.290 \\
uvm2 &   41.2 &  3.294 \\
uvm2 &   41.3 &  3.298 \\
uvm2 &   41.4 &  3.302 \\
uvm2 &   41.5 &  3.306 \\
uvm2 &   41.6 &  3.310 \\
uvm2 &   41.7 &  3.314 \\
uvm2 &   41.8 &  3.318 \\
uvm2 &   41.9 &  3.322 \\
uvm2 &   42.0 &  3.326 \\
uvm2 &   42.1 &  3.330 \\
uvm2 &   42.2 &  3.334 \\
uvm2 &   42.3 &  3.338 \\
uvm2 &   42.4 &  3.342 \\
uvm2 &   42.5 &  3.346 \\
uvm2 &   42.6 &  3.351 \\
uvm2 &   42.7 &  3.355 \\
uvm2 &   42.8 &  3.359 \\
uvm2 &   42.9 &  3.363 \\
uvm2 &   43.0 &  3.367 \\
uvm2 &   43.1 &  3.371 \\
uvm2 &   43.2 &  3.376 \\
uvm2 &   43.3 &  3.380 \\
uvm2 &   43.4 &  3.384 \\
uvm2 &   43.5 &  3.388 \\
uvm2 &   43.6 &  3.393 \\
uvm2 &   43.7 &  3.397 \\
uvm2 &   43.8 &  3.401 \\
uvm2 &   43.9 &  3.406 \\
uvm2 &   44.0 &  3.410 \\
uvm2 &   44.1 &  3.414 \\
uvm2 &   44.2 &  3.418 \\
uvm2 &   44.3 &  3.423 \\
uvm2 &   44.4 &  3.427 \\
uvm2 &   44.5 &  3.432 \\
uvm2 &   44.6 &  3.436 \\
uvm2 &   44.7 &  3.440 \\
uvm2 &   44.8 &  3.445 \\
uvm2 &   44.9 &  3.449 \\
uvm2 &   45.0 &  3.453 \\
uvm2 &   45.1 &  3.458 \\
uvm2 &   45.2 &  3.462 \\
uvm2 &   45.3 &  3.467 \\
uvm2 &   45.4 &  3.471 \\
uvm2 &   45.5 &  3.475 \\
uvm2 &   45.6 &  3.480 \\
uvm2 &   45.7 &  3.484 \\
uvm2 &   45.8 &  3.489 \\
uvm2 &   45.9 &  3.493 \\
uvm2 &   46.0 &  3.498 \\
uvm2 &   46.1 &  3.502 \\
uvm2 &   46.2 &  3.506 \\
uvm2 &   46.3 &  3.511 \\
uvm2 &   46.4 &  3.515 \\
uvm2 &   46.5 &  3.520 \\
uvm2 &   46.6 &  3.524 \\
uvm2 &   46.7 &  3.529 \\
uvm2 &   46.8 &  3.533 \\
uvm2 &   46.9 &  3.538 \\
uvm2 &   47.0 &  3.542 \\
uvm2 &   47.1 &  3.546 \\
uvm2 &   47.2 &  3.551 \\
uvm2 &   47.3 &  3.555 \\
uvm2 &   47.4 &  3.560 \\
uvm2 &   47.5 &  3.564 \\
uvm2 &   47.6 &  3.568 \\
uvm2 &   47.7 &  3.573 \\
uvm2 &   47.8 &  3.577 \\
uvm2 &   47.9 &  3.582 \\
uvm2 &   48.0 &  3.586 \\
uvm2 &   48.1 &  3.590 \\
uvm2 &   48.2 &  3.595 \\
uvm2 &   48.3 &  3.599 \\
uvm2 &   48.4 &  3.603 \\
uvm2 &   48.5 &  3.608 \\
uvm2 &   48.6 &  3.612 \\
uvm2 &   48.7 &  3.616 \\
uvm2 &   48.8 &  3.620 \\
uvm2 &   48.9 &  3.625 \\
uvm2 &   49.0 &  3.629 \\
uvm2 &   49.1 &  3.633 \\
uvm2 &   49.2 &  3.637 \\
uvm2 &   49.3 &  3.641 \\
uvm2 &   49.4 &  3.646 \\
uvm2 &   49.5 &  3.650 \\
uvm2 &   49.6 &  3.654 \\
uvm2 &   49.7 &  3.658 \\
uvm2 &   49.8 &  3.662 \\
uvm2 &   49.9 &  3.666 \\
uvm2 &   50.0 &  3.670 \\
uvw1 &  -15.0 &  8.207 \\
uvw1 &  -14.9 &  7.980 \\
uvw1 &  -14.8 &  7.765 \\
uvw1 &  -14.7 &  7.560 \\
uvw1 &  -14.6 &  7.365 \\
uvw1 &  -14.5 &  7.180 \\
uvw1 &  -14.4 &  7.003 \\
uvw1 &  -14.3 &  6.836 \\
uvw1 &  -14.2 &  6.676 \\
uvw1 &  -14.1 &  6.523 \\
uvw1 &  -14.0 &  6.378 \\
uvw1 &  -13.9 &  6.239 \\
uvw1 &  -13.8 &  6.106 \\
uvw1 &  -13.7 &  5.978 \\
uvw1 &  -13.6 &  5.856 \\
uvw1 &  -13.5 &  5.739 \\
uvw1 &  -13.4 &  5.626 \\
uvw1 &  -13.3 &  5.518 \\
uvw1 &  -13.2 &  5.413 \\
uvw1 &  -13.1 &  5.312 \\
uvw1 &  -13.0 &  5.214 \\
uvw1 &  -12.9 &  5.119 \\
uvw1 &  -12.8 &  5.027 \\
uvw1 &  -12.7 &  4.937 \\
uvw1 &  -12.6 &  4.850 \\
uvw1 &  -12.5 &  4.764 \\
uvw1 &  -12.4 &  4.681 \\
uvw1 &  -12.3 &  4.599 \\
uvw1 &  -12.2 &  4.519 \\
uvw1 &  -12.1 &  4.440 \\
uvw1 &  -12.0 &  4.363 \\
uvw1 &  -11.9 &  4.286 \\
uvw1 &  -11.8 &  4.211 \\
uvw1 &  -11.7 &  4.136 \\
uvw1 &  -11.6 &  4.062 \\
uvw1 &  -11.5 &  3.989 \\
uvw1 &  -11.4 &  3.917 \\
uvw1 &  -11.3 &  3.845 \\
uvw1 &  -11.2 &  3.773 \\
uvw1 &  -11.1 &  3.702 \\
uvw1 &  -11.0 &  3.632 \\
uvw1 &  -10.9 &  3.561 \\
uvw1 &  -10.8 &  3.491 \\
uvw1 &  -10.7 &  3.422 \\
uvw1 &  -10.6 &  3.352 \\
uvw1 &  -10.5 &  3.283 \\
uvw1 &  -10.4 &  3.214 \\
uvw1 &  -10.3 &  3.145 \\
uvw1 &  -10.2 &  3.077 \\
uvw1 &  -10.1 &  3.008 \\
uvw1 &  -10.0 &  2.940 \\
uvw1 &   -9.9 &  2.872 \\
uvw1 &   -9.8 &  2.805 \\
uvw1 &   -9.7 &  2.737 \\
uvw1 &   -9.6 &  2.670 \\
uvw1 &   -9.5 &  2.604 \\
uvw1 &   -9.4 &  2.538 \\
uvw1 &   -9.3 &  2.472 \\
uvw1 &   -9.2 &  2.406 \\
uvw1 &   -9.1 &  2.341 \\
uvw1 &   -9.0 &  2.277 \\
uvw1 &   -8.9 &  2.213 \\
uvw1 &   -8.8 &  2.149 \\
uvw1 &   -8.7 &  2.087 \\
uvw1 &   -8.6 &  2.024 \\
uvw1 &   -8.5 &  1.963 \\
uvw1 &   -8.4 &  1.902 \\
uvw1 &   -8.3 &  1.842 \\
uvw1 &   -8.2 &  1.783 \\
uvw1 &   -8.1 &  1.725 \\
uvw1 &   -8.0 &  1.667 \\
uvw1 &   -7.9 &  1.611 \\
uvw1 &   -7.8 &  1.555 \\
uvw1 &   -7.7 &  1.500 \\
uvw1 &   -7.6 &  1.447 \\
uvw1 &   -7.5 &  1.394 \\
uvw1 &   -7.4 &  1.342 \\
uvw1 &   -7.3 &  1.292 \\
uvw1 &   -7.2 &  1.242 \\
uvw1 &   -7.1 &  1.194 \\
uvw1 &   -7.0 &  1.147 \\
uvw1 &   -6.9 &  1.101 \\
uvw1 &   -6.8 &  1.057 \\
uvw1 &   -6.7 &  1.013 \\
uvw1 &   -6.6 &  0.971 \\
uvw1 &   -6.5 &  0.930 \\
uvw1 &   -6.4 &  0.890 \\
uvw1 &   -6.3 &  0.852 \\
uvw1 &   -6.2 &  0.814 \\
uvw1 &   -6.1 &  0.778 \\
uvw1 &   -6.0 &  0.744 \\
uvw1 &   -5.9 &  0.710 \\
uvw1 &   -5.8 &  0.678 \\
uvw1 &   -5.7 &  0.647 \\
uvw1 &   -5.6 &  0.618 \\
uvw1 &   -5.5 &  0.589 \\
uvw1 &   -5.4 &  0.562 \\
uvw1 &   -5.3 &  0.536 \\
uvw1 &   -5.2 &  0.511 \\
uvw1 &   -5.1 &  0.487 \\
uvw1 &   -5.0 &  0.465 \\
uvw1 &   -4.9 &  0.443 \\
uvw1 &   -4.8 &  0.423 \\
uvw1 &   -4.7 &  0.403 \\
uvw1 &   -4.6 &  0.385 \\
uvw1 &   -4.5 &  0.368 \\
uvw1 &   -4.4 &  0.351 \\
uvw1 &   -4.3 &  0.336 \\
uvw1 &   -4.2 &  0.321 \\
uvw1 &   -4.1 &  0.307 \\
uvw1 &   -4.0 &  0.294 \\
uvw1 &   -3.9 &  0.282 \\
uvw1 &   -3.8 &  0.270 \\
uvw1 &   -3.8 &  0.271 \\
uvw1 &   -3.7 &  0.256 \\
uvw1 &   -3.6 &  0.241 \\
uvw1 &   -3.5 &  0.226 \\
uvw1 &   -3.4 &  0.213 \\
uvw1 &   -3.3 &  0.199 \\
uvw1 &   -3.2 &  0.186 \\
uvw1 &   -3.1 &  0.174 \\
uvw1 &   -3.0 &  0.162 \\
uvw1 &   -2.9 &  0.151 \\
uvw1 &   -2.8 &  0.140 \\
uvw1 &   -2.7 &  0.129 \\
uvw1 &   -2.6 &  0.119 \\
uvw1 &   -2.5 &  0.110 \\
uvw1 &   -2.4 &  0.100 \\
uvw1 &   -2.3 &  0.092 \\
uvw1 &   -2.2 &  0.083 \\
uvw1 &   -2.1 &  0.076 \\
uvw1 &   -2.0 &  0.068 \\
uvw1 &   -1.9 &  0.061 \\
uvw1 &   -1.8 &  0.055 \\
uvw1 &   -1.7 &  0.048 \\
uvw1 &   -1.6 &  0.043 \\
uvw1 &   -1.5 &  0.037 \\
uvw1 &   -1.4 &  0.032 \\
uvw1 &   -1.3 &  0.028 \\
uvw1 &   -1.2 &  0.023 \\
uvw1 &   -1.1 &  0.020 \\
uvw1 &   -1.0 &  0.016 \\
uvw1 &   -0.9 &  0.013 \\
uvw1 &   -0.8 &  0.010 \\
uvw1 &   -0.7 &  0.008 \\
uvw1 &   -0.6 &  0.006 \\
uvw1 &   -0.5 &  0.004 \\
uvw1 &   -0.4 &  0.002 \\
uvw1 &   -0.3 &  0.001 \\
uvw1 &   -0.2 &  0.001 \\
uvw1 &   -0.1 &  0.000 \\
uvw1 &    0.0 & -0.000 \\
uvw1 &    0.1 &  0.000 \\
uvw1 &    0.2 &  0.001 \\
uvw1 &    0.3 &  0.001 \\
uvw1 &    0.4 &  0.002 \\
uvw1 &    0.5 &  0.004 \\
uvw1 &    0.6 &  0.005 \\
uvw1 &    0.7 &  0.007 \\
uvw1 &    0.8 &  0.009 \\
uvw1 &    0.9 &  0.012 \\
uvw1 &    1.0 &  0.014 \\
uvw1 &    1.1 &  0.017 \\
uvw1 &    1.2 &  0.020 \\
uvw1 &    1.3 &  0.024 \\
uvw1 &    1.4 &  0.027 \\
uvw1 &    1.5 &  0.031 \\
uvw1 &    1.6 &  0.035 \\
uvw1 &    1.7 &  0.039 \\
uvw1 &    1.8 &  0.044 \\
uvw1 &    1.9 &  0.048 \\
uvw1 &    2.0 &  0.053 \\
uvw1 &    2.1 &  0.058 \\
uvw1 &    2.2 &  0.063 \\
uvw1 &    2.3 &  0.069 \\
uvw1 &    2.4 &  0.074 \\
uvw1 &    2.5 &  0.080 \\
uvw1 &    2.6 &  0.086 \\
uvw1 &    2.7 &  0.092 \\
uvw1 &    2.8 &  0.098 \\
uvw1 &    2.9 &  0.105 \\
uvw1 &    3.0 &  0.111 \\
uvw1 &    3.1 &  0.118 \\
uvw1 &    3.2 &  0.125 \\
uvw1 &    3.3 &  0.132 \\
uvw1 &    3.4 &  0.139 \\
uvw1 &    3.5 &  0.146 \\
uvw1 &    3.6 &  0.153 \\
uvw1 &    3.7 &  0.160 \\
uvw1 &    3.8 &  0.168 \\
uvw1 &    3.9 &  0.175 \\
uvw1 &    4.0 &  0.183 \\
uvw1 &    4.1 &  0.191 \\
uvw1 &    4.2 &  0.198 \\
uvw1 &    4.3 &  0.206 \\
uvw1 &    4.4 &  0.214 \\
uvw1 &    4.5 &  0.222 \\
uvw1 &    4.6 &  0.237 \\
uvw1 &    4.7 &  0.252 \\
uvw1 &    4.8 &  0.267 \\
uvw1 &    4.9 &  0.282 \\
uvw1 &    5.0 &  0.297 \\
uvw1 &    5.1 &  0.312 \\
uvw1 &    5.2 &  0.327 \\
uvw1 &    5.3 &  0.342 \\
uvw1 &    5.4 &  0.358 \\
uvw1 &    5.5 &  0.374 \\
uvw1 &    5.6 &  0.385 \\
uvw1 &    5.7 &  0.396 \\
uvw1 &    5.8 &  0.406 \\
uvw1 &    5.9 &  0.417 \\
uvw1 &    6.0 &  0.428 \\
uvw1 &    6.1 &  0.440 \\
uvw1 &    6.2 &  0.451 \\
uvw1 &    6.3 &  0.462 \\
uvw1 &    6.4 &  0.473 \\
uvw1 &    6.5 &  0.485 \\
uvw1 &    6.6 &  0.497 \\
uvw1 &    6.7 &  0.508 \\
uvw1 &    6.8 &  0.520 \\
uvw1 &    6.9 &  0.532 \\
uvw1 &    7.0 &  0.544 \\
uvw1 &    7.1 &  0.556 \\
uvw1 &    7.2 &  0.568 \\
uvw1 &    7.3 &  0.580 \\
uvw1 &    7.4 &  0.592 \\
uvw1 &    7.5 &  0.604 \\
uvw1 &    7.6 &  0.617 \\
uvw1 &    7.7 &  0.629 \\
uvw1 &    7.8 &  0.641 \\
uvw1 &    7.9 &  0.654 \\
uvw1 &    8.0 &  0.667 \\
uvw1 &    8.1 &  0.679 \\
uvw1 &    8.2 &  0.692 \\
uvw1 &    8.3 &  0.705 \\
uvw1 &    8.4 &  0.718 \\
uvw1 &    8.5 &  0.730 \\
uvw1 &    8.6 &  0.743 \\
uvw1 &    8.7 &  0.756 \\
uvw1 &    8.8 &  0.769 \\
uvw1 &    8.9 &  0.782 \\
uvw1 &    9.0 &  0.796 \\
uvw1 &    9.1 &  0.809 \\
uvw1 &    9.2 &  0.822 \\
uvw1 &    9.3 &  0.835 \\
uvw1 &    9.4 &  0.849 \\
uvw1 &    9.5 &  0.862 \\
uvw1 &    9.6 &  0.875 \\
uvw1 &    9.7 &  0.889 \\
uvw1 &    9.8 &  0.902 \\
uvw1 &    9.9 &  0.916 \\
uvw1 &   10.0 &  0.929 \\
uvw1 &   10.1 &  0.943 \\
uvw1 &   10.2 &  0.957 \\
uvw1 &   10.3 &  0.970 \\
uvw1 &   10.4 &  0.984 \\
uvw1 &   10.5 &  0.998 \\
uvw1 &   10.6 &  1.012 \\
uvw1 &   10.7 &  1.025 \\
uvw1 &   10.8 &  1.039 \\
uvw1 &   10.9 &  1.053 \\
uvw1 &   11.0 &  1.067 \\
uvw1 &   11.1 &  1.081 \\
uvw1 &   11.2 &  1.095 \\
uvw1 &   11.3 &  1.108 \\
uvw1 &   11.4 &  1.122 \\
uvw1 &   11.5 &  1.136 \\
uvw1 &   11.6 &  1.150 \\
uvw1 &   11.7 &  1.164 \\
uvw1 &   11.8 &  1.178 \\
uvw1 &   11.9 &  1.192 \\
uvw1 &   12.0 &  1.206 \\
uvw1 &   12.1 &  1.220 \\
uvw1 &   12.2 &  1.234 \\
uvw1 &   12.3 &  1.248 \\
uvw1 &   12.4 &  1.263 \\
uvw1 &   12.5 &  1.277 \\
uvw1 &   12.6 &  1.291 \\
uvw1 &   12.7 &  1.305 \\
uvw1 &   12.8 &  1.319 \\
uvw1 &   12.9 &  1.333 \\
uvw1 &   13.0 &  1.347 \\
uvw1 &   13.1 &  1.361 \\
uvw1 &   13.2 &  1.375 \\
uvw1 &   13.3 &  1.389 \\
uvw1 &   13.4 &  1.403 \\
uvw1 &   13.5 &  1.417 \\
uvw1 &   13.6 &  1.432 \\
uvw1 &   13.7 &  1.446 \\
uvw1 &   13.8 &  1.460 \\
uvw1 &   13.9 &  1.474 \\
uvw1 &   14.0 &  1.488 \\
uvw1 &   14.1 &  1.502 \\
uvw1 &   14.2 &  1.516 \\
uvw1 &   14.3 &  1.530 \\
uvw1 &   14.4 &  1.544 \\
uvw1 &   14.5 &  1.558 \\
uvw1 &   14.6 &  1.572 \\
uvw1 &   14.7 &  1.586 \\
uvw1 &   14.8 &  1.600 \\
uvw1 &   14.9 &  1.614 \\
uvw1 &   15.0 &  1.628 \\
uvw1 &   15.1 &  1.642 \\
uvw1 &   15.2 &  1.656 \\
uvw1 &   15.3 &  1.670 \\
uvw1 &   15.4 &  1.684 \\
uvw1 &   15.5 &  1.697 \\
uvw1 &   15.6 &  1.711 \\
uvw1 &   15.7 &  1.725 \\
uvw1 &   15.8 &  1.739 \\
uvw1 &   15.9 &  1.753 \\
uvw1 &   16.0 &  1.766 \\
uvw1 &   16.1 &  1.780 \\
uvw1 &   16.2 &  1.794 \\
uvw1 &   16.3 &  1.807 \\
uvw1 &   16.4 &  1.821 \\
uvw1 &   16.5 &  1.835 \\
uvw1 &   16.6 &  1.848 \\
uvw1 &   16.7 &  1.862 \\
uvw1 &   16.8 &  1.875 \\
uvw1 &   16.9 &  1.889 \\
uvw1 &   17.0 &  1.902 \\
uvw1 &   17.1 &  1.916 \\
uvw1 &   17.2 &  1.929 \\
uvw1 &   17.3 &  1.943 \\
uvw1 &   17.4 &  1.956 \\
uvw1 &   17.5 &  1.969 \\
uvw1 &   17.6 &  1.983 \\
uvw1 &   17.7 &  1.996 \\
uvw1 &   17.8 &  2.009 \\
uvw1 &   17.9 &  2.022 \\
uvw1 &   18.0 &  2.035 \\
uvw1 &   18.1 &  2.049 \\
uvw1 &   18.2 &  2.062 \\
uvw1 &   18.3 &  2.075 \\
uvw1 &   18.4 &  2.088 \\
uvw1 &   18.5 &  2.101 \\
uvw1 &   18.6 &  2.114 \\
uvw1 &   18.7 &  2.126 \\
uvw1 &   18.8 &  2.139 \\
uvw1 &   18.9 &  2.152 \\
uvw1 &   19.0 &  2.165 \\
uvw1 &   19.1 &  2.178 \\
uvw1 &   19.2 &  2.190 \\
uvw1 &   19.3 &  2.203 \\
uvw1 &   19.4 &  2.216 \\
uvw1 &   19.5 &  2.228 \\
uvw1 &   19.6 &  2.241 \\
uvw1 &   19.7 &  2.253 \\
uvw1 &   19.8 &  2.266 \\
uvw1 &   19.9 &  2.278 \\
uvw1 &   20.0 &  2.290 \\
uvw1 &   20.1 &  2.303 \\
uvw1 &   20.2 &  2.315 \\
uvw1 &   20.3 &  2.327 \\
uvw1 &   20.4 &  2.339 \\
uvw1 &   20.5 &  2.351 \\
uvw1 &   20.6 &  2.363 \\
uvw1 &   20.7 &  2.375 \\
uvw1 &   20.8 &  2.387 \\
uvw1 &   20.9 &  2.399 \\
uvw1 &   21.0 &  2.411 \\
uvw1 &   21.1 &  2.423 \\
uvw1 &   21.2 &  2.435 \\
uvw1 &   21.3 &  2.446 \\
uvw1 &   21.4 &  2.458 \\
uvw1 &   21.5 &  2.470 \\
uvw1 &   21.6 &  2.481 \\
uvw1 &   21.7 &  2.493 \\
uvw1 &   21.8 &  2.504 \\
uvw1 &   21.9 &  2.516 \\
uvw1 &   22.0 &  2.527 \\
uvw1 &   22.1 &  2.538 \\
uvw1 &   22.2 &  2.550 \\
uvw1 &   22.3 &  2.561 \\
uvw1 &   22.4 &  2.572 \\
uvw1 &   22.5 &  2.583 \\
uvw1 &   22.6 &  2.594 \\
uvw1 &   22.7 &  2.605 \\
uvw1 &   22.8 &  2.616 \\
uvw1 &   22.9 &  2.627 \\
uvw1 &   23.0 &  2.638 \\
uvw1 &   23.1 &  2.649 \\
uvw1 &   23.2 &  2.659 \\
uvw1 &   23.3 &  2.670 \\
uvw1 &   23.4 &  2.681 \\
uvw1 &   23.5 &  2.691 \\
uvw1 &   23.6 &  2.702 \\
uvw1 &   23.7 &  2.712 \\
uvw1 &   23.8 &  2.723 \\
uvw1 &   23.9 &  2.733 \\
uvw1 &   24.0 &  2.743 \\
uvw1 &   24.1 &  2.754 \\
uvw1 &   24.2 &  2.764 \\
uvw1 &   24.3 &  2.774 \\
uvw1 &   24.4 &  2.784 \\
uvw1 &   24.5 &  2.794 \\
uvw1 &   24.6 &  2.804 \\
uvw1 &   24.7 &  2.814 \\
uvw1 &   24.8 &  2.824 \\
uvw1 &   24.9 &  2.834 \\
uvw1 &   25.0 &  2.844 \\
uvw1 &   25.1 &  2.853 \\
uvw1 &   25.2 &  2.863 \\
uvw1 &   25.3 &  2.873 \\
uvw1 &   25.4 &  2.882 \\
uvw1 &   25.5 &  2.892 \\
uvw1 &   25.6 &  2.901 \\
uvw1 &   25.7 &  2.910 \\
uvw1 &   25.8 &  2.920 \\
uvw1 &   25.9 &  2.929 \\
uvw1 &   26.0 &  2.938 \\
uvw1 &   26.1 &  2.947 \\
uvw1 &   26.2 &  2.957 \\
uvw1 &   26.3 &  2.966 \\
uvw1 &   26.4 &  2.975 \\
uvw1 &   26.5 &  2.984 \\
uvw1 &   26.6 &  2.992 \\
uvw1 &   26.7 &  3.001 \\
uvw1 &   26.8 &  3.010 \\
uvw1 &   26.9 &  3.019 \\
uvw1 &   27.0 &  3.027 \\
uvw1 &   27.1 &  3.036 \\
uvw1 &   27.2 &  3.045 \\
uvw1 &   27.3 &  3.053 \\
uvw1 &   27.4 &  3.062 \\
uvw1 &   27.5 &  3.070 \\
uvw1 &   27.6 &  3.078 \\
uvw1 &   27.7 &  3.087 \\
uvw1 &   27.8 &  3.095 \\
uvw1 &   27.9 &  3.103 \\
uvw1 &   28.0 &  3.111 \\
uvw1 &   28.1 &  3.119 \\
uvw1 &   28.2 &  3.127 \\
uvw1 &   28.3 &  3.135 \\
uvw1 &   28.4 &  3.143 \\
uvw1 &   28.5 &  3.151 \\
uvw1 &   28.6 &  3.159 \\
uvw1 &   28.7 &  3.167 \\
uvw1 &   28.8 &  3.174 \\
uvw1 &   28.9 &  3.182 \\
uvw1 &   29.0 &  3.190 \\
uvw1 &   29.1 &  3.197 \\
uvw1 &   29.2 &  3.205 \\
uvw1 &   29.3 &  3.212 \\
uvw1 &   29.4 &  3.219 \\
uvw1 &   29.5 &  3.227 \\
uvw1 &   29.6 &  3.234 \\
uvw1 &   29.7 &  3.241 \\
uvw1 &   29.8 &  3.248 \\
uvw1 &   29.9 &  3.256 \\
uvw1 &   30.0 &  3.263 \\
uvw1 &   30.1 &  3.270 \\
uvw1 &   30.2 &  3.277 \\
uvw1 &   30.3 &  3.284 \\
uvw1 &   30.4 &  3.291 \\
uvw1 &   30.5 &  3.297 \\
uvw1 &   30.6 &  3.304 \\
uvw1 &   30.7 &  3.311 \\
uvw1 &   30.8 &  3.318 \\
uvw1 &   30.9 &  3.324 \\
uvw1 &   31.0 &  3.331 \\
uvw1 &   31.1 &  3.337 \\
uvw1 &   31.2 &  3.344 \\
uvw1 &   31.3 &  3.350 \\
uvw1 &   31.4 &  3.357 \\
uvw1 &   31.5 &  3.363 \\
uvw1 &   31.6 &  3.369 \\
uvw1 &   31.7 &  3.376 \\
uvw1 &   31.8 &  3.382 \\
uvw1 &   31.9 &  3.388 \\
uvw1 &   32.0 &  3.394 \\
uvw1 &   32.1 &  3.400 \\
uvw1 &   32.2 &  3.406 \\
uvw1 &   32.3 &  3.412 \\
uvw1 &   32.4 &  3.418 \\
uvw1 &   32.5 &  3.424 \\
uvw1 &   32.6 &  3.430 \\
uvw1 &   32.7 &  3.436 \\
uvw1 &   32.8 &  3.442 \\
uvw1 &   32.9 &  3.448 \\
uvw1 &   33.0 &  3.453 \\
uvw1 &   33.1 &  3.459 \\
uvw1 &   33.2 &  3.465 \\
uvw1 &   33.3 &  3.470 \\
uvw1 &   33.4 &  3.476 \\
uvw1 &   33.5 &  3.481 \\
uvw1 &   33.6 &  3.487 \\
uvw1 &   33.7 &  3.492 \\
uvw1 &   33.8 &  3.497 \\
uvw1 &   33.9 &  3.503 \\
uvw1 &   34.0 &  3.508 \\
uvw1 &   34.1 &  3.513 \\
uvw1 &   34.2 &  3.518 \\
uvw1 &   34.3 &  3.524 \\
uvw1 &   34.4 &  3.529 \\
uvw1 &   34.5 &  3.534 \\
uvw1 &   34.6 &  3.539 \\
uvw1 &   34.7 &  3.544 \\
uvw1 &   34.8 &  3.549 \\
uvw1 &   34.9 &  3.554 \\
uvw1 &   35.0 &  3.559 \\
uvw1 &   35.1 &  3.564 \\
uvw1 &   35.2 &  3.569 \\
uvw1 &   35.3 &  3.573 \\
uvw1 &   35.4 &  3.578 \\
uvw1 &   35.5 &  3.583 \\
uvw1 &   35.6 &  3.588 \\
uvw1 &   35.7 &  3.592 \\
uvw1 &   35.8 &  3.597 \\
uvw1 &   35.9 &  3.602 \\
uvw1 &   36.0 &  3.606 \\
uvw1 &   36.1 &  3.611 \\
uvw1 &   36.2 &  3.615 \\
uvw1 &   36.3 &  3.620 \\
uvw1 &   36.4 &  3.624 \\
uvw1 &   36.5 &  3.629 \\
uvw1 &   36.6 &  3.633 \\
uvw1 &   36.7 &  3.638 \\
uvw1 &   36.8 &  3.642 \\
uvw1 &   36.9 &  3.646 \\
uvw1 &   37.0 &  3.651 \\
uvw1 &   37.1 &  3.655 \\
uvw1 &   37.2 &  3.659 \\
uvw1 &   37.3 &  3.663 \\
uvw1 &   37.4 &  3.667 \\
uvw1 &   37.5 &  3.672 \\
uvw1 &   37.6 &  3.676 \\
uvw1 &   37.7 &  3.680 \\
uvw1 &   37.8 &  3.684 \\
uvw1 &   37.9 &  3.688 \\
uvw1 &   38.0 &  3.692 \\
uvw1 &   38.1 &  3.696 \\
uvw1 &   38.2 &  3.700 \\
uvw1 &   38.3 &  3.704 \\
uvw1 &   38.4 &  3.708 \\
uvw1 &   38.5 &  3.712 \\
uvw1 &   38.6 &  3.716 \\
uvw1 &   38.7 &  3.720 \\
uvw1 &   38.8 &  3.723 \\
uvw1 &   38.9 &  3.727 \\
uvw1 &   39.0 &  3.731 \\
uvw1 &   39.1 &  3.735 \\
uvw1 &   39.2 &  3.739 \\
uvw1 &   39.3 &  3.742 \\
uvw1 &   39.4 &  3.746 \\
uvw1 &   39.5 &  3.750 \\
uvw1 &   39.6 &  3.754 \\
uvw1 &   39.7 &  3.757 \\
uvw1 &   39.8 &  3.761 \\
uvw1 &   39.9 &  3.765 \\
uvw1 &   40.0 &  3.768 \\
uvw1 &   40.1 &  3.772 \\
uvw1 &   40.2 &  3.775 \\
uvw1 &   40.3 &  3.779 \\
uvw1 &   40.4 &  3.782 \\
uvw1 &   40.5 &  3.786 \\
uvw1 &   40.6 &  3.790 \\
uvw1 &   40.7 &  3.793 \\
uvw1 &   40.8 &  3.797 \\
uvw1 &   40.9 &  3.800 \\
uvw1 &   41.0 &  3.804 \\
uvw1 &   41.1 &  3.807 \\
uvw1 &   41.2 &  3.810 \\
uvw1 &   41.3 &  3.814 \\
uvw1 &   41.4 &  3.817 \\
uvw1 &   41.5 &  3.821 \\
uvw1 &   41.6 &  3.824 \\
uvw1 &   41.7 &  3.827 \\
uvw1 &   41.8 &  3.831 \\
uvw1 &   41.9 &  3.834 \\
uvw1 &   42.0 &  3.838 \\
uvw1 &   42.1 &  3.841 \\
uvw1 &   42.2 &  3.844 \\
uvw1 &   42.3 &  3.848 \\
uvw1 &   42.4 &  3.851 \\
uvw1 &   42.5 &  3.854 \\
uvw1 &   42.6 &  3.858 \\
uvw1 &   42.7 &  3.861 \\
uvw1 &   42.8 &  3.864 \\
uvw1 &   42.9 &  3.867 \\
uvw1 &   43.0 &  3.871 \\
uvw1 &   43.1 &  3.874 \\
uvw1 &   43.2 &  3.877 \\
uvw1 &   43.3 &  3.880 \\
uvw1 &   43.4 &  3.884 \\
uvw1 &   43.5 &  3.887 \\
uvw1 &   43.6 &  3.890 \\
uvw1 &   43.7 &  3.893 \\
uvw1 &   43.8 &  3.897 \\
uvw1 &   43.9 &  3.900 \\
uvw1 &   44.0 &  3.903 \\
uvw1 &   44.1 &  3.906 \\
uvw1 &   44.2 &  3.909 \\
uvw1 &   44.3 &  3.913 \\
uvw1 &   44.4 &  3.916 \\
uvw1 &   44.5 &  3.919 \\
uvw1 &   44.6 &  3.922 \\
uvw1 &   44.7 &  3.925 \\
uvw1 &   44.8 &  3.929 \\
uvw1 &   44.9 &  3.932 \\
uvw1 &   45.0 &  3.935 \\
uvw1 &   45.1 &  3.938 \\
uvw1 &   45.2 &  3.941 \\
uvw1 &   45.3 &  3.945 \\
uvw1 &   45.4 &  3.948 \\
uvw1 &   45.5 &  3.951 \\
uvw1 &   45.6 &  3.954 \\
uvw1 &   45.7 &  3.957 \\
uvw1 &   45.8 &  3.960 \\
uvw1 &   45.9 &  3.964 \\
uvw1 &   46.0 &  3.967 \\
uvw1 &   46.1 &  3.970 \\
uvw1 &   46.2 &  3.973 \\
uvw1 &   46.3 &  3.976 \\
uvw1 &   46.4 &  3.980 \\
uvw1 &   46.5 &  3.983 \\
uvw1 &   46.6 &  3.986 \\
uvw1 &   46.7 &  3.989 \\
uvw1 &   46.8 &  3.992 \\
uvw1 &   46.9 &  3.995 \\
uvw1 &   47.0 &  3.999 \\
uvw1 &   47.1 &  4.002 \\
uvw1 &   47.2 &  4.005 \\
uvw1 &   47.3 &  4.008 \\
uvw1 &   47.4 &  4.011 \\
uvw1 &   47.5 &  4.015 \\
uvw1 &   47.6 &  4.018 \\
uvw1 &   47.7 &  4.021 \\
uvw1 &   47.8 &  4.024 \\
uvw1 &   47.9 &  4.027 \\
uvw1 &   48.0 &  4.031 \\
uvw1 &   48.1 &  4.034 \\
uvw1 &   48.2 &  4.037 \\
uvw1 &   48.3 &  4.040 \\
uvw1 &   48.4 &  4.043 \\
uvw1 &   48.5 &  4.047 \\
uvw1 &   48.6 &  4.050 \\
uvw1 &   48.7 &  4.053 \\
uvw1 &   48.8 &  4.056 \\
uvw1 &   48.9 &  4.059 \\
uvw1 &   49.0 &  4.063 \\
uvw1 &   49.1 &  4.066 \\
uvw1 &   49.2 &  4.069 \\
uvw1 &   49.3 &  4.072 \\
uvw1 &   49.4 &  4.076 \\
uvw1 &   49.5 &  4.079 \\
uvw1 &   49.6 &  4.082 \\
uvw1 &   49.7 &  4.085 \\
uvw1 &   49.8 &  4.088 \\
uvw1 &   49.9 &  4.092 \\
uvw1 &   50.0 &  4.095 \\

